A Causal Inference Framework for Data Rich Environments

We propose a formal model for counterfactual estimation with unobserved confounding in "data-rich" settings, i.e., where there are a large number of units and a large number of measurements per unit. Our model provides a bridge between the structural causal model view of causal inference common in the graphical models literature with that of the latent factor model view common in the potential outcomes literature. We show how classic models for potential outcomes and treatment assignments fit within our framework. We provide an identification argument for the average treatment effect, the average treatment effect on the treated, and the average treatment effect on the untreated. For any estimator that has a fast enough estimation error rate for a certain nuisance parameter, we establish it is consistent for these various causal parameters. We then show principal component regression is one such estimator that leads to consistent estimation, and we analyze the minimal smoothness required of the potential outcomes function for consistency.

==> Old/archived/DAG_interpretation.tex <==
\section{DAG Interpretation}

Consider the causal diagram
\begin{center}
\begin{tikzpicture}
\node (A) at (0,0) {$A$};
\node (U) at (1.5,1) {$U$};
\node (Y) at (3,0) {$Y$};
\draw[thick, ->] (U) -- (A);
\draw[thick, ->] (U) -- (Y);
\draw[thick, ->] (A) -- (Y);
\end{tikzpicture}
\end{center}


Because other variables causing $A$ and $Y$ are not shown in the graph, they are considered independent (see, e.g., Pearl's Causality book, second edition, page 29). So this figure is a representation of 
\begin{align*}
Y &=f(A,U,\varepsilon),\\
A &=g(U,\nu),
\end{align*}
where $U$, $\varepsilon$, and $\nu$ are independent. That is, the figure is equivalent to 
\begin{center}
\begin{tikzpicture}
\node (A) at (0,0) {$A$};
\node (U) at (1,1) {$U$};
\node (Y) at (2,0) {$Y$};
\node (nu) at (-1,1) {$\nu$};
\node (varepsilon) at (3,1) {$\varepsilon$};
\draw[thick, ->] (U) -- (A);
\draw[thick, ->] (U) -- (Y);
\draw[thick, ->] (A) -- (Y);
\draw[thick, ->] (nu) -- (A);
\draw[thick, ->] (varepsilon) -- (Y);
\end{tikzpicture}
\end{center}

Suppose, however, that we start with models like
\begin{center}
\begin{tikzpicture}
\node (A) at (0,0) {$A$};
\node (U) at (1,1) {$U$};
\node (Y) at (2,0) {$Y$};
\node (nu) at (-1,1) {$\nu$};
\node (varepsilon) at (3,1) {$\varepsilon$};
\draw[thick, ->] (U) -- (A);
\draw[thick, ->] (U) -- (Y);
\draw[thick, ->] (A) -- (Y);
\draw[thick, ->] (nu) -- (A);
\draw[thick, ->] (varepsilon) -- (Y);
\draw[thick, ->] (U) -- (nu);
\end{tikzpicture}
\end{center}

or 
\begin{center}
\begin{tikzpicture}
\node (A) at (0,0) {$A$};
\node (U) at (1,1) {$U$};
\node (Y) at (2,0) {$Y$};
\node (nu) at (-1,1) {$\nu$};
\node (varepsilon) at (3,1) {$\varepsilon$};
\draw[thick, ->] (U) -- (A);
\draw[thick, ->] (U) -- (Y);
\draw[thick, ->] (A) -- (Y);
\draw[thick, ->] (nu) -- (A);
\draw[thick, ->] (varepsilon) -- (Y);
\draw[thick, ->] (varepsilon) -- (U);
\end{tikzpicture}
\end{center}

Given that we do not claim to observe $U$, it seems that the first graph would be without loss of generality. In the third graph, we can eliminate $\nu$, because $\nu$ is just mediating the effect of $U$ on $A$ (and $A$ could have extra independent causes not shown in the graph). In the fourth graph, we could merge $U$ and $\varepsilon$ into a ``new'' $U$ (and $Y$ could have extra independent causes not shown in the graph).
That is, it seems that we should be able to redefine $U$ to include all common causes of $A$ and $Y$ (observed or unobserved). Then, $U$ should be independent of all other determinants of $A$ and $Y$. Is this true? Can we make it precise? There must be a reference in the literature.

Also, once we condition on all common causes, $U$, we should have unconfoundedness conditional on $U$. Here is an argument. Backdoor paths, $A\leftarrow \cdots Y$, cannot have only $\leftarrow$ edges, because then the graph would be cyclic. They cannot have only $\rightarrow$ edges, because a backdoor path starts with $\leftarrow$. So, there should be at least an instance of $\leftarrow\rightarrow$. If there is also an instance of $\rightarrow\leftarrow$, the path is blocked by a collider and does not include common causes of $A$ and $Y$. If the path does not include a collider, then there is one instance of  $\leftarrow\rightarrow$. In that case, we have a common cause and the backdoor path is blocked by conditioning on the common cause. (There must be a much more elegant argument somewhere in the literature!)


Added on 8/24. From VanderWeele and Robins (2009) ``Minimal sufficient causation and directed acyclic graphs'',
\begin{quote}
``The requirement that the [$\varepsilon_i$] be mutually independent is essentially a requirement that there
is no variable absent from the graph which, if included on the graph, would be a
parent of two or more variables.''
\end{quote}
But any variable that we can add as a parent of two other variables to the first graph above becomes a common cause. So, except for the ``essentially'', this means that if we have all common causes in $U$ then
$U$, $\varepsilon$, and $\nu$ are independent.


Addressing Anish's concerns: If our conjecture is right, it is sufficient to put in $U$ all common causes. But that does not rule out other scenarios. Consider the following DAG.
\begin{center}
\begin{tikzpicture}
\node (A) at (0,0) {$A$};
\node (U) at (1,1) {$U$};
\node (Y) at (2,0) {$Y$};
\node (varepsilon) at (3,0) {$\varepsilon$};
\node (nu) at (-1,0) {$\nu$};
\draw[thick, ->] (U) -- (Y);
\draw[thick, ->] (A) -- (Y);
\draw[thick, ->] (nu) -- (A);
\draw[thick, ->] (varepsilon) -- (Y);
\end{tikzpicture}
\end{center}
This is the setting of an experiment. There are no common causes, but we can still write
\begin{align*}
%
A &= g(\nu), \quad 
%
Y = f(A, U, \varepsilon),
%
\end{align*}
with $U$, $\varepsilon$, and $\nu$ independent. So this is still a special case of our model. 


==> Old/archived/causal_framework.tex <==
\section{Causal Framework}\label{sec:framework}

{\bf Potential Outcomes.} 
We consider a framework with potential outcomes. Let there be $N \geq 1$ units of interest. For each unit, there are $T \geq 1$ measurements of interest. This can simply represent $T$ repeated one-dimensional measurements, or a $T$-dimensional single measurement, or combination of these two. For the time being, we shall not differentiate between these two models of measurement. But when we we later discuss the appropriate structural properties of our framework, these differentiation will play important role. Each unit can be subjected to interventions from a set $\bD$. For an intervention $d \in \bD$, let $Y_{ndt}$ be potential outcome random variable for unit $n$ under intervention $d$ for measurement $t \in [T]$\footnote{Throughout, we shall use notation $[T] = \{1,\dots, T\}$ for a positive integer $T \geq 1$.}.  In summary, the potential outcomes of interest is a random three-order tensor $\bY = [Y_{ndt} : n \in [N], d \in \bD, t \in [T]]$.

\noindent {\bf Data Availability.}  The potential outcomes corresponding to a subset of entries of the tensor $\bY$, denoted as $\Omega \subset [N]\times \bD \times [T]$, is observed. That is, for each $(n, d, t) \in \Omega$, $Y_{ndt}$ is observed. 

In general, we may additionally observe covariates or features associated with units, interventions
and measurement. Specifically, let $\balpha_n \in \Rb^{q_1}$ be the observed covariates associated with unit $n \in [N]$ with $q_1 \geq 1$, $\bbeta_t \in \Rb^{q_2}$ be the observed covariates associated with index or time $t \in [T]$  with $q_2 \geq 1$, and $\bgamma_d \in \Rb^{q_3}$ be the observed covariates associated with intervention $d \in \bD$ with $q_3 \geq 1$. 

\noindent {\bf Goal.} 
%% estimating the potential outcomes. moments.
The fundamental question of causal inference is the ability to estimate the distribution of the elements of the tensor $\bY = [Y_{ndt}: n \in [N], d\in \bD, t\in [T]]$. Now estimating the entire distribution can be extremely challenging, if not impossible, in most settings. Given that, a reasonable objective is estimating functional of the distribution. Formally, consider any measurable function $f: \Rb \to \Rb$. Then, a quantity of interest is $\Ex[f(\bY)] = [\Ex[f(Y_{ndt})]: n \in [N], d\in \bD, t\in [T]]$. For example, identity function $f(x) = x$ corresponds to estimating 
\begin{align} 
\Ex[f(\bY)] & = [\Ex[f(Y_{ndt})]: n \in [N], d\in \bD, t\in [T]].
\end{align}
Let $\bA = [A_{ndt}: n \in [N], d\in \bD, t\in [T]]$ denote the mean of tensor
$\bY$ with $A_{ndt} = \Ex[Y_{ndt}]$. Similarly, let $\bV = [V_{ndt}: n \in [N], d\in \bD, t\in [T]]$
denote the component-wise variance, i.e. $V_{ndt} = \Var[Y_{ndt}]$.

%
In this work, we shall focus on estimating $\bA$ and $\bV$. However, more general functional of distribution
of $\bY$ can be of interest.


\medskip
\noindent
{\bf Generative Model: Factorization, Confounders, Covariates.}
%% 
We describe generative model for $\bY, \Omega$. Along the way, we introduce factorization of 
tensors of interest, $\bA, \bV$ and discuss how it imposes structure that can be exploited for
estimation. We also discuss what sorts of confounded in the observations we permit through
dependencies between $\bY$ and $\Omega$. 

\medskip
\noindent{\em Latent Factors.} Let the latent factors associated unit $n \in [N]$ be $U_n$, 
intervention $d \in \bD$ be $W_d$ and index or time $t \in [T]$ be $Z_t$. 
%
Without loss of generality, let $U_n, W_d, Z_t \in \mathbb{R}^M$ for some $M \geq 1$. 
%
We shall assume that these latent factors $\LF = (U_n, W_d, Z_t: n \in [N], d \in \bD, t \in [T])$ 
are generated as per an arbitrary distribution and sampled once. 

\medskip
\noindent{\em Distribution of $\bY$, Tensor Factorization.} 
Given $\LF$, $\bY$ is generated as follows: for $n \in [N], d\in \bD, t\in [T]$,
\begin{align}\label{eq:potential}
    Y_{ndt} & = A_{ndt} + \varepsilon_{ndt}. 
\end{align}
Here $\bA = [A_{ndt}]$ is determined by $\LF$; precisely, 
\begin{align}
    A_{ntd} & = \sum_{r=1}^R u_{nr} v_{tr} w_{dr},
\end{align}
\textcolor{orange}{AA: Here, it may be good to include some examples. E.g., if 
\[
\bu_n = \left(\begin{array}{c}u_n\\1\\1\end{array}\right),\quad
\bv_t = \left(\begin{array}{c}1\\v_t\\1\end{array}\right),\quad
\bw_d = \left(\begin{array}{c}1\\1\\w_d\end{array}\right),
\]
then
\[
A_{ntd}= u_n+v_t+w_d.
\]
This is the ``two-way fixed-effects'' model for panel data. 
}

\textcolor{orange}{AA: Would not be easier to estimate average treatment effects?
\[
\frac{1}{N}\sum_{n=1}^N (Y_{nd_2t}-Y_{nd_1t})
\]
or alternatively
\[
\frac{1}{N}\sum_{n=1}^N (A_{nd_2t}-A_{nd_1t})
\]
As $N$ increases the difference between the two parameters go to zero in probability. Identification of these parameters (or, more fundamentally, identification of the average potential outcomes) is much easier because it does not require identification of the individual quantities.\\
}
where $\bu_n = [u_{nr}] \in \Rb^R$, $\bz_t = [z_{tr}] \in \Rb^R$,
and $\bw_d = [w_{dr}] \in \Rb^R$ with $\bu_n$ being deterministic, but
arbitrary map from $U_n$, $\bw_d$ being deterministic, but arbitrary map from  $W_d$ and 
$\bz_t$ being deterministic, but arbitrary map from $Z_t$. 
%
The random variables $\varepsilon_{ndt}$, $n \in [N], d \in \bD, t\in [T]$ are such 
that 
\begin{align}\label{eq:epsilon}
    \Ex[\varepsilon_{ndt} \,|\, \LF ] & = 0, \nonumber \\
    \Ex[\varepsilon_{ndt}^2 \,|\, \LF ] & = V_{ndt}. \nonumber \\
\end{align}
Therefore, $\Ex[\bY | \LF] = \bA$ and $\Var[Y_{ntd} | \LF] = V_{ndt}$. 
%
Further, let 
\begin{align}
    V_{ndt} & = \sum_{r=1}^{\Rp} \up_{nr}  \wp_{dr} \zp_{tr},
\end{align}
where $\bup_n = [\up_{nr}] \in \Rb^{\Rp}$, $\bzp_t = [\zp_{tr}] \in \Rb^{\Rp}$,
and $\bwp_d = [\wp_{dr}] \in \Rb^{\Rp}$ 
%
with $\bup_n$ being deterministic, but arbitrary map from $U_n$, $\bwp_d$ 
being deterministic, but arbitrary map from  $W_d$ and $\bzp_t$ being deterministic, but arbitrary map 
from $Z_t$.

\medskip
\noindent{\em $\LF$ as Confounders.} Recall that $\Omega$ represents the set of observed entries 
of potential outcome tensor $\bY$. We model $\Omega$ as arbitrary (potentially random) function of $\LF$. 
That is, $\LF$ acts as {\em confounders} that determine both the entries observed of potential outcome
tensor, i.e. $\Omega$ and the entries of the potential outcomes themselves, i.e. $\bY$. 

\medskip
\noindent{\em Selection on Latent Confounders.} We impose restriction that conditioned on 
$\LF$, $\Omega$ is independent of $\beps = [\varepsilon_{ndt}: n \in [N], d \in \bD, t \in [T]]$. 
This is akin to the {\em selection on confounder (or covariates)} condition in the literature on causal inference. 
%
{\color{orange} Can we generalize to selection on latent factors + observed covariates?}


%%
% Summary of Problem Statement
\medskip
\noindent{\em The Problem. Causal Tensor Estimation.} Given the generative model described, the goal
of estimating $\bA$ (respectively $\bV$) becomes the problem of estimating entries of a three-order tensor
from its partial, noisy observation. That is, it is the problem of {\em tensor estimation}. The
underlying tensor of interest is {\em low-rank} if $R$ (respective $R'$) are small or constant 
(do not scale {\color{orange}(scale slowly)} with units, index or number of interventions). The locations of the entries of
the tensor that are observed, $\Omega$, is {\em confounded} with the values of the entries of the 
tensor $\bA$ (respectively $\bV$) we want to estimate. Indeed, this {\em confounding} is of specific
form (i.e. through latent factors $\LF$). Due to such confounding in observation, we call such
a tensor estimation problem as {\em Causal Tensor Estimation}. 

The goal is to understand the {\em observational patterns} $\Omega$ that allow for solving 
such an estimation problem. Indeed, when entries are observed at random (i.e. no or very limited 
confounding) as in the recent literature, there has been reasonable progress made. However, 
with generic confounding as considered in this work, not much is known. 


%%
% Role of covariates
\medskip
\noindent{\em The Role of Covariates.} We remark on the role of {\em observed} covariates for 
{\em Causal Tensor Estimation}. In particular, the tensors of interest, $\bA$ and $\bV$, are
entirely determined through latent factors. Therefore, observed covariates can be useful if they  
can provide information about latent factors. To that end, we discuss a natural structural 
relationship next. 

For the tensor $\bA$ corresponding to the average of potential outcomes, let the factor associated with 
unit $n \in [N]$, $\bu_n$, be such that $\bu_n = [\bul_n : \buo_n]$ with $\bul_n \in \Rb^{\Ro}, \buo_n \in \Rb^{R-\Ro}$ 
and $\buo_n = f(\balpha_n)$ for some $f : \Rb^{q_1} \to \Rb^{R-\Ro}$. 
%
That is, part of factor $\bu_n$, $\buo_n$, is explained by covariates $\balpha_n$ while remainder, $\bul_n$ is {\em latent}. 
%
Similarly, let the factor associated with time $t \in [T]$, $\bv_t$, be such that 
$\bv_t = [\bvl_t : \bvo_t]$ with $\bvl_t \in \Rb^{\Ro}, \bvo_t \in \Rb^{R-\Ro}$ and 
$\bvo_t = g(\bbeta_t)$ for some $t : \Rb^{q_1} \to \Rb^{R-\Ro}$; 
%
and the factor associated with intervention $d \in [D]$, $\bw_d$, be such that
$\bw_d = [\bwl_d : \bwo_d]$ with $\bwl_d \in \Rb^{\Ro}, \bwo_d \in \Rb^{R-\Ro}$ and 
$\bwo_d = h(\bgamma_d)$ for some $d : \Rb^{q_1} \to \Rb^{R-\Ro}$.

Similarly, for the tensor $\bV$ corresponding to the variance of potential outcomes, 
let the factor associated with unit $n \in [N]$, $\bup_n$, be such that
$\bup_n = [\bupl_n : \bupo_n]$ with $\bupl_n \in \Rb^{\Rop}, \bupo_n \in \Rb^{\Rp-\Rop}$ and 
$\bupo_n = \fp(\balpha_n)$ for some $\fp : \Rb^{q_1} \to \Rb^{\Rp-\Rop}$; 
let the factor associated with time $t \in [T]$, $\bvp_t$, be such that
$\bvp_t = [\bvpl_t : \bvpo_t]$ with $\bvpl_t \in \Rb^{\Rop}, \bvpo_t \in \Rb^{\Rp-\Rop}$ and 
$\bvpo_t = \gp(\bbeta_t)$ for some $t : \Rb^{q_1} \to \Rb^{\Rp-\Rop}$; and
the factor associated with intervention $d \in [D]$, $\bwp_d$, be such that
$\bwp_d = [\bwpl_d : \bwpo_d]$ with $\bwpl_d \in \Rb^{\Rop}, \bwo_d \in \Rb^{\Rp-\Rop}$ and 
$\bwpo_d = \hp(\bgamma_d)$ for some $d : \Rb^{q_1} \to \Rb^{\Rp-\Rop}$.
%%

{\color{orange} Can we bypass regressing observed covariates on estimated latent factors, by regressing on estimated potential outcomes?}

{\color{orange} To-do: define target causal parameter for out-of-sample covariate - show how it connects with CATE.}




% \newpage 

% For simplicity, let $\bD$ be a finite set $\bD = [D] \equiv \{1,\dots, D\}$. 
% Let $A_{ntd} \in \Rb$ denote the true or potential outcome of interest associated with unit $n \in [N]$, time or trial $t \in [T]$ and intervention $d \in \bD = [D]$. 
% Under the potential outcome framework, the observation or outcome associated with unit $n$, time or trial $t$ and intervention $d$ is given by 
% \begin{align}\label{eq:potential}
%     Y_{ntd} & = A_{ntd} + \varepsilon_{ntd}, 
% \end{align}
% where $A_{ntd} \in \Rb$ is the (deterministic) mean of random variable $Y_{ntd}$ and 
% $\varepsilon_{ntd}$ (of mean $0$) captures the idiosyncratic random variation in $Y_{ntd}$.  


% %
% \medskip
% {\bf Observations.} For each unit $n \in [N]$ and for each repeat or time $t \in [T]$, it is subjected to a subset
% of interventions $I(n, t) \subset \bD$. Equivalently, let $\Omega \subset [N]  \times [T]\times [D] $
% be set of all indices corresponding to which observation of potential outcomes are available. Formally, 
% the observation tensor $\bZ = [Z_{ntd}] \in (\Rb \cup \{\star\})^{N \times T \times D}$ is such that
% \begin{align}
%     Z_{ntd} & = \begin{cases}
%                     Y_{ntd} & \mbox{~if~} (n,t,d) \in \Omega, \\
%                     \star & \mbox{otherwise,}
%     \end{cases}
% \end{align} 
% where $\star$ denotes `missing' observation. 


% \medskip
% {\bf Causal Tensor Factor Model.} We discuss the causal mechanism modeling the joint distribution of the random variables, tensor 
% $\bY = [Y_{ntd}]$ and observation subset $\Omega \subset [N] \times [T]\times [D]$. We introduce confounders that influences 
% the potential outcomes and observations collectively. 
% %

% %
% \medskip
% \noindent
% {\em Tensor Factor Model for $\bY$.}
% %
% To that end, we introduce {\em factors} associated with units, repeats or time steps, and interventions. Specifically, we start
% by introducing a factor model for mean tensor $\bA$ and component-wise variance tensor $\bV$. 
% Now $\bA$ is a $3$-order tensor and hence it has a finite CP-rank with decomposition (which may not be unique) of the form:
% \begin{align}
%     A_{ntd} & = \sum_{r=1}^R u_{nr} v_{tr} w_{dr},
% \end{align}
% where $\bu_n = [u_{nr}] \in \Rb^R$, $\bv_t = [v_{tr}] \in \Rb^R$,
% and $\bw_d = [w_{dr}] \in \Rb^R$ are {\em factors} associated with unit $n$, repeat or time $t$
% and intervention $d$. In general, $R \geq 1$ is at most $N \times T \times D$. The key
% {\em operating} assumption arises in assuming $R$ to be much smaller than $N, T$, effectively 
% constant. 

% \medskip
% \noindent
% {\em Factors Are Confounders.} 
% %
% We shall assume that the confounder is simply  
% $\LF = (\bu_n, \bup_n, \bv_t,\bvp_t, \bw_d, \bwp_d: n \in [N], t \in [T], d \in [D])$. This subsumes the 
% setting where the underlying confounder is realized once per (unit, time, intervention) 
% tuple, is finite dimensional, and has `low CP-rank' structure like the observational tensor. 

% \medskip
% \noindent
% {\em Mechanism for Observations $\Omega$.} 
% %
% The causal mechanism that leads to observation is as follows. The random subset corresponding to the 
% observation pattern $\Omega$ is determined by confounder $\LF$. The observation tensor $\bZ$ is determined 
% by tensor $\bY$ and $\Omega$. Recall that tensor $\bY = \bA + \beps$. Here, $\bA$ is determined by $\LF$. 
% The idiosyncratic noise $\beps = [\varepsilon_{ntd}]$ is such that $\Ex[\beps | \LF] = [0]$ and $\beps$
% is conditionally independent of $\Omega$ conditioned on $\LF$. 
% %
% We further assume that conditioned on $\LF$, $\varepsilon_{ntd}$ has sub-Gaussian distribution.

% Similarly, the component-wise variance $\bV = [V_{ntd}]$ can be represented as 
% \begin{align}
%     V_{ntd} & = \sum_{r=1}^{\Rp} \up_{nr} \vp_{tr} \wp_{dr},
% \end{align}
% where $\bup_n = [\up_{nr}] \in \Rb^{\Rp}$, $\bvp_t = [\vp_{tr}] \in \Rb^{\Rp}$,
% and $\bwp_d = [\wp_{dr}] \in \Rb^{\Rp}$ are {\em factors} associated with unit $n$, time $t$
% and intervention $d$.



% \medskip
% \noindent
% {\em Factors, Some Latent, Some Observed.} In general, in the absence of any other information, we shall 
% assume factors, $\LF$, associated with unit, time and interventions as being {\em latent}. In general, 
% however, aspects of these factors may be observed. 

% To this end, let $\balpha_n \in \Rb^{q_1}$ be observed covariates associated with unit $n \in [N]$ 
% with $q_1 \geq 1$, $\bbeta_t \in \Rb^{q_2}$ be observed covariates associated with repeat or time $t \in [T]$ 
% with $q_2 \geq 1$, and $\bgamma_d \in \Rb^{q_3}$ be observed covariates associated with intervention 
% $d \in [D]$ with $q_3 \geq 1$. 

% For the tensor $\bA$ corresponding to the average of potential outcomes, let the factor associated with 
% unit $n \in [N]$, $\bu_n$, be such that $\bu_n = [\bul_n : \buo_n]$ with $\bul_n \in \Rb^{\Ro}, \buo_n \in \Rb^{R-\Ro}$ 
% and $\buo_n = f(\balpha_n)$ for some $f : \Rb^{q_1} \to \Rb^{R-\Ro}$. 
% %
% That is, part of factor $\bu_n$, $\buo_n$, is explained by covariates $\balpha_n$ while remainder, $\bul_n$ is {\em latent}. 
% %
% Similarly, let the factor associated with time $t \in [T]$, $\bv_t$, be such that 
% $\bv_t = [\bvl_t : \bvo_t]$ with $\bvl_t \in \Rb^{\Ro}, \bvo_t \in \Rb^{R-\Ro}$ and 
% $\bvo_t = g(\bbeta_t)$ for some $t : \Rb^{q_1} \to \Rb^{R-\Ro}$; 
% %
% and the factor associated with intervention $d \in [D]$, $\bw_d$, be such that
% $\bw_d = [\bwl_d : \bwo_d]$ with $\bwl_d \in \Rb^{\Ro}, \bwo_d \in \Rb^{R-\Ro}$ and 
% $\bwo_d = h(\bgamma_d)$ for some $d : \Rb^{q_1} \to \Rb^{R-\Ro}$.

% Similarly, for the tensor $\bV$ corresponding to the variance of potential outcomes, 
% let the factor associated with unit $n \in [N]$, $\bup_n$, be such that
% $\bup_n = [\bupl_n : \bupo_n]$ with $\bupl_n \in \Rb^{\Rop}, \bupo_n \in \Rb^{\Rp-\Rop}$ and 
% $\bupo_n = \fp(\balpha_n)$ for some $\fp : \Rb^{q_1} \to \Rb^{\Rp-\Rop}$; 
% let the factor associated with time $t \in [T]$, $\bvp_t$, be such that
% $\bvp_t = [\bvpl_t : \bvpo_t]$ with $\bvpl_t \in \Rb^{\Rop}, \bvpo_t \in \Rb^{\Rp-\Rop}$ and 
% $\bvpo_t = \gp(\bbeta_t)$ for some $t : \Rb^{q_1} \to \Rb^{\Rp-\Rop}$; and
% the factor associated with intervention $d \in [D]$, $\bwp_d$, be such that
% $\bwp_d = [\bwpl_d : \bwpo_d]$ with $\bwpl_d \in \Rb^{\Rop}, \bwo_d \in \Rb^{\Rp-\Rop}$ and 
% $\bwpo_d = \hp(\bgamma_d)$ for some $d : \Rb^{q_1} \to \Rb^{\Rp-\Rop}$.


% \medskip
% {\bf Quantity of Interest.} The fundamental question of causal inference is ability to estimate the distribution of each element of the tensor $\bY = [Y_{ntd}]$. 
% Now estimating entire distribution can be extremely challenging, if not impossible, in most settings. Given that, a simpler objectives may be estimating functionals 
% of the distribution. Formally, consider any measurable function $f: \Rb \to \Rb$. Then a quantity of interest is $\Ex[f(\bY)] = [\Ex[f(Y_{ntd})]]$. 
% %
% For example, $f(x) = x$ corresponds to estimating means:
% \begin{align} 
% \Ex[f(\bY)] & = [\Ex[f(Y_{ntd})]] = [f(A_{ntd} + \varepsilon_{ntd}) ] ~=~ [A_{ntd} + \Ex[\varepsilon_{ntd}] ] = \bA.
% \end{align}
% %
% Similarly, $f(x) = x^2$, corresponds to estimating second moment:
% \begin{align}
%     \Ex[f(\bY)] & = [\Ex[Y_{ntd}^2]] = [A_{ntd}^2 + \Ex[\varepsilon_{ntd}^2]] \nonumber \\
%     & = f(\bA) + [\Ex[\varepsilon_{ntd}^2]].
% \end{align}
% We shall denote componentwise variance, $\bV = [V_{ntd}]$ where $V_{ntd} = \Ex[\varepsilon_{ntd}^2]$.



% \medskip
% {\bf The Goal.} The {\em ideal} goal is to estimate the distribution of each component of the potential
% outcome tensor $\bY$. This may not be feasible in generality. However, in a restricted sense, it may be.
% Precisely, a {\em pragmatic} or {\em feasible} goal is to estimate tensors $\bA$ and $\bV$ 
% from observed tensor $\bZ$ which obey above causal structure. Indeed, the ability to estimate 
% $\bA$ and $\bV$ must depend on the `observation patterns' or data availability, i.e. 
% $I(n, t), n \in [N], t \in [T]$. 

==> Old/archived/causal_tensor_estimation.tex <==
\section{Causal Tensor Estimation}

\subsection{The question}

The key question boils down to estimating the tensors $\bA, \bV \in \Rb^{N \times T \times D}$ (with $M = 1$)
from observation tensor $\bZ \in (\Rb \cup \{\star\})^{N \times T \times D} $ subject to the 
setup of Section \ref{sec:framework}. 

In particular, the tensor of interest is {\em low-rank} (with respect to CP-rank) with observed data 
generated {\em causally} rather than at random. That is, the key question is that of {\em causal tensor 
estimation} to estimate the causal quantity of interest across various scenarios. 

Let $\hbA = \hbA(\bZ)$ and $\hbV = \hbV(\bZ)$ be estimated tensors from $\bZ$. Then, an estimation
errors of interest is
\begin{align}
    \error(\hbA) & = \max_{n, t, d} |\hA_{ntd} - A_{ntd}|, \nonumber \\
    \error(\hbV) & = \max_{n, t, d} |\hV_{ntd} - V_{ntd}|.
\end{align}
As a simpler notion, it may make sense to study the ``point-wise'' error $|\hA_{ntd} - A_{ntd}|$ (resp. $|\hV_{ntd} - V_{ntd}|$) 
for a given $n, t, d$. 

\subsection{Identification}

{\color{red} The question of identification is ... what are conditions on observational patterns, etc.}


\subsection{Method}

{\color{red}
Discuss an approach to identify is to find latent factors or similarities between factors}
\\

{\color{red}
Discuss nearest neighbors or remove?}
\\ \\

We present a method for causal tensor estimation. The method is a natural adaptation of the Synthetic Interventions (SI). 
The method of SI is directly applicable for estimating $\bA$. We discuss the modification of it for estimating $\bV$ 
through a two-step application of SI (to $\bZ$ and $\bZ^2$). We discuss the conditions under which the estimated tensors, $\hbA, \hbV$ are such that $\error(\hbA), \error(\hbV)$ go to $0$. 



\subsection{Implications}

We discuss the implication of the method described above to various scenarios here. Specifically, we discuss implications for
the comparative setup of regression discontinuity, temporal structure, unseen interventions and experiment design. 

\subsection{Causal structure discovery} 

The factors learnt associated with the tensors $\bA, \bV$ provide sufficient representation for the mean, variance of potential
outcomes. However, they do not necessarily provide insights into the causal structure or mechanism behind it. To that end, let
$\balpha_n$ be observed covariates associated with unit $n \in [N]$. Let $\bu_n$ be factor learnt. Then identifying a function
$f$ such that $f(\balpha_n) \approx \bu_n$ for all $n \in [N]$ may provide insights into the causal relationship between the
covariates of the unit and potential outcomes of interest. 



==> Old/archived/covariates.tex <==
{\color{blue}
\section{Role of Covariates}

%
{\bf Use Case 1.}
%

Suppose we estimate $\textsf{ATE}_{t}$ for all $t$. 
%
Further suppose we have access to covariates $X_t$ for all $t$.
%
Assume $$\textsf{ATE}_{t} = g(X_t) + \nu_t.$$
%
Then for an unseen measurement $t^* \notin [T]$, we could estimate $\textsf{ATE}_{t^*}$ as follows:
%
\begin{enumerate}
%
\item For $t \in [T]$, estimate $\hat{\textsf{ATE}}_{t}$ using the estimator in \eqref{eq:ATE_synthetic_estiamtor}.
%
\item Estimate $$\hat{g} = \min_{g \in \Gc} \sum_{t \in [T]} \ell\left(g(X_t), \hat{\textsf{ATE}}_{t}\right).$$
%
\item Predict $$\hat{\textsf{ATE}}_{t^*} = \hat{g}(X_{t^*})$$
%
\end{enumerate}


{\bf Use Case 2.}
%

Extend the model in \eqref{eq:treatment_assignment} and \eqref{eq:observed_outcomes} as follows:
%
\begin{align}
%
A_{n, t} &= h(n, t, \textsf{U}, \textsf{X}, \nu), 
%
\\ Y_{n, t} &= f(n, t, A_{n, t}, \textsf{U}, \textsf{X}, \varepsilon),
%
\end{align}
%
where $\textsf{X} = \{X_{n, t, a}\}_{n \in [N], t \in [T], a \in \Ac}$ are observed covariates associated with the various units, measurements, and interventions.
%
Hence, now we have 
%
\begin{align}
Y^{(a)}_{n, t} &\indep \Omega ~|~ \textsf{U}, \textsf{X}
\end{align}

OR

\begin{align}
%
A_{n, t} &= h(n, t, \textsf{X}, \nu), 
%
\\ Y_{n, t} &= f(n, t, A_{n, t}, \textsf{X}, \varepsilon).
%
\end{align}
%
That is, $\textsf{U} = \textsf{X}$ and we have 
\begin{align}
Y^{(a)}_{n, t} &\indep \Omega ~|~ \textsf{X}
\end{align}

{\color{red}
How does this what we are doing compare with selection on observables, $X$, where $Y^{(a)} \indep \Omega \mid X$, and we have
\begin{align}
%
\Ex[Y^{(1)} - Y^{(0)}] &= \Ex[\Ex[Y^{(1)} \mid X]] - \Ex[\Ex[Y^{(0)} \mid X]]
%
\\ &= \Ex[\Ex[Y^{(1)} \mid A = 1, X]] - \Ex[\Ex[Y^{(0)} \mid A = 0, X]]
%
\\ &= \Ex[\Ex[Y \mid A = 1, X]] - \Ex[\Ex[Y \mid A = 0, X]]
%
\end{align}
%

I think we are estimating something analogous to $\Ex[Y^{(1)} \mid X]$, without the outer expectation.


Also, is it the case that 
\begin{align}
%
\frac{1}{|\Ic^{(a)}_{t}|}\sum_{n \in\Ic^{(a)}_{t}} Y_{n, t} \mid \Omega, \textsf{U} \xrightarrow[]{d} \frac{1}{N}\sum^N_{n = 1} Y^{(a)}_{n, t} \mid \textsf{U}.
%
\end{align}
since we have that $Y^{(a)}_{n, t} \indep \Omega \mid \textsf{U}$? Don't think so, but just want to understand.

A good, focused motivation for this paper could be: 

\centering{\em ``Comparing selection on observables versus selection on latent factors.''}
}
}

==> Old/archived/notes.tex <==
\newpage
{\color{blue}
TO-DO: \textcolor{teal}{New in teal color.}
\begin{itemize}
\item \textcolor{teal}{Average of estimates or estimate of average}
\item \textcolor{teal}{Sampling}
\item \textcolor{teal}{Rates for Nonparametric regression with unobserved factors}
\item \textcolor{teal}{An idea for the empirical part: Take the Nielsen data. Split at random, perhaps 25/75 percent. Call the first group treated and the second untreated. Check that difference in outcomes is zero. De-randomize by dropping control observations with probability of dropping based on aggregates of outcomes for periods that we will not use for estimation. Check that difference in mean outcomes in not zero. Check that controlling for low-dimensional covariates does not make the difference disappear. Check that (hopefully) our method makes the difference disappear. Perhaps, after validation, we could also apply the method to estimate the effect of discounts (although discounts are clustered, so that may require additional derivations.)}
\item {About the structure of the paper and the set of assumption we adopt. I think we can proceed as in my paper with Imbens, Wooldridge, and Athey ({\it Econometrica}, 2020), where we first explain the conceptual framework and results in a simple context (diff in means) and in the next section we go for the general case.}
\item {Anish and Alberto Seattle breakfast discussion. Exploit factor structure in assignment equation. Stack matrix of $A_{n,t}$ with potential outcome matrices into a tensor?}
\begin{itemize}
    \item Could be a way of verifying if there is confounding
\end{itemize}
\item Different intervention assignments

\begin{itemize}
    \item If there is factorization in intervention assignment (e.g. reg discontinuity)
    \item Staggered adoption \& pilot studies
\end{itemize}

\item Dynamic treatment regimes: $A_{nt}=h_t(A_{nt-1}, A_{nt-2} …, Y_{nt-1}, Y_{nt-2}, …., U_n,\mu_{nt})$. I.e., G-estimation with a factor model for unobserved. 
\item Old idea about double robustness in factor models for treatment and outcomes
%
\item Incorporating covariates
    \begin{itemize}
    %
    \item Investigate potential role of alternating regression (known properties?)
    \item Reducing sample complexity
    %
    \item Generalizing to unseen units, interventions
    %
    \item Connection to selection on observables
    \end{itemize}

%
\item Empirical example (let's start talking about potential data sets)
%
%
    \begin{itemize}
    %
    \item {Devavrat idea about validation with the NFL data made me think about the LaLonde ({\it AER}, 1986) study. This is a classic in econ. There, Robert LaLonde took data from an experiment, estimated ATE=ATET with the experimental data, and then discarded the non-treated obsevations from the experiment, instead using non-treated observational data and econometric techniques to try to reproduce the experimental results. It would be neat if we could do the same with modern data and online experiments.}
    \item Scanner data (Nielsen)
    \item Selection on observables (hide observables)
    \item NFL re-opening
    \item Price vs. Demand
    \item Stock prices
    \item Event studies
    \item Acemoglu paper (connections)
    \end{itemize}
%
\item Navigating the document: Put everything in one tex file and eliminate percent symbols. Eliminate or severely limit user-defined commands for notation. Also eliminate table of contents.
\item very explicitly explain restrictions to the assignment mechanism 
\end{itemize}
}

==> Old/archived/old_introduction.tex <==
\section{Old}

{\bf Representing potential outcomes as matrix/tensor.}
%
Given our goal of connecting causal inference with tensor estimation, we show first show, without loss of generality, how to represent the various potential outcomes of interest through a matrix/tensor.
%
Suppose $\Uc$ and $\Ac$ are finite, i.e., $|\Uc| = U$, $| \Ac| = A$, where $U, A < \infty$.
%
Then we can represent the various potential outcomes through the following matrix, $\bM = [M_{ua}]_{u \in \Uc, a \in \Ac} \in \Rb^{U \times A}$, where:
%
\begin{align}
    M_{ua} = Y^{(a)}_u.
\end{align}
%
Now suppose there is additional structure in $\Uc$ and $\Ac$ such that they further factorize. 
%
For example $\Uc = \Uc_1 \times \Uc_2$ where say $\Uc_1, \Uc_2$ represent factors about different individuals and time periods, respectively, as is common in panel data.
%
Similarly, $\Ac = \Ac_1 \times \Ac_2$ where say $\Ac_1, \Ac_2$ represent dosage levels of two different drugs.
%
Then the various potential outcomes can be written as %
\begin{align}
    Y^{(a_1, a_2)}_{u_1, u_2} \coloneqq f(\bU_1 = u_1, \bU_2 = u_2, \bA_1 = a_1, \bA_2 = a_2).
\end{align}
%
Now the $Y^{(a_1, a_2)}_{u_1, u_2}$ can be represented as an order-four tensor $\bT = [T_{u_1, u_2, a_1, a_2}]_{u_1 \in \Uc_1, u_2 \in \Uc_2, a_1 \in \Ac_1, a_2 \in \Ac_2} \in \Rb^{U_1 \times U_2 \times A_1 \times A_2}$, where
%
\begin{align}
    T_{u_1, u_2, a_1, a_2} = Y^{(a_1, a_2)}_{u_1, u_2}.
\end{align}
%
So we see that at least in the case where $\Uc$ and $\Ac$ are finite, we can represent the various potential outcomes as a tensor, where the order of the tensor depends on the amount of additional factorization in $\Uc$ and $\Ac$---note that a matrix is an order-2 tensor.
%
For the majority of the article, we will focus on the setting of order-three tensors.
%
That is, potential outcomes of the form $Y^{(a)}_{u_1, u_2}$.
%
However, our analysis generalizes to arbitrary order tensors.
%
In fact in {\color{blue} Section \ref{sec:continous_actions_confounders}}, we will generalize our results to the setting where $\Uc$ and/or $\Ac$ are not finite.

{\bf Linear factor models: a ``universal'' representation.}
%
Recall from \eqref{eq:PO_1} that the potential outcomes are given by the function $f(\cdot)$ which takes as input the confounders and actions.
%
We argue that if $f(\cdot)$ is sufficiently ``smooth'' in either of $\Uc$ or $\Ac$, there exists a ``universal'' representation of $f(\cdot)$ as a (approximate) low dimensional linear factor model.
%
There are different notions of smoothness that lead to different approximation error results. 
%
We detail them below.

{\em H\"older smooth functions.}
%
We first focus on the matrix setting and without loss of generality, we assume that $f(\cdot)$ is smooth in its first argument, $\Uc$.
%
Below we define H\"older smooth functions.
%
\begin{definition}[H\"older class]
The H\"older class $\Hc(q,S,C_H)$ on $[0, 1)^q$ is the set of functions $h: [0, 1)^q \to \mathbb{R}$ whose partial derivatives satisfy
%
$$
\sum_{s: |s| = \lfloor S \rfloor} \frac{1}{s!} |\nabla_s h(\mu) - \nabla_s h(\mu') | \le C_H \norm{\mu - \mu'}_{\max}^{S - \lfloor S \rfloor},\quad \forall \mu, \mu' \in [0, 1)^q,
$$
where $\lfloor S \rfloor$ denotes the largest integer strictly smaller than $S$.
%
% Note as a special case where $S = 1$ leads to Lipschitz continuous functions with parameter $C_H$.
\end{definition}

\begin{assumption}[Generalized factor model]
%
Assume there exists $\tilde{f}(\lambda_u,\mu_a)$ where $\lambda_u, \mu_a \in [0,1)^{q}$ such that $\tilde{f}(\lambda_u,\mu_a) = f(u, a)$
and $g(\cdot, \mu_a)\in\Hc(q,S,C_H)$ for all $u \in \Uc$, $a \in \Ac$.
%
\end{assumption}
%
A linear factor model is a special case of a generalized factor model where $\tilde{f}(\lambda_i,\mu_j) = \lambda_i ^T \mu_j$. Such a model satisfies Definition \ref{def:holder} for all $S \in \mathbb{N}$ and $C_H = C$, for some absolute positive constant $C<\infty$. 
%
\begin{proposition}[H\"older low rank matrix approximation \cite{agarwal2021robustness}]
%
Suppose Assumption~\ref{assumption:factor_model} holds for some fixed $\mathcal{H}(q,S,C_H)$.
%
Let $\bM = [f(u, a)]_{u \in \Uc, a \in \Ac}$.
%
Then for any  $\delta>0$, there exists $\bM^{(lr)}$ such that
%
\begin{align*}
%
r = \text{rank}(\bM^{(lr)})\leq C \cdot \delta^{-q},
%
\quad \Delta_E = \|\bM-\bM^{(lr)}\|_{\max} \leq C_H \cdot \delta^S
%
\end{align*}
where $C$ is allowed to depend on $(q,S)$.
%
\end{proposition}
%
Proposition \ref{prop:factor_model_approx} establishes that if $f(\cdot)$ has a smooth generalized factor model representation, it implies joint control over $(r,\Delta_E)$ as desired.
%
Intuitively, as latent dimension $q$ increases, the rank $r$ increases. 
%
As smoothness $S$ increases, the approximation error $\Delta_E$ decreases. 
%
Given $\text{rank}(\bM^{(lr)}) = r \le  C \cdot \delta^{-q}$, there exists $[\bar{\lambda}_u]_{u \in \Uc}, [\bar{\mu}_a]_{j \in \Ac}$ with $\bar{\lambda}_u, \bar{\mu}_a \in \Rb^{r}$ such that
%
\begin{align}
    \bM^{(lr)}_{ua} = \sum^r_{\ell = 1} \bar{\lambda}_{u \ell} \bar{\mu}_{a \ell}
\end{align}
%
Hence, Assumption \ref{assumption:factor_model} and Proposition \ref{prop:factor_model_approx} together imply that for all $u \in \Uc$ and $a \in \Ac$,
%
\begin{align}
    \left| f(u, a) - \sum^{C \delta^{-q}}_{\ell = 1} \bar{\lambda}_{u \ell} \bar{\mu}_{a \ell} \right| \ \le \ C_H \delta^S.
\end{align}
%
That is, if $f(\cdot)$ has a H\"older smooth representation, that it is point-wise, well-approximated by a linear factor model of appropriate dimension.

{\em Lipschitz smooth functions.}

% \begin{definition}[Lipshitz  class]\label{definition:lipshitz_}
% %
% The Lipschitz class $\Lc(q_1, q_2, q_3, C_L)$ is the set of functions $h : [0, 1)^{q_1} \times [0, 1)^{q_2} \times [0, 1)^{q_3} \to \Rb$ such that for any $\theta_n, \theta_{n'} \in [0,1]^{d_1}, \rho_s,\rho_{s'} \in [0,1]^{d_2}, \omega_a, \omega_{a'} \in [0,1]^{d_3}$,
% %
% \begin{align}
%     h(\theta_{n'}, \rho_{s'}, \omega_{a'}) - h(\theta_n, \rho_s, \omega_a) | \le L \left(\| \theta_{n'} - \theta_n \|_2 + \|\rho_{s'} - \rho_s \|_2 + \| \omega_{a'} - \omega_a \|_2\right).
% \end{align}
% %%
% \end{definition}

% \begin{assumption}[Generalized factor model]\label{assumption:factor_model}
% %
% Assume there exists $\tilde{f}(\lambda_u,\mu_a)$ where $\lambda_u, \mu_a \in [0,1)^{q}$ such that $\tilde{f}(\lambda_u,\mu_a) = f(u, a)$
% and $g(\cdot, \mu_a)\in\Hc(q,S,C_H)$ for all $u \in \Uc$, $a \in \Ac$.
% %
% \end{assumption}

% \begin{proposition}[H\"older low rank matrix approximation \cite{agarwal2021persim}]\label{prop:factor_model_lipschitz_approx}
% %
% Suppose Assumption~\ref{assumption:factor_model} holds for some fixed $\mathcal{H}(q,S,C_H)$.
% %
% Let $\bM = [f(u, a)]_{u \in \Uc, a \in \Ac}$.
% %
% Then for any  $\delta>0$, there exists $\bM^{(lr)}$ such that
% %
% \begin{align*}
% %
% r = \text{rank}(\bM^{(lr)})\leq C \cdot \delta^{-q},
% %
% \quad \Delta_E = \|\bM-\bM^{(lr)}\|_{\max} \leq C_H \cdot \delta^S
% %
% \end{align*}
% where $C$ is allowed to depend on $(q,S)$.
% %
% \end{proposition}

{\em Sobolev smooth functions.}

{\em Analytic functions.}

{\em Reproducing kernel hilbert space (RKHS).}


{\color{orange} 
%
A lot of these arguments imply something stronger than just a bound on the rank $r$.
%
In particular, there are only $r$ ``types of rows''.
%
Hence, for any given row, there exists other rows that are approximately identical to it. 
%
This motivates nearest neighbor (i.e., ``exact matching'' style estimators) along with synthetic controls type estimators.
%
}

==> Old/archived/outline.tex <==
\section*{Outline}

{\color{orange}
%
\begin{enumerate}
%
\item Core issue of causal inference: unobserved confounding. 
%
\item Diabetes example + Dag. $\bY, \bA, \bU$
%
\item Many existing approaches: RCT, IV, Proxies
%
\item Rather than introduce new variables to the DAG that are in essence a source of exogenous variation, we show that in a setting with multiple natural experiments, i.e., many units, and many measurements per unit, $\bU$ naturally admits a latent factorization
%
\item $Y^{(a)}_u$ where $a \in [\Ac]$ and $u \in [N] \times [T]$. $N$ units and $T$ measurements.
%
\item $Y^{(a)}_u = f(U = u, A = a)$. Now assume $f$ satisfies the following two assumptions: (i) Latent Variable Model (LVM): $f(U = u, A = a) = \tilde{f}(\theta_u, \rho_a)$ where $\theta_u, \rho_a \in \Rb^r$; (ii) LVM is ``smooth'', i.e., $\tilde{f}$ is Holder continuous. Interpret conditions (i) and (ii).
%
\item If conditions (i) and (ii) above are satisfied, then LVM is arbitrarily well-approximated by a linear factor model as $N$ and $U$ grow.
%
\item ATE motivating example
%
\end{enumerate}
%
}

==> Old/content/abstract.tex <==
% \noindent 
% %
% We present a framework of causal tensor estimation where the goal is to estimate treatment effects as functionals of a three-order tensor representation of potential outcomes from partial/noisy observations and when the set of entries that are observed depend on potentially unobserved confounders. This framework captures various prior works including framework of synthetic controls (SC), synthetic differences in differences (SDID) and synthetic interventions (SI) as a special instances, and enables novel settings including a variation of the classical setup of regression discontinuity. We establish identification of causal estimands of interest in terms of the {\em observation pattern} of the underlying tensor. Finally, we discuss the task of estimating the causal estimands. {\color{red} Causal tensor estimation: ``blessing of dimensionality"}

{\color{blue}
{\bf To-do before the conference: (the first two are the most important)}
\begin{itemize}
\item How is this different from the previous literature (including JoE paper)?
\item Understand issue with bias. Do we have a bias term that we have to take care of, like in the related literature? If yes, how will we do that? If no, why?
\item For the slides, focus on ATT. 
\item Can we dispose of the condition that we do not like for consistency and asymptotic normality with PCR?
\item Simulation/application.
\item Check proofs.
\item We need slides. 
\end{itemize}

{\bf To-Do for this paper}
\begin{itemize}
    \item Add in Empirics - Simulations, Nielsen, Glance
    \item Literature review - non-linear factor models + non-linear models with fixed effects
    \item Fix slant of symbols in assumption/theorem
    \item Exploiting structure in both outcomes and assignments
\end{itemize}

\vspace{2mm}
{\bf Future papers(?)}
\begin{itemize}
\item Continuous interventions
     \begin{itemize}
     \item Covariates about unit/measurements/actions
     \begin{itemize}
            \item selection on observables vs. projection on observables
        \end{itemize}   
    \end{itemize}
\item Doubly robust matrix completion 
    \begin{itemize}
        \item Matrix of treatment assignments AND/OR potential outcomes has factor structure
    \end{itemize}
\item Dynamic Treatment Assignment
\item Nonparametric regression with a latent factor model
\end{itemize}
}




==> Old/content/assignment_factor_structure.tex <==
\section{Identification and Estimation of Treatment Effects \\ with Factor Structure in Potential Outcomes and Intervention Assignment}\label{sec:assignment_factor_structure}

==> Old/content/conclusion.tex <==
\section{Conclusion}
%
We provide a framework for modern causal inference when there are high-dimensional measurements collected per unit under a variety of interventions, which is becoming ubiquitous in modern datasets.
%
We establish that despite unobserved confounding if there is a latent low-dimensional representation of the confounders, and the various potential outcomes are a smooth non-linear function of the confounders and interventions, then the potential outcomes are well-approximated by a {\em linear} factor model as long as there are a sufficiently large number of units and measurements.
%
Under this model, we establish an identification result for ATE for a given measurement and intervention.
%
Subsequently, we propose a novel estimator for ATE and establish its finite-sample consistency.





==> Old/content/introduction.tex <==
\section{Introduction}

One of the central goals of empirical research in economics is to ascertain the effects of treatments (policies, interventions) on the outcomes of interest. A fundamental challenge for the estimation of treatment effects is the pervasive presence of unobserved confounders. For example, in a study of the effects of health insurance on healthcare utilization, unobserved or latent health determinants may differ between insured and uninsured individuals, biasing treatment effect estimates. Several approaches have been put forward to estimate treatment effects in the presence of confounders, including explicit randomization of the treatment, controlling for measured confounders, and instrumental variable methods. Traditionally, these methods are not designed to operate in data-rich environments where the curse of dimensionality creates challenges for estimation and inference or to take advantage of the information contained in high-dimensional data to identify treatment effects.

In recent times, the availability of high-dimensional data on economic behavior has become commonplace. Modern data harvesting technologies, based on digitization and pervasive sensors, enable the collection of detailed high-frequency attribute and outcome information on individuals (or other observational units; e.g., geo-locations) concurrently undergoing different interventions. For example, electronic health records contain rich information about patients' medical history over time. Similarly, internet retailers and marketing firms using scanner data collect high-dimensional information on customers' purchases. The goal of this article is to provide a framework for causal inference that takes advantage of modern data-rich environments to counter the effect of unobserved or latent confounders.

Given this goal, we consider a setting where we have access to data for $N$ units (e.g., individuals, sub-populations, firms, geographic locations) and $T$ measurements of outcomes per unit. Different measurements may represent the same outcome metric at different time periods, different outcome metrics (e.g., customers' expenditures in different product categories) for the same time period, or a combination of both. We argue that (high-dimensional) data-rich environments---i.e., large $N$ and large $T$---make it possible to estimate treatment effects in the presence of (relatively low-dimensional) unobserved or latent confounding, without parametric assumptions in the manner in which unobserved confounders affect selection for treatment and the outcome metrics.

==> Old/content/model.tex <==
\section{Model}

\subsection{Notation}


For a matrix $\bA \in \Rb^{a \times b}$, we denote its transpose as $\bA^T \in \Rb^{b \times a}$. We denote the operator (spectral) and Frobenius norms of $\bA$ as $\|\bA\|_{\text{op}}$ and $\|\bA\|_F$, respectively. The columnspace (or range) of $\bA$ is the span of its columns, which we denote as  $\Rc(\bA) = \{v \in \Rb^a: v = \bA x, x \in \Rb^b\}$. The rowspace of $\bA$, given by $\Rc(\bA^T)$, is the span of its rows. Recall that the nullspace of $\bA$ is the set of vectors that are mapped to zero under $\bA$. For any vector $v \in \Rb^a$, let $\|v\|_p$ denote its $\ell_p$-norm, and let $\|v\|_\infty$ denote its max-norm. The inner product between vectors $v, x \in \Rb^a$ is $\langle v, x \rangle = \sum_{\ell=1}^a v_\ell x_\ell$. If $v$ is a random variable, we denote its sub-Gaussian (Orlicz) norm as $\|v\|_{\psi_2}$. For any positive integer $a$, we use the notation $[a] = \{1, \dots, a\}$. 

Let $f$ and $g$ be two real-valued functions defined on $\mathcal X$, an unbounded subset of $[0,\infty)$. We say that $f(x)$ = $O(g(x))$ if and only if there exist a positive real number $M$ and $x_0\in \mathcal X$ such that, for all $x \ge x_0$, we have $|f (x)| \le M|g(x)|$. Analogously, we say that $f (x) = \Theta(g(x))$ if and only if there exist positive real numbers $m, M$ and $x_0\in \mathcal X$ such that for all $x \ge x_0$, we have $m|g(x)| \le |f(x)| \le M|g(x)|$; $f (x) = o(g(x))$ if for any $m > 0$, there exists $x_0\in \mathcal X$ such that for all $x \ge x_0$, we have $|f(x)| \le m|g(x)|$. 

We adopt standard notation and definitions for stochastic convergence. We employ $\xrightarrow{d}$ and $\xrightarrow{p}$ to indicate convergence in distribution and probability, respectively. For any sequence of random vectors, $X_n$, and any sequence of positive real numbers, $a_n$, we say $X_n = O_p(a_n)$ if for every $\varepsilon>0$, there exists constants $C_\varepsilon$ and $n_\varepsilon$ such that $\Pb( \| X_n \|_2 > C_\varepsilon a_n) < \varepsilon$ for every $n \ge n_\varepsilon$; equivalently, we say $(1/a_n) X_n$ is uniformly tight or bounded in probability. $X_n = o_p(a_n)$ means $X_n/a_n\xrightarrow{p} 0$. We say a sequence of events $\Ec_n$, indexed by $n$, holds ``with probability approaching one'' (w.p.a.1) if $\Pb(\Ec_n) \rightarrow 1$ as $n \rightarrow \infty$, i.e., for any $\varepsilon > 0$, there exists a $n_\varepsilon$ such that for all $n > n_\varepsilon$, $\Pb(\Ec_n) > 1 - \varepsilon$. More generally, a multi-indexed sequence of events $\Ec_{n_1,\dots, n_d}$, with indices $n_1,\dots, n_d$ with $d \geq 1$, is said to hold w.p.a.1 if $\Pb(\Ec_{n_1,\dots, n_d}) \rightarrow 1$ as $\min\{n_1,\dots, n_d\} \rightarrow \infty$. We also use $\Nc(\mu, \sigma^2)$ to denote a normal or Gaussian distribution with mean $\mu$ and variance $\sigma^2$---we call it {\em standard} normal or Gaussian if $\mu = 0$ and $\sigma^2 = 1$.
We use $C$ to denote a positive constant, with a value that can change across instances. 

%We also introduce the notion of a H\"older continuous function.
\begin{definition}[H\"older continuity, e.g., \citeauthor{jiaming_spectral_convergence}, \citeyear{jiaming_spectral_convergence}]\label{def:holder}
Let $s = (s_1, \dots, s_q)$ be a $q$-tuple of non-negative integers with $|s| = \sum^q_{\ell = 1} s_\ell$. For $S>0$ and $C_H>0$, the H\"older class $\Hc(q,S,C_H)$ on $[0, 1)^q$
is the set of functions $g: [0, 1)^q \to \mathbb{R}$ with partial derivatives that satisfy
\[
\sum_{s: |s| = \lfloor S \rfloor} \frac{1}{s!} |\nabla_{\!s} g(\mu) - \nabla_{\!s} g(\mu') | \le C_H \norm{\mu - \mu'}_{\infty}^{S - \lfloor S \rfloor},\quad \forall \mu, \mu' \in [0, 1)^q,
\]
where $\lfloor S \rfloor$ denotes the largest integer strictly smaller than $S$.
\footnote{We impose $[0,1)^q$ without loss of generality. Note that for any compact set $\Xc \in \Rb^q$, we have $\Xc \subset [-c, c)^q$, where $c \le \infty$. Then, $[-c, c)^q$ can be replaced by $[0, 1)^q$, without loss of generality by re-scaling.}
\end{definition}
\textcolor{blue}{Because we rarely go into Holder continuity with exponent less than one (or we do?), it seems natural to restrict $S$ (at least in our minds) to be a positive integer. Then, the condition means we have $S-1$ Lipschitz-continuous derivatives, with Lipschitz constant equal to $C_H$. Anything important we are excluding with this?}

\subsection{Data Generating Process} 
%
We are interested in evaluating the effect of treatments on outcomes of interest. 
%
Specifically, we observe $T$ outcomes or measurements for $N$ units. 
%
For each measurement $t \in [T]$ and unit $n \in [N]$, we observe $Y_{n, t} \in \Rb$ under intervention $A_{n, t} \in \Ac$. 
%
Let $\bA = [A_{n, t}]_{n \in [N], t \in [T]} \in \Ac^{N \times T}$ and $\bY = [Y_{n, t}]_{n \in [N], t \in [T]} \in \Rb^{N \times T}$ collect the matrix of intervention assignments and outcomes, respectively.
%
We now define how the intervention assignments and outcomes are generated.
%
We define the (random) variable $\bU \in \bar{\mathcal{U}}$ and functions $\bar{h}: \bar{\mathcal{U}} \to \Ac^{N \times T}, \bar{f}: \bar{\mathcal{U}} \times \Ac^{N \times T} \to \Rb^{N \times T}$ such that
%
\begin{align}
%
\bA &= \bar{h}(\bU) \label{eq:basic_DGP_1}
%
\\ \bY &= \bar{f}(\bU, \bA) \label{eq:basic_DGP_2}
%
\end{align}
%
\textcolor{blue}{There should be additional errors here. Variables that affect $\bA$ or $\bY$, but not both. Otherwise, it is not clear where $\varepsilon^{(a)}_{n, t}$ comes from. As we write things now, $\varepsilon^{(a)}_{n, t}$ could only come from variation in $U_j$ for $j \neq n$ and $U_{l,b}$ for $(l,b)\neq (t,a)$ conditional on $U_n,U_{t,a}$.}

\eqref{eq:basic_DGP_1} and \eqref{eq:basic_DGP_2} imply that $\bU$ is a confounder. 
%
That is, it affects both the intervention assignment and the outcomes.
%
We allow $\bU$ to be partially observed, or completely unobserved.
%
Figure \ref{figure:dag} provides a DAG consistent with \eqref{eq:basic_DGP_1} and \eqref{eq:basic_DGP_2}.
%
Let $\bar{h}(\bU; n, t)$ and $\bar{f}(\bU, \bA; n, t)$ refer to the $(n, t)$-th coordinate of $\bar{h}, \bar{f}$, respectively.
%
Thus far the setup is very general. 
%
To make progress, we must impose structure on $\bar{h}$ and $\bar{f}$, which we do in the following section.
%

\begin{figure}[t!]
\begin{center}
\begin{tikzpicture}
\node (A) at (0,0) {$\bA$};
\node (U) at (1,1) {$\bU$};
\node (Y) at (2,0) {$\bY$};
% \node (V) at (-1,1) {$\bN$};
% \node (W) at (3,1) {$\bE$};
\draw[thick, ->] (U) -- (A);
\draw[thick, ->] (U) -- (Y);
\draw[thick, ->] (A) -- (Y);
% \draw[thick, ->] (U) -- (V);
% \draw[thick, ->] (U) -- (W);
% \draw[thick, ->] (V) -- (A);
% \draw[thick, ->] (W) -- (Y);
\end{tikzpicture}\vspace*{-.5cm}
\end{center}
\caption{A DAG representation consistent with the data generating process.}
\label{figure:dag}
\end{figure}

\subsubsection{Latent Factorization of Confounders}
%
The key assumption we make is that the confounder $\bU$ has a latent factorization into unit and (measurement, intervention) specific factors.
%
\begin{assumption}\label{assumption:confounder_structure}
%
We assume $\bU$ factorizes as follows.
%
\begin{align}\label{eq:confounder_structure}
%
\bU = [ (U_n)_{n \in [N]}, (U_{t, a})_{t \in [T], a \in \Ac}],
%
\end{align}
%
where $U_n \in \mathcal{U}, U_{t, a} \in \tilde{\mathcal{U}}$.
\end{assumption}
%
Given this structure that we impose on the confounders, we next impose that the outcome for measurement $(n, t)$ is only a function of the confounders $U_n$ and $U_{t, A_{n, t}}$.
%
\begin{assumption}\label{assumption:outcome_function}
%
There exists a function $f: \mathcal{U} \times \tilde{\mathcal{U}} \to \Rb$, such that the observed outcomes for all $(n, t)$ can be written as
%
\begin{align}\label{eq:observed_outcomes_local}
%
Y_{n, t} = \bar{f}(\bU, \bA; n, t) = f(U_n, U_{t, A_{n, t}}) + \varepsilon^{(A_{n, t})}_{n, t}.
%
\end{align}
%
Here $\varepsilon^{(A_{n, t})}_{n, t} \in \Rb$ is a random variable such that 
%
\begin{align}\label{eq:conditional_mean_zero}
%
\Ex[\varepsilon^{(A_{n, t})}_{n, t} \mid \bU] = 0.
%
\end{align}
%
\end{assumption}
\textcolor{blue}{First define potential outcomes. Then, observed outcomes as function of potential outcomes and the treatment.}

%
$\varepsilon^{(A_{n, t})}_{n, t}$ can be thought of as the variation in $\bar{f}(\bU, \bA; n, t)$ not captured by the latent factors $(U_n, U_{t, A_{n, t}})$.
%
Assumption \ref{assumption:outcome_function} implicitly imposes that observed outcome $Y_{n, t}$ is only a function of the intervention $A_{n, t}$ that unit $n$ receives for measurement $t$.
%
That is, conditioned on $(U_n, U_{t, A_{n, t}})$, $A_{n, t}$ does not depend on $A_{n', t'}, Y_{n', t'}$ for $n' \neq n$ and/or $t' \neq t$.
%
Further, the effect of intervention $A_{n, t}$ affects the observed outcome only through the variables $(U_{t, A_{n, t}}, \varepsilon^{(A_{n, t})}_{n, t})$.
%

We can now define potential outcomes for $n$, measurement $t$, and intervention $a$ as 
%
\begin{align}\label{eq:potential_outcomes}
%
Y^{(a)}_{n, t} = f(U_n, U_{t,a}) + \varepsilon^{(a)}_{n, t}.
%
\end{align}
%
Assumption \ref{assumption:outcome_function} states that the potential outcome can $Y^{(a)}_{n, t}$ be written as a function of the factors $(U_n, U_{t, a})$; $\varepsilon^{(a)}_{n, t}$ is the variation in the potential outcome $Y^{(a)}_{n, t}$ not explained by $(U_n, U_{t, a})$.
%
Hence, the no-interference (SUTVA) restriction \citep{rubin1980basu} holds.
%
\begin{remark}\label{remark:non-linear_epsilon}
%
We note that a potential outcome function of the form $Y^{(a)}_{n, t} = \bar{f}(U_n, U_{t, a}, \bar{\varepsilon}^{(a)}_{n, t})$ can be nested into \eqref{eq:potential_outcomes} under additional conditions on the distribution of $\varepsilon^{(a)}_{n, t}$.
%
In particular, assume that the distribution of $\bar{\varepsilon}^{(a)}_{n, t}$ is identical across $n, t, a$.
%
Then we can write $$\Ex[Y^{(a)}_{n, t} \mid U_n, U_{t, a}] = \Ex[\bar{f}(U_n, U_{t, a}, \bar{\varepsilon}^{(a)}_{n, t}) \mid U_n, U_{t, a}] = f(U_n, U_{t, a}).$$
%
In particular, because the distribution of $\bar{\varepsilon}^{(a)}_{n, t}$ is not dependent on $(n, t, a)$, the conditional expectation $\Ex[Y^{(a)}_{n, t} \mid U_n, U_{t, a}]$ can be written as only a function of $U_n, U_{t, a}$.
%
Then define 
%
$$\varepsilon^{(a)}_{n, t} = Y^{(a)}_{n, t} - \Ex[Y^{(a)}_{n, t} \mid U_n, U_{t, a}].$$
%
By construction, we have that {\color{blue} $\Ex[\varepsilon^{(A_{n, t})}_{n, t} \mid \bU] = 0.$}
%
Hence Assumption \ref{assumption:outcome_function} holds. 
%
\end{remark}


%
Analagously to the outcome function, we next impose that the outcome for measurement $(n, t)$ is only a function of the confounders $U_n$ and $U_{t, A_{n, t}}$.%
\begin{assumption}\label{assumption:intervention_function}
%
There exists a function $h: \mathcal{U} \times \tilde{\mathcal{U}}^{|\Ac|} \to \Ac$, such that the intervention assignment for unit $n$ and measurement $t$ is given by 
%
\begin{align}
    A_{n, t} = \bar{h}(\bU; n, t) = h(U_n, (U_{t, a})_{a \in \Ac}) + \nu_{n, t}
\end{align}
%
Here $\nu_{n, t} \in \Rb$ is a random variable such that 
\begin{align}
    \Ex[\nu_{n, t} \mid \bU] = 0.
\end{align}
%
\end{assumption}
%
Assumption \ref{assumption:intervention_function} states that the intervention assignment $A_{n, t}$ be written as a function of the factors $(U_n, (U_{t, a})_{a \in \Ac})$;
%
$\nu_{n, t}$ is the variation in the intervention assignment  not explained by $(U_n, U_{t, a})$.
%
Assumption \ref{assumption:intervention_function} implicitly imposes that if say different measurements indexed by $t$ correspond to measurements obtained at different time periods, then $A_{n, t}$ cannot be adaptive to previously observed outcomes and intervention assignments; it also cannot be adaptive to the observed outcomes and intervention assignments for other units $n' \neq n$.
%


%
We call $\bU$ possible confounders as they affect both the treatment assignments $\bA$ and the outcomes $\bY$.
%
For $\bU$ to represent {\em all} possible confounders, we require making the following assumption.
%
We first introduce some necessary notation: let $\bE = [\varepsilon^{(a)}_{n, t}]_{n \in [N], t \in [T], a \in \Ac}$ and $\bN = [\nu_{n, t}]_{n \in [N], t \in [T]}$.
%

\begin{assumption}[Conditional Independence]\label{assumption:conditional_independence}
%
We assume independence of $\bE$ and $\bN$ conditional on $\bU$.
%
That is,
%
$\bE \indep \bN  \mid \bU.$
%
\end{assumption}
\textcolor{blue}{Should we use that the $\nu_{n,t}$ are independent of the $\varepsilon_{n,t}^{(a)}$ or similar? Plus independence across $n$?}
%
As an immediate consequence of Assumptions \ref{assumption:confounder_structure}, \ref{assumption:outcome_function}, \ref{assumption:intervention_function}, and \ref{assumption:conditional_independence} we have that 
%
$$Y^{(a)}_{n, t} \indep \bA \mid \bU.$$
%
Figure \ref{figure:dag} provides a directed acyclic graph (DAG) that is consistent with the assumptions above.
%
We note that the various factors $[ (U_n)_{n \in [N]}, (U_{t, a})_{t \in [T], a \in \Ac}]$ can be arbitrarily correlated with each other. 
%
However, these assumptions also imply that 
%
$$Y^{(a)}_{n, t} \mid \bU = Y^{(a)}_{n, t} \mid U_n, U_{t, a}.$$
%
That is conditional on $U_n, U_{t, a}$, the potential outcome $Y^{(a)}_{n, t}$ is independent of the other factors.



\subsection{Encoding Latent Structure Across Potential Outcomes}\label{sec:latent_structure}
%
Thus far, we have made no restrictions on $(U_n, U_{t, a})$, and $f$. 
%
For example, $(U_n, U_{t, a})$ could be infinite-dimensional, and $f$ could be an arbitrary function of these quantities.
%
To make progress, we impose some structure on the process that generates potential outcomes. 
%


\begin{assumption}[Holder continuity of outcome generating function]\label{assumption:holder.mech}
%
We make the following assumptions on $U_n$ and $f$.

\begin{enumerate}
%
\item $U_n \in \Rb^{q}$
%
\item For any $U_{t, a}$ for $t \in [T], a \in \Ac$, we have $f(\cdot, U_{t, a})$ is H\"older continuous (see Definition \ref{def:holder}), i.e., $f(\cdot, U_{t, a}) \in \Hc(q,S,C_H)$, where $C_H < C$.
\end{enumerate}
%
\end{assumption}
%
Assumption \ref{assumption:holder.mech} is a continuity condition that posits that if latent variables $U_{n_1}$ and $U_{n_2}$ for any two units $n_1$ and $n_2$ are close (that is, if $U_{n_1}\approx U_{n_2}$), then their average potential outcomes are close as well, (that is, $\Ex[Y^{(a)}_{n_1, t} | \bU] \approx \Ex[Y^{(a)}_{n_2, t} | \bU]$, for all $t \in [T], a \in \Ac$).
%
Assumption \ref{assumption:holder.mech} does not impose smoothness of $\Ex[Y^{(a)}_{n, t} | \bU]$ with respect to the latent variable $U_{t, a}$. 
%

A linear factor model, $f(U_n, U_{t, a}) = \ldot{U_n}{U_{t, a}}$, is a special case of Assumption \ref{assumption:holder.mech}. 
%
A linear factor model satisfies Definition \ref{def:holder} for all $S \in \mathbb{N}$ and $C_H = C$, for some absolute positive constant $C<\infty$. 
%
Proposition \ref{prop:factor_model_approx} establishes that linear factor models of sufficiently large dimension also provide a ``universal'' representation for smooth non-linear factor models.

\begin{proposition}[H\"older low rank matrix approximation, \citeauthor{agarwal2021robustness}, \citeyear{agarwal2021causal}]\label{prop:factor_model_approx}
%
Suppose Assumption \ref{assumption:holder.mech} holds.
%
Then, for any $\delta>0$, there exist latent variables $\lambda_n, \rho_{t, a} \in \Rb^r$ such that:
%
\begin{align}
%
\left| f(U_n, U_{t, a}) - \ldot{\lambda_n}{\rho_{t, a}} \right| \leq \Delta_E,
%
\end{align}
%
where for $C$ that is allowed to depend on $(q,S)$,
%
\begin{align}
%
r \le C \cdot \delta^{-q}, \quad \Delta_E \le C_H \cdot \delta^S.
%
\end{align}
%
\end{proposition}
%
\textcolor{blue}{There is something weird in this result. From the statement of the Proposition, one would think that $f(\cdot, U_{t,a})$ is a infinitely-differentiable function with bounded derivatives, then we can reproduce it without error (given the second inequality in the proposition and the fact that $C$ in the first equality is (presumably) decreasing in $S$.}
Proposition \ref{prop:factor_model_approx} establishes that if $f$ has a H\"older smooth latent variable representation, then it is uniformly well-approximated by a linear factor model of finite dimension, $r$.
%
For $\delta<1$ we have that as the latent dimension $q$ increases, the bound on the rank $r$ increases, and as smoothness $S$ increases, the bounds on the approximation error $\Delta_E$ decreases.
%
If we take $\delta = (\mbox{min}\{N, T\})^{-c}$ for some constant $c$, such that $0<c<1/q$, we obtain $r \ll \mbox{min}\{N, T\}$ and $\Delta_E = o(1)$ as $N, T \to \infty$.
%




\subsubsection{Nesting Classical Econometric Models}\label{sec:econometric_models}
%
Our framework nests some classical econometric models, which we describe below.
%
\begin{example}[Two-way fixed effects model]
%
Suppose 
\[
f(U_n, U_{t, a}) = \ldot{U_n}{U_{t, a}},
\]
where 
\[
U_n = \left(\begin{array}{c} \beta_n\\ \mu_n\\1 \end{array}\right),
\quad  U_{t, a} = \left(\begin{array}{c}a \\ 1 \\ v_t \end{array}\right).\vspace{.2cm}
\]
Here, $\mu_n$, $v_t$ are scalars, and $a$ and $\beta_n$ have dimension $p$. Then, $r = p+2$ and 
\[
Y^{(a)}_{n, t} = \ldot{a}{\beta_n} + \mu_n + v_t + \varepsilon^{(a)}_{n, t},
%
\quad Y_{n, t} = \ldot{A_{n, t}}{\beta_n} +\mu_n + v_t + \varepsilon^{(A_{n, t})}_{n, t}.
\]
%
This corresponds to a two-way fixed effect model with heterogeneous coefficients on the intervention. Time-varying intervention coefficients can be easily accommodated in the same setting. 
%
A simple example is  
\[
U_n = \left(\begin{array}{c} \beta_n\\ \mu_n\\1 \end{array}\right),
\quad  U_{t, a} = \left(\begin{array}{c} \ldot{F_t}{a}  \\ 1 \\ v_t \end{array}\right).\vspace{.2cm}
\]
where $F_t$ is a $(p\times p)$ matrix of time-varying coefficients and the dimensions of the other components is unchanged. Then,
\[
Y^{(a)}_{n, t} = \ldot{a}{\beta_{n, t}}+\mu_n + v_t + \varepsilon^{(a)}_{n, t},
\quad Y_{n, t} = \ldot{A_{n, t}}{\beta_{n, t}} +\mu_n + v_t + \varepsilon_{n, t},
\]
where $\beta_{n,t}=F_t\beta_n$.
%
\end{example}

\begin{example}[Interactive fixed effects model, \citeauthor{bai2009interactive}, \citeyear{bai2009interactive}]
Suppose
\[
f(U_n, U_{t, a}) = \ldot{U_n}{U_{t, a}},
\]
where 
\[
U_n = \left(\begin{array}{c} 1\\ \mu_n\end{array}\right),
\quad  U_{t, a} = \left(\begin{array}{c}\ldot{a}{\beta} \\ v_t \end{array}\right), 
\]
and $\mu_n$ and $v_t$ are factors of dimension $k$. 
Then, $r=k+1$ and
\[
Y^{(a)}_{n, t} = 
\ldot{a}{\beta} + \ldot{\mu_n}{v_t} + \varepsilon^{(a)}_{n, t},
\quad Y_{n, t} = \ldot{A_{n, t}}{\beta}
+ \ldot{\mu_n}{v_t} + \varepsilon_{n, t}.
\]
\end{example}
\textcolor{blue}{Include similar example with Martin Weidner model.}

\begin{example}[Binary choice]
%
Let $I_{\mathcal S}$ be the indicator function for set $\mathcal S$. 
%
Consider
\[
Y_{n, t}^{(a)}=I_{[0,\infty)}\left(F\left(\ldot{a}{\beta}+\mu_n+v_t\right)-e_{n, t}^{(a)}\right),
\]
where $F(\cdot)$ is a (H\"{o}lder) continuous function mapping to $[0, 1]$, and for every $(n, t, a)$, $e_{n, t}^{(a)}$ is an independent realization of a continuous random variable. 
%
Without loss of generality, we can assume that $e_{n, t}^{(a)}$ is uniformly distributed on $[0,1]$ (if $e_{n, t}^{(a)}$ is not uniform on $[0,1]$, we can apply the probability integral transform, $f$, to both $F\left(\ldot{a}{\beta}+\mu_n+v_t\right)$ and $e_{n, t}^{(a)}$, where $f$ is the cumulative distribution function of $e_{n, t}^{(a)}$). 
%
Then, by Remark \ref{remark:non-linear_epsilon}, we have that 
\[
f(U_n,U_{t,a}) = F\left(\ldot{U_n}{U_{t,a}}\right),
\]
with
\[
U_n = \left(\begin{array}{c} 1\\ \mu_n\\1 \end{array}\right),
\quad  U_{t, a} = \left(\begin{array}{c}\ldot{a}{\beta} \\ 1 \\ v_t \end{array}\right).\vspace{.2cm}
\]
\end{example}


\begin{example}[Dictionary basis expansion]
%
Consider 
\[
Y_{n, t}^{(a)}= \gamma_n(a, X_t) + \varepsilon^{(a)}_{n, t},
\]
where $X_t, a \in \Rb^p$, and $\gamma_n: \Rb^{2p} \to \Rb$ has the following dictionary representation
\[
\gamma_n(a, X_t) = \sum^r_{\ell = 1} \alpha_{n, \ell} b_{\ell}(a, X_t),
\]
\end{example}
where $\alpha_{n, \ell} \in \Rb$, and $ b_{\ell}: \Rb^{2p} \to \Rb$ are dictionary basis functions. 
%
For example, $b_{\ell}$ could be a polynomial of $a$ and $X_t$.
%
Then,
\[
f(U_n, U_{t, a}) = \ldot{U_n}{U_{t,a}},
\]
with
\[
U_n = \left(\begin{array}{c} \alpha_{n, 0}\\ \vdots \\ \alpha_{n, L} \end{array}\right),
\quad  U_{t, a} = \left(\begin{array}{c}b_{0}(a, X_t)\\ \vdots \\ b_{L}(a, X_t) \end{array}\right).\vspace{.2cm}
\] 

{\color{blue} Need to add another non-linear model}

\subsection{Intervention Assignment Function}\label{sec:latent_structure_intervention}
%
\begin{assumption}[Holder continuity of outcome generating gunction]\label{assumption:holder.mech_intervention}
%
We make the following assumptions on $U_n$ and $h$.

\begin{enumerate}
%
\item $U_n \in \Rb^{q}$
%
\item For any $U_{t, a}$ for $t \in [T], a \in \Ac$, we have, $h(\cdot, U_{t, a})$ is H\"older continuous (see Definition \ref{def:holder}), i.e., $h(\cdot, U_{t, a}) \in \Hc(q,\bar{S},\bar{C}_H).$, where $\bar{C}_H < C$.
\end{enumerate}
%
\end{assumption}
%
We discuss two types of intervention assignment functions.
%
The first type are those that satisfy Assumptions \ref{assumption:confounder_structure}, \ref{assumption:outcome_function}, \ref{assumption:intervention_function}, and \ref{assumption:conditional_independence}.
%
That is, the confounders have a latent factorization and there is selection on this . 
%
The second type are assignment functions that in addition satisfy Assumption \ref{assumption:holder.mech_intervention}, i.e., there 

\subsubsection{Nesting Classical Intervention Assignment  Mechanisms}\label{sec:intervention_assignment_models}
%
Below we give illustrative concrete examples of treatment assignments seen in data and how they fit with our model.

\begin{example}[Randomized trial]\label{example:RCT}
%
Let $\Ac = \{0, 1\}$.
%
Consider a setup of a randomized trial where the $N$ units are assigned one of the two treatments at random, where the probability can differ across measurements.
%%
Specifically, for all $n \in [N], t \in [T]$
%
\begin{align}
%
A_{n, t}
%
= \begin{cases}
%
1 &  \mbox{with probability}~p_t, \\
%
0 & \mbox{otherwise.} 
%
\end{cases}
%
\end{align}
%
In this case, there is no confounding as the treatment assignment is not correlated with the outcomes, i.e., $h(U_n, U_{t,a}) = 0$. 
%
We can see $\nu_{n, t}$ to be a random variable that takes value $1$ with probability $p_t$ and $0$ with probability $1 - p_t$.
%
\end{example}

\begin{example}[Selection on observables]\label{example:observables}
%
Suppose there are observables covariates 
$X_n, X_{t, a}\in \Rb^q$ such that the intervention assignment is given by
%
\begin{align}
%
\Ex[\mathbbm{1}(A_{n, t} = a) \mid X_n, X_{t, a}]
 = p_{n, t, a} = \sigma(X_n, X_{t, a}),
%
\end{align}
%
such that $\sum_{a \in \Ac} p_{n, t, a} = 1$, and where $\sigma$ is a (H\"{o}lder) continuous function mapping to $[0, 1]$ (e.g., the logistic function).
%
Here we can take 
%
$$
h(U_n, U_{t, a}) = \sigma(X_n, X_{t, a})
$$
%
with
\[
U_n = X_n,
\quad  U_{t, a} = X_{t, a}.\vspace{.2cm}
\] 
%
This would be considered selection on observables if
\begin{align}
    Y^{(a)}_{n, t} = f(X_n, X_{t, a}) + \varepsilon^{(a)}_{n, t}.
\end{align}
%
That is, all confounders are observed.
%
\end{example}

{\color{blue} Anish: Following examples allow for selection on latent factors, but I don't believe the intervention assignment function satisfies a H\"{o}lder) continuous function assumption - they are all threshold functions}

\begin{example}[Regression Discontinuity]\label{example:regdisc_score}
%
Let $\Ac = \{0, 1\}$.
%
Suppose units correspond to schools.
%
Measurements correspond to a tuple of different grade levels and subjects.
%
Intervention $1$ corresponds to additional teaching resources being given and $0$ refers to the current standard.
%
The outcome $Y_{n, t}$ of interest can be the end-of-year passing rate for a school and (grade, subject).
%
A school $n$ is given intervention $1$ for a particular measurement $t$---corresponding to a (grade, subject)---if and only if the average test score, $X_{n, t}$ for that (grade, subject) is lower than $\theta_t$.
%
Specifically,
%
\begin{align}
A_{n, t}
= \begin{cases}
1, &  \text{if} ~ X_{n, t} < \theta_t \\
0 &  \text{otherwise} 
\end{cases}
\end{align}
%
Let $U_n, U_t$ be latent confounders that affect both the test score for a particular school and (grade, subject), and the end-of-year passing rate. 
%
That is,
%
\begin{align}
%
X_{n, t} = \ell(U_n, U_{t}), 
%
\quad Y^{(a)}_{n, t} = f(U_n, U_{t}) + \varepsilon^{(a)}_{n, t}
%
\end{align}

Here we can take 
%
$$
h(U_n, U_{t, a}) = \mathbbm{1}(\ell(U_n, U_{t}) < \theta_t)
$$
%
with
\[
U_n = U_n,
\quad  U_{t, a} = (U_t, \theta_t).\vspace{.2cm}
\] 
%
\end{example}


{\color{blue} 
\begin{example}[Threshold Rules: Block Missingness pattern]\label{example:block}
%
Let $\Ac = \{0, 1\}$.
%
Let $U_n, U_{t, a} \in \Rb$. 
%
Let $\mu, \tilde{\mu} \in \Rb$ be given thresholds. Let the intervention assignment be
\begin{align}
A_{n, t}
= \begin{cases}
1 &  \mbox{if\ \,} U_n > \mu \mbox{ and\ }U_{t, 1} - U_{t, 0} > \tilde{\mu}, \\
0 & \mbox{otherwise.} 
\end{cases}
\end{align}
That is, unit $n$ receives intervention $A_{n,t} = 1$ only if both the unit specific confounder $U_n$ and the measurement, intervention specific confounders $\sum_{\ell=1}^r(U_{t,1,\ell} - U_{t,0,\ell})$ are greater than $\mu$ and $\tilde{\mu}$, respectively.
\end{example}

\begin{example}[Staggered Adoption]\label{example:staircase}
Let $\Ac = \{0, 1\}$, $U_n \in \Rb^r$, and $U_{t, a} \in \Rb^r$.
Let the intervention assignment be: 
\begin{align}
A_{n, t}
= \begin{cases}
1, &  \exists\, t' \le t: \ldot{U_n \ }{\ \sum^{t'}_{\ell = 1}U_{\ell, 1} - U_{\ell, 0}} > 0 \\
0 &  \text{otherwise} 
\end{cases}
\end{align}
A key difference relative to Example \ref{example:block} is that the treatment assignment rule implies $A_{n, t} = 1$ if $A_{n, t - 1} = 1$, regardless of $U_n, U_{t, 0}, U_{t, 1}$.
That is, the intervention $1$ is an ``absorbing state''.
% The assignment mechanism in this example generates the staircase sparsity pattern in {\color{red} Figure \ref{fig:xxx}}.
\end{example}

\begin{example}[Regression Discontinuity - Time]\label{example:regdisc_time}
%
Let $\Ac = \{0, 1\}$.
%
Suppose units correspond to individuals. 
%
Each individual is assigned intervention $1$ 
if and only if they are above certain age, $\theta$.
%
Let $U_n$
Individual $n$ has associated 
$U_n \in \Rb^r$ with $U_{n}$ representing the birth year of the individual $n$ which might be observed while other co-ordinates are unobserved. 
Let $t$ denote the year.
By design, 
\begin{align}
A_{n, t}
= \begin{cases}
1, &  \text{if} ~ t - U_{n1} > \bar\theta \\
0 &  \text{otherwise} 
\end{cases}
\end{align}
\end{example}

Anish: Fix/discuss above examples
}

==> Old/content/outcome_factor_structure.tex <==
\section{Identification and Estimation of Treatment Effects \\ with Factor Structure in Potential Outcomes}\label{sec:outcomes_factor_structure}
%
In this section, we focus on the identification and estimation of treatment effects when we only impose a smooth non-linear factor model in the potential outcomes (i.e., Assumption \ref{assumption:holder.mech}).
%
We {\em do not} assume a smooth non-linear factor model holds for the intervention assignment mechanism (i.e., Assumption \ref{assumption:holder.mech_intervention}).
%
We study how to exploit factor structure in both the outcome generating function and the intervention assignment function in Section \ref{sec:assignment_factor_structure}.

%
{\bf Causal parameters of interest.}
%
In this section, we restrict our attention to the binary treatment setting where for all $t \in [T]$, we let $\Ac = \{0, 1\}$.
%
{\color{blue} Our analysis easily extends for any finite $\Ac$.}
%
We focus on the estimation of the average treatment effect for a given measurement $t^*$, and for a subset of units $\Mc \subset [N]$, with $|\Mc| = M$: 
%
\begin{align}
%
\mathsf{ATE}_{\Mc} = \frac{1}{M}\sum_{n \in \Mc} \Big(Y^{(1)}_{n, t^*} - Y^{(0)}_{n, t^*} \Big).
%
\end{align}
%
Let 
%
\begin{align}
%
\Ic^{(a)} = \{n \in [N] : A_{n, t^*} = a\}, \quad N_a = |\Ic^{(a)}|.
%
\end{align}
%
That is, $\Ic^{(a)}$ is the set of units that received intervention $a$ for measurement $t^*$, and $N_a$ is the number of units in that set.
%
For different subsets $\Mc$, $\mathsf{ATE}_{\Mc}$ nests a variety of causal parameters of interest:
%
\begin{itemize}
%
\item If $\Mc = \Ic^{(1)}$ (all the units that were treated during measurement $t^*$), then $\mathsf{ATE}_{\Mc}$ corresponds to the {\em average treatment effect on the treated}, which we denote as $\mathsf{ATT}$.
%
\item If $\Mc = \Ic^{(0)}$ (all the units that were untreated during measurement $t^*$), then $\mathsf{ATE}_{\Mc}$ corresponds to the {\em average treatment effect on the  untreated}, which we denote as $\mathsf{ATU}$.
%
\item If $\Mc = [N]$ , then $\mathsf{ATE}_{\Mc}$ corresponds to the {\em average treatment effect}, which we denote as $\mathsf{ATE}$.
%
% \item {\color{red} Suppose we have access to covariates $[X_n]_{n \in [N]}$ for the various units (e.g. demographic data, historical purchasing data). If we let $\Mc = \{n \in [N]: X_n = x\}$, then $\mathsf{ATE}_{\Mc}$ corresponds to the {\em conditional average treatment effect} for a given covariate $X$, which we denote as $\mathsf{CATE}(x)$.}
\end{itemize}
%
{\color{blue} For concreteness, we focus our estimation results on $\mathsf{ATT}, \mathsf{ATU}$, and $\mathsf{ATE}$. However, our results easily extend to any set of units $\Mc \subset [N]$.}

\subsection{Identification}
%
We now show how the model for treatment assignment and potential outcomes, summarized by Assumptions \ref{assumption:conditonal_independence},
\ref{assumption:outcome_generating_function_factor_structure}, and \ref{assumption:holder.mech} lead to a novel identification argument for $\mathsf{ATE}_{\Mc}$.
%
Motivated by Proposition \ref{prop:factor_model_approx}, we define the linear factor model approximation error to $g(U_n, \tilde{U}_{t, a})$ as follows.
%
\begin{definition}[Linear factor model approximation]\label{def:linear_factor_approx}
%
For $r \in \Nb$, let $\{\lambda_n \}_{n \in [N]} \cup  \{ \rho_{t, a} \}_{t \in [T], a \in \Ac}$, with $\lambda_n, \rho_{t, a} \in \Rb^r,$ be (one of) the linear factor model approximations of $g(U_n, \tilde{U}_{t, a})$ that minimizes $\Delta_E$ where, 
%
\begin{align}
%
\Delta_E = \max_{n \in [N], t \in [T], a \in \Ac}| \eta^{(a)}_{n, t} |, \quad \text{and } \eta^{(a)}_{n, t} = g(U_n, \tilde{U}_{t, a}) - \ldot{\lambda_{n}}{\rho_{t, a}}.
%
\end{align}
%
\end{definition}
%
Recall that if $g$ is H\"older continuous, then Proposition \ref{prop:factor_model_approx} implies that both $r$ and $\Delta_E$ can be simultaneously controlled.

%
We define two subsets of $\Mc$: for $a \in \{0, 1\}$,
%
\begin{align}
%
\Mc^{(a)} = \{ n \in \Mc : A_{n, t^*} = a \},
%
\quad M_a = |\Mc^{(a)}|.
%
\end{align}
%
Note that $\Mc^{(a)} \subset \Ic^{(a)}$.
%
We are now equipped to define the key assumption we require for identification of the causal parameter of interest.
%
\begin{assumption}[Linear span inclusion]\label{assumption:linear_span_inclusion}
%
For $a \in \{0, 1\}$, let $\lambda_{\Mc^{(1 - a)}} = \sum_{n \in \Mc^{(1 - a)}} \lambda_n$.
%
We assume there exists linear weights $\beta^{(a)} \in \Rb^{N_{a}}$ such that 
%
\begin{align}\label{equation:weights}
%
\lambda_{\Mc^{(1 - a)}} = \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \lambda_n.
%
\end{align}
%
That is, $\lambda_{\Mc^{(1 - a)}}$ lies in the linear span of $\{\lambda_n\}_{n \in \Ic^{(a)}}$.
%
In settings where there are multiple weights that satisfy condition \eqref{equation:weights}, we define $\beta^{(a)}$ to be the unique one with minimum $\ell_2$-norm.
%
\end{assumption}
%
\begin{remark}
%
{\color{blue} Remark about norm of $\beta^{(a)}$.}
%
\end{remark}
%
This assumption implicitly adds another restriction on the treatment assignment over what is already imposed by Assumption 
\ref{assumption:outcome_generating_function_factor_structure}.
%
For example, Assumption \ref{assumption:linear_span_inclusion} does not allow for a treatment assignment mechanism such that the latent factors associated with the units in $\Ic^{(a)}$ and $\Mc^{(1 - a)}$ live in orthogonal spaces.
%
Hence the assignment mechanism needs to be diverse enough, so that the latent factors associated with the units in different treatments are linearly expressible in terms of each other.
%
We only require the weaker condition that this linear span inclusion holds for the {\em sum} of the unit latent factors associated with $\Mc^{(1 - a)}$, as opposed to it holding for {\em each} latent factor $\lambda_n$ for $n \in \Mc^{(1 - a)}$. 

\begin{theorem}[Identification]\label{thm:ate_idenfication}
%
Let Assumptions \ref{assumption:conditional_independence}, and \ref{assumption:linear_span_inclusion} hold.
%
Then, given $\beta^{(a)}$ for $a \in \{0, 1\}$,
%
\begin{align}\label{eq:ate_identification}
%
\sum_{n \in \Mc} \Ex[Y^{(a)}_{n, t^*} \mid \LF]
%
&= \sum_{n \in \Mc^{(a)}} \Ex[Y_{n, t^*} \mid \bA, \LF] 
%
+ \sum_{n \in\Ic^{(a)}} \beta^{(a)}_n \Ex\left[Y_{n, t^*} \mid \bA, \LF\right]
%
- \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \eta^{(a)}_{n, t^*}
%
+ \sum_{n \in \Mc^{(1-a)}} \eta^{(a)}_{n, t^*},\quad
%
\end{align}
%
where expectations are taken over the distribution of $\varepsilon^{(a)}_{n, t^*}$.
%
\end{theorem}

\begin{corollary}[Identification]\label{cor:ate_identification}
Let 
\begin{align}
\mathsf{Observed}_{a} = 
%
\frac{1}{M}\left(\sum_{n \in \Mc^{(a)}} \Ex[Y_{n, t^*} \mid \bA, \LF] 
%
+ \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \Ex\left[ Y_{{n, t^*}} \mid \bA, \LF \right]\right),
%
\end{align}
%
and
%
\begin{align}
%
\mathsf{Observed} =
%
\mathsf{Observed}_{1} - \mathsf{Observed}_{0}.
%
\end{align}
%
Then, under the conditions of Theorem \ref{thm:ate_idenfication},
%
\begin{align}\label{eq:ate_identification_full}
%
\Big| \Ex[\mathsf{ATE}_{\mathcal{M}} \mid \LF] - \mathsf{Observed} \Big| 
%
\le \Delta_E \left(1 + \frac{\| \beta^{(0)}\|_1 + \| \beta^{(1)}\|_1}{M} \right).
%
\end{align}
%
\end{corollary}

% {\color{blue}
% \begin{remark}
% Note by simply integrating \eqref{eq:ate_identification} and \eqref{eq:ate_identification_full} with respect to $\LF$, we have an identification result that is not conditional on $\LF$. \textcolor{teal}{But then, the assumptions hold a.s.~for all $\LF$?} Don't we already need to make that assumption? \textcolor{teal}{I think it is a bit more complicated than this. Two issues. First: To obtain Corollary 1, we are applying Proposition 1 which is a point-wise result. Second: $\beta^{(0)}$ and $\beta^{(1)}$ change with $\LF$. So the bound on the right-hand side depends on $\LF$.}
% \end{remark} 
% }

\subsection{Estimator}
The identification result in Corollary \ref{cor:ate_identification} suggests an estimator of the form 
%
\begin{align}\label{eq:ATE_synthetic_estiamtor}
%
\widehat{\mathsf{ATE}}_{\Mc}
%
= \frac{1}{M} \left(\sum_{n \in \Mc^{(1)}} Y_{n, t^*} 
%
+ \sum_{n \in \Ic^{(1)}} \hbeta^{(1)}_n Y_{n, t^*} \right)  
%
- \frac{1}{M} \left(\sum_{n \in \Mc^{(0)}} Y_{n, t^*} 
%
+  \sum_{n \in \Ic^{(0)}} \hbeta^{(0)}_n Y_{n, t^*} \right),
%
\end{align}
%
where $\hbeta^{(1)}_j$ and $\hbeta^{(0)}_j$ are estimates of $\beta^{(1)}_j$ and $\beta^{(0)}_j$, respectively. 
%
That is, $\widehat{\mathsf{ATE}}_{\Mc}$ imputes the sums of the unobserved potential outcomes with and without treatment by $\sum_{n \in \Ic^{(1)}} \hbeta^{(1)}_n Y_{n, t^*}$ and $\sum_{n \in \Ic^{(0)}} \hbeta^{(0)}_n Y_{n, t^*}$, respectively.

%
In Sections \ref{sec:abstract_finite_sample} and \ref{sec:abstract_normality}, we provide sufficient conditions on any estimator $\hbeta^{(a)}$ of $\beta^{(a)}$, which establish the finite-sample consistency and asymptotic normality of $\widehat{\mathsf{ATE}}_{\Mc}$.
%
Hence, we denote 
%
\begin{align}
%
\Delta_{\beta^{(a)}} = \hbeta^{(a)} - \beta^{(a)}.
%
\end{align}
%
In Section \ref{sec:PCR}, we provide explicit conditions for consistency and normality when the estimator for $\hbeta^{(a)}$ is principal component regression (PCR).  


\subsection{Finite-Sample Consistency}\label{sec:abstract_finite_sample}
%
To establish consistency, we make the (mild) assumption that the potential outcomes $Y^{(a)}_{n, t}$ have a sub-Gaussian distribution.

{\color{blue}
\begin{assumption}[Sub-Gaussian potential outcomes]\label{assumption:sub-gaussian_noise}
%
Let $Y^{(a)}_{n, t} \mid \LF$ be a sub-Gaussian random variable with standard deviation $\sigma^{(a)}_{n, t}$. 
%
Hence, $\varepsilon^{(a)}_{n, t} \mid \LF$ is also a sub-Gaussian random variable with standard deviation $\sigma^{(a)}_{n, t}$.
%
Let $\sigma_\max = \max_{n \in [N], t \in [T], a \in \{0, 1\}} \sigma^{(a)}_{n, t}$, and assume $\sigma_\max < C$.
%
\end{assumption}}

% \textcolor{teal}{Abadie: This is an assumption in terms of the epsilons, but the epsilons are not primitives of the model. Should not the assumption be done on the model instead?}

% \textcolor{teal}{Sub-Gaussianity of the distribution of potential outcomes (given $\LF$ ) seems enough. Also, in the future we may want to relax the independence assumptions on $\varepsilon^{(a)}_{n, t}$. It does not seem necessary.}


% \textcolor{teal}{Abadie: I do not think $\varepsilon^{(a)}_{n, t} \mid \LF$ has a conventional meaning. $\varepsilon^{(a)}_{n, t} \mid \LF=u$ is a r.v., $E[\varepsilon^{(a)}_{n, t} \mid \LF]$ is also a r.v. What exactly do we mean when we use $\varepsilon^{(a)}_{n, t} \mid \LF$ and the like? This will confuse people and we may want to stick to conventional notation.
% }

%
\begin{proposition}[Conditions for consistency for any linear estimator]\label{prop:ate_estimation}
%
Let Assumptions \ref{assumption:conditonal_independence},
\ref{assumption:outcome_generating_function_factor_structure},  \ref{assumption:linear_span_inclusion}, and \ref{assumption:sub-gaussian_noise} hold.
%
Let $Y_{\Ic^{(a)}} = [Y_{n, t^*}]_{n \in \Ic^{(a)}}$.
%
Then,
%
\begin{align}
\widehat{\mathsf{ATE}}_{\Mc} &- \Ex[\mathsf{ATE}_{\Mc} \mid \LF]\\ 
&\le \Delta_E \left(1 + \frac{\| \beta^{(0)}\|_1 + \| \beta^{(1)}\|_1}{M} \right)\\
&+ O_p\left( \sum_{a \in \{0, 1\}} \frac{\sigma_\max \left(\sqrt{M_a} +  \|\beta^{(a)} \|_2 + \|\Delta_{\beta^{(a)}}\|_2\right) +  \ldot{\Delta_{\beta^{(a)}}  }{\Ex\left[ Y_{\Ic^{(a)}} \right]}}{M} \right). \label{eq:ate_est_thm}
\end{align}

\end{proposition}

\begin{corollary}\label{cor:ate_estimation}
%
Let the conditions of Proposition \ref{prop:ate_estimation} hold. 
%
Then
%
\begin{align}\label{eq:ate_est_thm_non_expected}
%
\widehat{\mathsf{ATE}}_{\Mc}  - \mathsf{ATE}_{\Mc} \mid \LF \le  \mathsf{Bound} 
%
\end{align}
%
where $\mathsf{Bound}$ is defined as the right hand side of \eqref{eq:ate_est_thm}.
%
\end{corollary}

% {\color{blue}
% \begin{remark}
% Note by simply integrating \eqref{eq:ate_est_thm} and \eqref{eq:ate_est_thm_non_expected} with respect to $\LF$, we have a finite-sample consistency result that is not conditional on $\LF$.
% \end{remark}
% }
% %

\subsection{Asymptotic Normality}\label{sec:abstract_normality}

For $a \in \{0, 1\}$, let
\begin{align}
%
\tau_{a} &= \frac{1}{M} \left( \left( \sum_{n \in \Mc^{(a)}} Y_{n, t^*} - \Ex[Y_{n, t^*} \mid \bA, \LF] \right) + \left( \sum_{n \in \Ic^{(a)}} \hbeta^{(a)}_n Y_{n, t^*} - \beta^{(a)}_n \Ex[Y_{n, t^*} \mid \bA, \LF] \right) \right) 
\end{align}
and
\begin{align}
\\ \mathsf{Approx} &=  \frac{1}{M} \left(\sum_{a \in \{0, 1\}}  \left(\sum_{n \in \Mc^{(1-a)}} \eta^{(a)}_{n, t^*} - \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \eta^{(a)}_{n, t^*} \right)\right).
%
\end{align}
%
By Theorem \ref{thm:ate_idenfication}, we have that 
\begin{align}
%
\widehat{\mathsf{ATE}}_{\Mc} - \Ex[\mathsf{ATE}_{\Mc} \mid \LF]
%
&= \mathsf{Approx} + \tau_{1} - \tau_{0}
%
\end{align}
%
Let 
\begin{align}
%
\bar{\sigma}^{(a)} &= \sqrt{\frac{\sum_{n \in \Mc^{(a)}} ((1 + \beta^{(a)}_n)\sigma^{(a)}_{n, t^*})^2 + \sum_{n \in \Ic^{(a)} \setminus \Mc^{(a)}} (\beta^{(a)}_n \sigma^{(a)}_{n, t^*})^2}{M}},
%
\\ \bar{\sigma} &= \sqrt{(\bar{\sigma}^{(1)})^2 + (\bar{\sigma}^{(0)})^2}
\end{align}
%
\begin{proposition}[Conditions for asymptotic normality for any linear estimator]\label{prop:ate_normality}
%
Let $\varepsilon_{\Ic^{(a)}} = [\varepsilon_{n, t^*}]_{n \in \Ic^{(a)}}$.
%
Let the conditions of Proposition \ref{prop:ate_estimation} hold. 
Assume the following additional conditions hold for $a \in \{0, 1\}$:
%
\begin{enumerate}
%
\item $
\frac{1}{\bar{\sigma} \sqrt{M}}  \ldot{\Delta_{\beta^{(a)}}}{\varepsilon_{\Ic^{(a)}}}
= o_p(1),$
%
\item $
\frac{1}{\bar{\sigma} \sqrt{M}}\ldot{\Delta_{\beta^{(a)}}}{\Ex\left[ Y_{\Ic^{(a)}} \mid \bA, \LF\right]}
= o_p(1).$
%
\item $\frac{\sqrt{M}}{\bar{\sigma}}  \mathsf{Approx} = o_p(1).$
%
\item $\frac{1}{(\bar{\sigma} \sqrt{M})^4}\sum^N_{n = 1} s_n = o(1)$,
%
where
%
\begin{align}
s_n
%
= \begin{cases}
%
C (1 + \beta^{(a)}_n)^4  & \text{ if } n \in \Mc^{(a)}, \\
%
C (\beta^{(a)}_n)^4  & \text{ if } n \in \Ic^{(a)} \setminus \Mc^{(a)}.
%
\end{cases}
\end{align}
%
\end{enumerate}
%
Then,
%
\begin{align}
%
\frac{\sqrt{M}}{\bar{\sigma}} \left( \widehat{\mathsf{ATE}}_{\Mc} - \Ex[\mathsf{ATE}_{\Mc} \mid \LF] \right) &\to \Nc(0, 1).
%
\end{align}
%
\end{proposition}


\section{Estimation results using Principal Component Regression (PCR)}
\label{sec:PCR}%

%
In Section \ref{sec:ate_pcr} below, we provide explicit bounds on $\Delta_{\beta^{(a)}}$ for the case when PCR is used to estimate the coefficients $\hbeta^{(a)}$.
%
Theorem \ref{thm:consistency_summary} collects sufficient conditions for consistency of $\widehat{\mathsf{ATE}}_{\Mc}$.


\subsection{Estimating Linear Weights via PCR}\label{sec:ate_pcr}
%
We now show how to estimate $\hbeta^{(a)}$ via PCR, and subsequently control $\Delta_{\beta^{(a)}}$ for the case when there are many measurements of all units under a common set of interventions. 

\noindent
{\bf Necessary notation to define PCR.}
%
We introduce now additional notation that we will use to discuss PCR estimation of $\hbeta^{(a)}$. 
%
Let $\bar{\Tc} \subset [T]$ be defined as follows:
%
\begin{align}
%
\bar{\Tc} = \{ t \in [T]: A_{n, t} = A_{n', t}\,\, \forall n, n' \in [N]\},
%
\quad \bar{T} = |\bar{\Tc}|.
%
\end{align}
%
That is, $\bar{\Tc}$ is the of measurements for which all units are seen under the same intervention.
%
Let $a_t$ be the common treatment value for $t \in \bar{\Tc}$.
%
For $a \in \{0, 1\}$, define
%
\begin{align}
%
\bY &= \left[\sum_{n \in \Mc^{(1 - a)}}Y_{n, t}\right]_{t \in \bar{\Tc}} \in \Rb^{\bar{T}},
%
\\ \bZ &= \Big[ Y_{n, t} \Big]_{t \in \bar{\Tc}, j \in \Ic^{(a)}} \in \Rb^{\bar{T} \times N_a},
%
\\ \bX &= \Big[ \Ex[Y_{n, t}] \Big]_{t \in \bar{\Tc}, j \in \Ic^{(a)}} \in \Rb^{\bar{T} \times N_a},
%
\\ \bX^{\text{lr}} &= \Big[\ldot{\lambda_{n}}{\rho_{t, a_t}}\Big]_{t \in \bar{\Tc}, n \in \Ic^{(a)}} \in \Rb^{\bar{T} \times N_a},
%
\end{align}
%
where to reduce notational burden we suppress dependence on $a$ in the notation for $\bY$, $\bZ$, and $\bX$.
%
$\bY$ is a vector of summed outcomes of the units in $\Mc^{(1 - a)}$ for the measurements in $\bar{\Tc}$,
%
$\bZ$ is a matrix of outcomes for the units in $\Ic^{(a)}$, and measurements in $\bar{\Tc}$, and $\bX$ is defined analogously to $\bZ$, but with respect to the expected observed outcomes.
%
$\bX^{\text{lr}}$ is the low-rank approximation of $\bX$; note $\bX - \bX^{\text{lr}} = [\eta^{(a_t)}_{n, t}]_{t \in \bar{\Tc}, n \in \Ic^{(a)}}$.

\noindent
{\bf PCR estimator for $\hbeta^{(a)}$.}
%
Define the singular value decomposition (SVD) of $\bZ$ as 
%
\begin{align}
%
\bZ = \sum^{\min(\bar{T}, N_a)}_{\ell = 1} \hat{s}_\ell \hat{u}_{\ell} \hat{v}^T_{\ell},
%
\end{align}
%
where $\hat{s}_\ell, \hat{u}_\ell, \hat{v}_\ell$ refer to the $\ell$-th singular value, left singular vector, and right singular vector, respectively.
%
For any SVD, we order the singular values by decreasing magnitude.
Given hyper-parameter $k \in [\min(\bar{T}, N_a)]$, we define $\widehat{\bX}^{\text{lr}}$ as follows:
%
\begin{align}\label{eq:PCR_step1}
%
\widehat{\bX}^{\text{lr}} = \sum^{k}_{\ell = 1} \hat{s}_\ell \hat{u}_{\ell} \hat{v}^T_{\ell}.
%
\end{align}
%
That is, $\widehat{\bX}^{\text{lr}}$ is a low-rank approximation of $\bZ$.
$\hbeta^{(a)}$ is then estimated by simply doing ordinary least squares (OLS) on $\bY$ and $\widehat{\bX}^{\text{lr}}$ as follows:
%
\begin{align}\label{eq:PCR_step2}
%
\hbeta^{(a)} = \Big(\widehat{\bX}^{\text{lr}})^{+} \bY.
%
\end{align}
%
Here $\Big(\widehat{\bX}^{\text{lr}})^{+}$ denotes the Moore-Penrose pseudoinverse of $\widehat{\bX}^{\text{lr}}$ defined as
%
\begin{align}
%
\Big(\widehat{\bX}^{\text{lr}})^{+} = \left( \sum^k_{\ell = 1}\frac{\hat{v}_{\ell} \hat{u}^T_{\ell}}{\hat{s}_\ell}  \right).
%
\end{align}
%
That is, PCR can be seen as doing ordinary least squares (OLS) on the best $k$-rank approximation of $\bZ$, given by $\Big(\widehat{\bX}^{\text{lr}})^{+}.$ If the ordinary least squares problem has multiple solutions, $\hbeta^{(a)}$ in equation \eqref{eq:PCR_step2} is the minimum $\ell_2$-norm solution \textcolor{teal}{[Need reference here]}.


\noindent
{\bf Interpreting PCR.}
%
Using Assumption \ref{assumption:holder.mech} and Definition \ref{def:linear_factor_approx}, we have that for all $n \in [N], t \in \bar{\Tc}$, 
%
\begin{align}\label{eq:PCR_remark_0}
%
Y_{n, t} 
%
= \ldot{\lambda_{n}}{\rho_{t, a_t}} 
%
+  \eta^{(a_t)}_{n, t} 
%
+ \varepsilon^{(a_t)}_{n, t}.
%
\end{align}
%
Hence, using \eqref{eq:PCR_remark_0} and the definitions of $\bY, \bZ, \bX, \bX^{\text{lr}}$, we have
%
\begin{align}
%
Y_{t}  
%
&= \sum_{n \in \Mc^{(1 - a)}} \left(\ldot{\lambda_{n}}{\rho_{t, a_t}} +  \eta^{(a_t)}_{n, t} + \varepsilon^{(a_t)}_{n, t} \right) 
%
\\ \bX^{\text{lr}}_{t, n} 
%
&= \ldot{\lambda_n}{\rho_{t, a_t}}  
%
\\ \bX_{t, n} 
%
&= \ldot{\lambda_n}{\rho_{t, a_t}} + \eta^{(a_t)}_{n, t} 
%
\\ \bZ_{t, n} 
%
&= \ldot{\lambda_n}{\rho_{t, a_t}} + \eta^{(a_t)}_{n, t} +\varepsilon^{(a_t)}_{n, t} 
%
\end{align}
%
By Assumption \ref{assumption:linear_span_inclusion}, we have 
$\lambda_{\Mc^{(1 - a)}}  = \sum_{n \in \Ic^{(a)}} \beta^{(a)}_{n} \lambda_n$.
%
Hence, we can write
%
\begin{align}
\bY &= \bX^{\text{lr}}\beta^{(a)}  
%
+ \phi^{\text{lr}} + \bar{\varepsilon} \label{eq:PCR_remark_1}
%
\\ \bX &= \bX^{\text{lr}} + \bE^{\text{lr}} \label{eq:PCR_remark_2}
%
\\ \bZ &= \bX + \bH \label{eq:PCR_remark_3}
%
\end{align}
%
where 
%
$\phi^{\text{lr}} = \left[\sum_{n \in \Mc^{(1 - a)}} \eta^{(a_t)}_{n, t} \right]_{t \in \bar{\Tc}} \ $, 
%
$\bar{\varepsilon} = \left[\sum_{n \in \Mc^{(1 - a)}} \varepsilon^{(a_t)}_{n, t} \right]_{t \in \bar{\Tc}} \ $, 
%
$\bE^{\text{lr}} = [\eta^{(a_t)}_{n, t}]_{t \in \bar{\Tc}, n \in \Ic^{(a)}} \ $, 
%
$\bH = [\varepsilon^{(a_t)}_{n, t}]_{t \in \bar{\Tc}, n \in \Ic^{(a)}}$.
%
Thus we have reduced our problem of estimating $\beta^{(a)}$ to that of linear regression where:
%
(i) the covariates are noisily observed (i.e., error-in-variables regression), i.e. \eqref{eq:PCR_remark_3} holds;
%
(ii) the noiseless covariate matrix has an approximate low-rank representation, i.e. \eqref{eq:PCR_remark_2} holds;
%
(ii) an approximate linear model holds between the approximate low-rank representation of the noiseless covariates and the response variable, i.e. \eqref{eq:PCR_remark_1} holds.

Hence, we can interpret PCR as follows:
%
(1) the first step of doing PCA given in \eqref{eq:PCR_step1} creates an estimate of the approximate low-rank approximation $\bX^{\text{lr}}$; 
%
(2) the second step of doing OLS given in \eqref{eq:PCR_step2} creates an estimate of $\beta^{(a)}$ by regressing $\bY$ on $\widehat{\bX}^{\text{lr}}$, which is motivated by \eqref{eq:PCR_remark_1}.

\subsection{Additional Assumptions for Estimation Results with PCR}
%
We make the following additional assumptions to state our consistency results. 
%
Note by Assumption \ref{assumption:holder.mech} and Proposition \ref{prop:factor_model_approx}, for all $\delta > 0$,
\[
\text{rank}(\bX^{\text{lr}}) := \bar{r} \le r \le C \cdot \delta^{-q}, \quad
\|\bX - \bX^{\text{lr}} \|_{\infty} = \Delta_E \le C_H \cdot \delta^S.
\]

\begin{remark}
Previewing our consistency results, we will pick $\delta = \left( \frac{1}{(\min(N_0, N_1, \bar{T})}\right)^{\frac{1}{2S}}$.
Then, $r \le C \min(N_0, N_1, \bar{T})^{\frac{q}{2S}}$ and $\Delta_E \le C_H \left(\frac{1}{(\min(N_0, N_1, \bar{T})}\right)^{\frac{1}{2}}.$
Hence, if $q < 2S$, then as $\min(N_0, N_1, \bar{T}) \to \infty$, $r \ll \min(N_0, N_1, \bar{T})$ and $\Delta_E = o(1)$.
\end{remark}

% \textcolor{teal}{
% It could be the case that $|\bar{\mathcal T}|<r$, right? But generally, do not we need the assumption that $|\bar{\mathcal T}|\geq r$?
% {\color{blue} Please see remark above}.
% }




\begin{assumption}[Well-balanced spectra.]\label{assumption:pcr_well_balanced}
%
Given the SVD of $\bX^{\text{lr}} = \sum^{\bar{r}}_{\ell = 1} s_\ell u_{\ell} v^T_{\ell},$ we have
%
\begin{align}
%
s_{\bar{r}} \ge C \sqrt{\frac{ \bar{T} N_a }{\bar{r}}}.   
%
\end{align}
%
\end{assumption}
%
An interpretation of Assumption \ref{assumption:pcr_well_balanced} is as follows.
%
Suppose that each entry of $\bX^{\text{lr}} \ge c > 0$, i.e. is bounded below by an absolute constant $c$.
%
Then since $\bX^{\text{lr}} \in \Rb^{\bar{T} \times N_a}$ we have that $\sum^{\bar{r}}_{\ell = 1} s^2_\ell = \| \bX^{\text{lr}} \|^2_F \ge C \bar{T} N_a$.
%
If all the singular values of $\bX^{\text{lr}}$ are of the same order of magnitude, i.e., $\frac{s_{\bar{r}}}{s_1} \ge C$, this immediately implies that $s_r \ge C \sqrt{\frac{ \bar{T} N_a }{\bar{r}}}$.

\begin{assumption}[Subspace inclusion.]\label{assumption:pcr_subspace}
%
For intervention $a \in \{0, 1\}$ and measurement $t$, $\Big[\ldot{\lambda_n}{\rho_{t^*, a}}\Big]_{n \in \Ic^{(a)}}$ lies in the rowspace of $\bX^{\text{lr}} = \Big[\ldot{\lambda_{n}}{\rho_{t, a_t}} \Big]_{t \in \bar{\Tc}, n \in \Ic^{(a)}}$.
%
\end{assumption}
%
Note a sufficient condition for Assumption 
\ref{assumption:pcr_subspace} is for $a \in \{0, 1\}$ 
%
\begin{align}
%
\rho_{t^*, a} \in \text{span}\{\rho_{t, a_t} \}_{t \in \bar{\Tc}}.
%
\end{align}
%
Hence, intuitively, we require that the target measurement $t^*$ for which we wish to compute $\mathsf{ATE}_{\Mc}$, the latent factors $\rho_{t^*, 0}, \rho_{t^*, 1}$, are linearly expressible in terms of the latent factors $\{\rho_{t, a_t} \}_{t \in \bar{\Tc}}$ corresponding to the measurements under which all units are under a common intervention.
%
This is the key condition that lets us {\em generalize} from the measurements $\bar{T}$ we learn on to the measurement $t^*$ we make counterfactual predictions on.

%
Below, we provide exact conditions if the linear estimator is PCR, the appropriateness of which was motivated in Section \ref{sec:ate_pcr}.

\subsection{Finite-sample Consistency using PCR}

{\color{blue} remove $N/T$ condition}


\begin{theorem}[ATT, ATU, ATE consistency using PCR]\label{thm:consistency_summary}
Let Assumptions \ref{assumption:conditonal_independence},
\ref{assumption:outcome_generating_function_factor_structure}, 
\ref{assumption:holder.mech} , \ref{assumption:linear_span_inclusion}, \ref{assumption:sub-gaussian_noise}, \ref{assumption:pcr_well_balanced}, and \ref{assumption:pcr_subspace} hold.
%
Let $\hbeta^{(a)}$ be estimated via PCR as in \eqref{eq:PCR_step1} and \eqref{eq:PCR_step2}.
%
Assume the following additional conditions hold.
%
\begin{enumerate}
%
\item Correct rank estimation for PCR: $k$ in \eqref{eq:PCR_step1} is such that $k = \bar{r}$.
%
\item Smooth outcome model: Let $\alpha = S / q > 0$, where recall $S$ is smoothness parameter of $g(U_n, \tilde{U}_{t, a})$ and $q$ is the latent dimension of $U_n$.  Assume $\alpha > 1.$
%
\item Disperse weights: For $a \in \{0, 1\}$, assume $\|\beta^{(a)}\|_2 = O\left( \frac{M_{1 - a}}{N^{w}_a} \right)$, where $\frac{1}{2\alpha} < w \le \frac{1}{2}$.
%
\item Growing common measurements, units: $\min(N_0, N_1, \bar{T}) \to \infty.$
%
\end{enumerate}
%
Then we have the following consistency results:

\begin{itemize}
%
\item {\bf $\mathsf{ATT}$ consistency:}
%
If $\frac{N_0^{1 - w}}{\bar{T}^{1 - \frac{1}{2 \alpha}}} = o(1)$, we have,
%
\begin{align}
%
\widehat{\mathsf{ATT}}  - \Ex[\mathsf{ATT} \mid \LF] &= o_p(1), \quad \widehat{\mathsf{ATT}}  - \mathsf{ATT} \mid \LF = o_p(1).
%
\end{align}
%
Further, we can take 
%
\begin{align}
%
r \le C \min(N_0, \bar{T})^{\frac{1}{2\alpha}}, \quad \Delta_E \le C \min(N_0, \bar{T})^{- \frac{1}{2}}.
%
\end{align}
%

\item {\bf $\mathsf{ATU}$ consistency:}
%
If $\frac{N_1^{1 - w}}{\bar{T}^{1 - \frac{1}{2 \alpha}}} = o(1)$, we have,
%
\begin{align}
%
\widehat{\mathsf{ATU}}  - \Ex[\mathsf{ATU} \mid \LF] &= o_p(1), \quad \widehat{\mathsf{ATU}}  - \mathsf{ATU} \mid \LF = o_p(1).
%
\end{align}
%
Further, we can take 
%
\begin{align}
%
r \le C \min(N_1, \bar{T})^{\frac{1}{2\alpha}}, \quad \Delta_E \le C \min(N_1, \bar{T})^{- \frac{1}{2}}.
%
\end{align}

\item {\bf $\mathsf{ATE}$ consistency:}
%
If $N_0, N_1 = \Theta(N)$, and $\frac{N^{1 - w}}{\bar{T}^{1 - \frac{1}{2 \alpha}}} = o(1)$, we have,
%
\begin{align}
%
\widehat{\mathsf{ATE}}  - \Ex[\mathsf{ATE} \mid \LF] &= o_p(1), \quad \widehat{\mathsf{ATE}}  - \mathsf{ATE} \mid \LF = o_p(1).
%
\end{align}
%
Further, we can take 
%
\begin{align}
%
r \le C \min(N, \bar{T})^{\frac{1}{2\alpha}}, \quad \Delta_E \le C \min(N, \bar{T})^{- \frac{1}{2}}.
%
\end{align}

\end{itemize}
%
\end{theorem}

\begin{proposition}\label{prop:beta_norm}
%
Assume for every set $\Ic \subset [N]$ where $|\Ic| = N^{\theta}$, with $0 < \theta < 1 -  \frac{3}{2\alpha}$, there exists a subset $\tilde{\Ic}$, where $|\tilde{\Ic}| = r$ and $\text{span}\{ \lambda_n\}_{j \in \tilde{\Ic}} = \Rb^r$.
%
Assume $r \le C\min(N_a, \bar{T})^{\frac{1}{2\alpha}}$.
%
Then the minimum $\ell_2$-norm $\beta^{(a)}$ is such that $\|\beta^{(a)}\|_2 =o\left(\frac{M_{1 - a}}{N_{a}^{{\frac{1}{2\alpha}}}}\right)$.
%
That is, the property, $\frac{1}{2 \alpha} < w$, in Condition 3 of Theorem \ref{thm:consistency_summary} holds.
%
\end{proposition}


\subsection{Asymptotic Normality using PCR}

\begin{theorem}[$\mathsf{ATT}$ and $\mathsf{ATU}$ Normality using PCR]\label{thm:att_atu_normality_PCR}
%
Let the conditions of Theorem \ref{thm:consistency_summary} hold.
%
Assume the following additional conditions hold.
%
\begin{enumerate}
%
\item $\frac{1}{C} \sqrt{M} \le \bar{\sigma}.$ 
%
\item The following inequalities hold $xxx.$
%
\end{enumerate}
%
Then we have the following asymptotic normality results:

\begin{itemize}
%
\item {\bf $\mathsf{ATT}$ asymptotic normality:}
%
If $N_1 = o(\min(N_0, \bar{T}))$, we have,
%
\begin{align}
%
\frac{M}{\bar{\sigma}} \left( \widehat{\mathsf{ATT}}  - \Ex[\mathsf{ATT}_{\Mc} \mid \LF] \right) &\to \Nc(0, 1).
%
\end{align}
%

\item {\bf $\mathsf{ATU}$ consistency:}
%
If $N_0 = o(\min(N_1, \bar{T}))$, we have,, we have,
%
\begin{align}
%
\frac{M}{\bar{\sigma}} \left( \widehat{\mathsf{ATU}} - \Ex[\mathsf{ATU}_{\Mc} \mid \LF] \right) &\to \Nc(0, 1).
%
\end{align}
%
\end{itemize}
%
\end{theorem}





==> Old/proofs/beta_norm.tex <==




% {\bf Setting 1}

% %
% Let $\boldsymbol{\varepsilon} \in \Rb^N$ be a vector of standard Gaussians.
% %
% For $j \in [N]$, let $\beta^j \in \Rb^N$ be a vector of coefficients.
% %
% Note, 
% %
% \begin{align}
% %
% \Ex[\ldot{\beta^j}{\boldsymbol{\varepsilon}}] = 0,  
% %
% \quad \Var(\ldot{\beta^j}{\boldsymbol{\varepsilon}}) = \| \beta^j \|^2_2
% %
% \end{align}
% %
% Then,
% %
% \begin{align}
% %
% \frac{1}{N}\sum^{N}_{j = 1} \ldot{\beta^j}{\boldsymbol{\varepsilon}} 
% %
% = \ldot{\frac{1}{N}\sum^{N}_{j = 1}\beta^j}{\boldsymbol{\varepsilon}}
% %
% = \Theta_p\left(\left\| \frac{1}{N}\sum^{N}_{j = 1}\beta^j \right\|_2\right)
% %
% \end{align}
% %
% $\ldot{\beta^j}{\boldsymbol{\varepsilon}}$ concentrates around $\| \beta^j \|_2$, but $\frac{1}{N}\sum^{N}_{j = 1} \ldot{\beta^j}{\boldsymbol{\varepsilon}}$ does not concentrate as $\ldot{\beta^{j_1}}{\boldsymbol{\varepsilon}}, \ldot{\beta^{j_2}}{\boldsymbol{\varepsilon}}$ are strongly correlated.

% {\color{blue}
% \vspace{2mm}
% \noindent
% {\bf Setting 1b}
% \vspace{2mm}

% Assume for every set $\Ic \subset [N]$ with $|\Ic| = N^{\delta}$, $\delta \in (0, 1]$ there exists a subset $\tilde{\Ic}$, where $|\tilde{\Ic}| = r$ and $\text{span}\{ \lambda_j\}_{j \in \tilde{\Ic}} = \Rb^r$.
% %
% Hence for $c \in [N^{1 - \delta}]$ there exists $\beta^{j, c} \in \Rb^{N^{\delta}}$ such that
% %
% \begin{align}
%   \lambda_j = \sum^{c N^\delta}_{i = 1 + (c - 1)N^\delta} \beta^{j, c}_i \lambda_i
% \end{align}
% and 
% \begin{align}
%   \| \beta^{j, c} \|_2 = O(r).
% \end{align}
% Define $\tilde{\beta}^j \in \Rb^N$ as follows
% \begin{align}
%  \tilde{\beta}^j = \frac{1}{N^{1 - \delta}}[\beta^{j, 1}, \dots, \beta^{j, N^{1 - \delta}}]
% \end{align}
% %
% Note
% \begin{align}
%     \lambda_j = \sum^N_{i = 1} \tilde{\beta}^j_i \lambda_i
% \end{align}
% Further observe
% \begin{align}
%     \| \tilde{\beta}^j \|_2 = O\left( \frac{r}{N^{\frac{1 - \delta}{2}}} \right)
% \end{align}
% Then,
% %
% \begin{align}
% %
% \frac{1}{N}\sum^{N}_{j = 1} \ldot{\tilde{\beta}^j}{\boldsymbol{\varepsilon}} 
% %
% = \ldot{\frac{1}{N}\sum^{N}_{j = 1}\tilde{\beta}^j}{\boldsymbol{\varepsilon}}
% %
% = O_p\left(\left\| \frac{1}{N}\sum^{N}_{j = 1}\tilde{\beta}^j \right\|_2\right)
% %
% = O_p\left( \frac{r}{N^{\frac{1 - \delta}{2}}} \right)
% %
% \end{align}
% }


% \vspace{2mm}
% \noindent
% {\bf Setting 2}
% \vspace{2mm}

% %
% For $t \in [T]$, $\boldsymbol{\varepsilon}^t \in \Rb^T$ be a vector of standard Gaussians.
% %
% Let $\beta \in \Rb^T$ be a vector of coefficients.
% %
% Note, for $t \in [T]$
% %
% \begin{align}
% %
% \Ex[\ldot{\beta}{\boldsymbol{\varepsilon}^t}] = 0,  
% %
% \quad \Var(\ldot{\beta}{\boldsymbol{\varepsilon}^t}) = \| \beta \|^2_2
% %
% \end{align}
% %
% Then,
% %
% \begin{align}
% %
% \frac{1}{T}\sum^{T}_{t = 1} \ldot{\beta}{\boldsymbol{\varepsilon}^t} = \Theta_p\left( \frac{\| \beta \|_2}{\sqrt{T}} \right)
% %
% \end{align}
% %
% This is because $\ldot{\beta}{\boldsymbol{\varepsilon}^{t_1}}$, $\ldot{\beta}{\boldsymbol{\varepsilon}^{t_2}}$ are independent and their sum concentrates.

% {\color{blue}
% If $\|\beta^j \|_0 = O(r)$,  then it is reasonable that $\|\beta^j \|_2 = O(r)$.
% %
% Hence,
% %
% \begin{align}
%     \|\frac{1}{N} \beta^j \|_2 \to 0 
% \end{align}
% %
% However,
% \begin{align}
%     \|\frac{1}{N} \sum^N_{j = 1}\beta^j \|_2 \not\to 0
% \end{align}
% }

==> Old/proofs/proofs_ate_consistency.tex <==
\section{ATE: Identification Proofs}
%
\subsection{Proof of Theorem \ref{thm:ate_idenfication}}
%
From Assumptions \ref{assumption:conditonal_independence} and \ref{assumption:outcome_generating_function_factor_structure}, we have that for $a \in \{0, 1\},$
%
\begin{align}
%
\sum_{n \in \Mc} \Ex[Y^{(a)}_{n, t^*} \mid \LF]
%
&= \sum_{n \in \Mc^{(a)}} \Ex[Y^{(a)}_{n, t^*} \mid \LF] + \sum_{n \in \Mc^{(1 - a)}} \Ex[Y^{(a)}_{n, t^*} \mid \LF]\\
%
&= \sum_{n \in \Mc^{(a)}} \Ex[Y^{(a)}_{n, t^*} \mid \bA, \LF] + \sum_{n \in \Mc^{(1 - a)}} \Ex[Y^{(a)}_{n, t^*} \mid \LF]
%
\\&= \sum_{n \in \Mc^{(a)}} \Ex[Y_{n, t^*} \mid \bA, \LF] + \sum_{n \in \Mc^{(1 - a)}} \Ex[Y^{(a)}_{n, t^*} \mid \LF]. \label{eq:ate_id_1}
%
\end{align}
%
What remains to be tackled is the second term in \eqref{eq:ate_id_1}.
%
Assumptions \ref{assumption:conditonal_independence} and \ref{assumption:outcome_generating_function_factor_structure}, and
Definition \ref{def:linear_factor_approx} implies $Y^{(a)}_{n, t^*} = \ldot{\lambda_n}{\rho_{t^*, a}} + \eta^{(a)}_{n, t^*} + \varepsilon^{(a)}_{n, t^*}$, where $\Ex[\varepsilon^{(a)}_{n, t^*} \mid \LF] = 0$.
%
Hence, from Assumption \ref{assumption:linear_span_inclusion},
%
\begin{align}
%
\sum_{n \in \Mc^{(1 - a)}} \Ex[Y^{(a)}_{n, t^*} \mid \LF]
%
&= \sum_{n \in \Mc^{(1 - a)}} 
\left(\ldot{\lambda_n}{\rho_{t^*, a}} + \eta^{(a)}_{n, t^*}\right)
%
\nonumber\\ &= \ldot{\lambda_{\Mc^{(1 - a)}}}{\rho_{t^*, a}}  + \sum_{n \in \Mc^{(1-a)}} \eta^{(a)}_{n, t^*}\nonumber\\
&= \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n  \ldot{\lambda_n}{\rho_{t^*, a}}  + \sum_{n \in \Mc^{(1-a)}} \eta^{(a)}_{n, t^*}
%
\label{eq:ate_id_2}
\end{align}
%
where in the last line we have used the definition of $\lambda_{\Mc^{(1 - a)}}$.

%
In addition,
%
\begin{align}
%
\sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \ldot{  \lambda_n}{\rho_{t^*, a}}
%
% &= \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \ldot{  \lambda_n}{\rho_{t^*, a}} \pm \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \eta^{(a)}_{n, t^*} 
% %
% + \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \Ex\left[\varepsilon^{(a)}_{n, t^*} \mid \bA, \LF\right]
% %
%\\ 
&= 
\sum_{n \in\Ic^{(a)}} \beta^{(a)}_n \Ex\left[Y^{(a)}_{n, t^*} \mid \LF\right]
%
- \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \eta^{(a)}_{n, t^*}\nonumber\\
&=\sum_{n \in\Ic^{(a)}} \beta^{(a)}_n \Ex\left[Y_{n, t^*} \mid \bA, \LF\right]
%
- \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \eta^{(a)}_{n, t^*}.
\label{eq:ate_id_3}
%
\end{align}
%


Combining \eqref{eq:ate_id_1}, \eqref{eq:ate_id_2}, and \eqref{eq:ate_id_3}, we conclude the proof. 
%

% %
% From Assumption \ref{assumption:basic_model}, we have that for $a \in \{0, 1\},$
% %
% \begin{align}
% %
% \sum_{n \in \Mc} \Ex[Y^{(a)}_{n, t^*} \mid \LF]
% %
% &= \sum_{n \in \Mc} \Ex[Y^{(a)}_{n, t^*} \mid \bA, \LF]
% %
% \\&= \sum_{n \in \Mc^{(a)}} \Ex[Y^{(a)}_{n, t^*} \mid \bA, \LF] + \sum_{n \in \Mc^{(1 - a)}} \Ex[Y^{(a)}_{n, t^*} \mid \bA, \LF]
% %
% \\&= \sum_{n \in \Mc^{(a)}} \Ex[Y_{n, t^*} \mid \bA, \LF] + \sum_{n \in \Mc^{(1 - a)}} \Ex[Y^{(a)}_{n, t^*} \mid \bA, \LF]. \label{eq:ate_id_1}
% %
% \end{align}
% %
% What remains to be tackled is the second term in \eqref{eq:ate_id_1}.
% %
% %Assumptions \ref{assumption:basic_model}, \ref{assumption:LVM_model} and and 
% Definition \ref{def:linear_factor_approx} implies $Y^{(a)}_{n, t^*} = \ldot{\lambda_n}{\rho_{t^*, a}} + \eta^{(a)}_{n, t^*} + \varepsilon^{(a)}_{n, t^*}$, where $\Ex[\varepsilon^{(a)}_{n, t^*} \mid \bA, \LF] = 0$.
% %
% Hence,
% %
% \begin{align}
% %
% \sum_{n \in \Mc^{(1 - a)}} \Ex[Y^{(a)}_{n, t^*} \mid \bA, \LF]
% %
% &= \sum_{n \in \Mc^{(1 - a)}} 
% \left(\ldot{\lambda_n}{\rho_{t^*, a}} + \eta^{(a)}_{n, t^*}\right)
% %
% \nonumber\\ &= \ldot{\lambda_{\Mc^{(1 - a)}}}{\rho_{t^*, a}}  + \sum_{n \in \Mc^{(1-a)}} \eta^{(a)}_{n, t^*}.
% %
% \label{eq:ate_id_2}
% \end{align}
% %
% where in the last line we have used the definition of $\lambda_{\Mc^{(1 - a)}}$.

% %
% From Assumption \ref{assumption:linear_span_inclusion},
% %
% \begin{align*}
% %
% \ldot{\lambda_{\Mc^{(1 - a)}}}{\rho_{t^*, a}}
% &= \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n  \ldot{\lambda_n}{\rho_{t^*, a}}.
% %
% \end{align*}
% %
% Therefore, 
% %
% \begin{align}
% %
% \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \ldot{  \lambda_n}{\rho_{t^*, a}}
% %
% % &= \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \ldot{  \lambda_n}{\rho_{t^*, a}} \pm \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \eta^{(a)}_{n, t^*} 
% % %
% % + \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \Ex\left[\varepsilon^{(a)}_{n, t^*} \mid \bA, \LF\right]
% % %
% %\\ 
% &= 
% \sum_{n \in\Ic^{(a)}} \beta^{(a)}_n \Ex\left[Y_{n, t^*} \mid \bA, \LF\right]
% %
% - \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \eta^{(a)}_{n, t^*}.
% \label{eq:ate_id_3}
% %
% \end{align}
% %


% Combining \eqref{eq:ate_id_1}, \eqref{eq:ate_id_2}, and \eqref{eq:ate_id_3}, we conclude the proof. 
% %



\subsection{Proof of Corollary \ref{cor:ate_identification}.}
%
Using Theorem \ref{thm:ate_idenfication}, we have 
%
\begin{align}
%
\Big| \Ex[\mathsf{ATE}_{\mathcal{M}} \mid \LF] - \mathsf{Observed} \Big| 
%
&\le  \frac{1}{M} \left(\left| \sum_{j \in \Mc^{(0)}} \eta^{(1)}_{n, t^*}\right|
%
+ \left| \sum_{j \in \Ic^{(1)}} \beta^{(1)}_j \eta^{(1)}_{n, t^*}\right|
%
+ \left| \sum_{j \in \Mc^{(1)}} \eta^{(0)}_{n, t^*}\right|
%
+ \left| \sum_{j \in \Ic^{(0)}} \beta^{(0)}_j \eta^{(0)}_{n, t^*}\right|\right) \label{eq:ate_identification_cor_1}
%
\\&\le  \Delta_E \left(1 + \frac{\| \beta^{(0)}\|_1 + \| \beta^{(1)}\|_1}{M} \right). \label{eq:ate_identification_cor_2}
%
\end{align}

% \subsection{Proofs of Propositions \ref{prop:pcr_est} and \ref{prop:pcr_est_proj}}

\section{ATE: Estimation Proofs}

\subsection{Proof of Proposition \ref{prop:ate_estimation}.}

We recall notation required for the proofs of this section.
%
Let $\varepsilon_{\Ic^{(a)}} \coloneqq [\varepsilon^{(a)}_{n, t^*}]_{n \in \Ic^{(a)}}$, $Y_{\Ic^{(a)}} \coloneqq [Y_{n, t^*}]_{n \in \Ic^{(a)}}$.
%
%For simplicity, we suppress the conditioning on $\bA, \LF$ in the remainder of the proof.

From Corollary \ref{cor:ate_identification} and the definition of a linear estimator in \eqref{eq:ATE_synthetic_estiamtor}, we have that
%
\begin{align}
%
|&\widehat{\mathsf{ATE}}_{\Mc}-\Ex\left[\mathsf{ATE}_{\Mc} \mid \LF \right] | \\
%
&\le  \Delta_E \left(1 + \frac{\| \beta^{(0)}\|_1 + \| \beta^{(1)}\|_1}{M} \right)\\
%
 &+ \sum_{a \in \{0, 1\}} \left| \frac{1}{M}\left(\sum_{n \in \Mc^{(a)}} \Ex[Y_{n, t^*}\mid \bA, \LF] 
%
+ \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \Ex\left[ Y_{n, t^*} \mid \bA, \LF \right]\right)
%
- \frac{1}{M} \left(\sum_{n \in \Ic^{(a)}} Y_{n, t^*} 
%
+ \sum_{n \in \Ic^{(a)}} \hbeta^{(a)}_j Y_{n, t^*} \right) \right|.\label{eq:ate_est_target}
%
\end{align}
%
From \eqref{eq:ate_est_target}, it suffices to bound the following terms for $a \in \{0, 1\}$, 
%
\begin{align}
%
\left| \frac{1}{M} \left(\sum_{n \in \Mc^{(a)}} Y_{n, t^*} \right)  
%
- \frac{1}{M}\left(\sum_{n \in \Mc^{(a)}} \Ex[Y_{n, t^*} \mid \bA, \LF ] \right) \right|, \label{eq:ate_est_target_2.1}
%
\\ \left| \frac{1}{M} \left(\sum_{n \in \Ic^{(a)}} \hbeta^{(a)}_n Y_{n, t^*} \right)  
%
- \frac{1}{M}\left(\sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \Ex\left[ Y_{n, t^*} \mid \bA, \LF \right]\right) \right|.\label{eq:ate_est_target_3}
%
\end{align}

{\em Bounding \eqref{eq:ate_est_target_2.1}.}
%

Using Assumptions \ref{assumption:conditonal_independence} and \ref{assumption:outcome_generating_function_factor_structure},
%
\begin{align}\label{eq:ate_est_target_4}
%
\frac{1}{M} \left(\sum_{n \in \Mc^{(a)}} Y_{n, t^*} \right) 
%
- \frac{1}{M}\left(\sum_{n \in \Mc^{(a)}} \Ex[Y_{n, t^*}  \mid \bA, \LF] \right) 
%
&= \frac{1}{M} \left(\sum_{n \in \Mc^{(a)}} \varepsilon^{(a)}_{n, t^*} \right)
%
\end{align}

We now apply Hoeffding's inequality, which we restate next.
%
\begin{lemma}[Hoeffding's inequality, e.g., \citeauthor{vershynin_2018}, \citeyear{vershynin_2018}]\label{lemma:hoeffdings}
%
Let $X_1, \dots, X_N$ be independent mean zero sub-Gaussian random variables, and $a = (a_1, \dots, a_N) \in \Rb^N$.
%
Then, for every $t \ge 0,$ we have
%
\begin{align}
%
\Pb\left( \left| \sum^N_{n = 1} a_n X_n \right| \ge t \right) \le 2 \exp\left( - \frac{Ct^2}{K^2 \|a \|_2^2}\right)
%
\end{align}
%
where $K = \max \{\| X_n \|_{\psi_2}\}_{n=1}^N$.
\end{lemma}


%
Using Assumptions \ref{assumption:conditonal_independence}, \ref{assumption:outcome_generating_function_factor_structure}, and \ref{assumption:sub-gaussian_noise}, and applying Hoeffding's inequality from Lemma \ref{lemma:hoeffdings} (with $X_n =  \varepsilon^{(a)}_{n, t^*}$, $a_n = 1$, $K = \sigma_{\max}, t = \sigma_{\max}\sqrt{M_a}$), we have that \eqref{eq:ate_est_target_4} is bounded by
%
\begin{align}
%
\frac{1}{M} \left(\sum_{n \in \Mc^{(a)}} \varepsilon^{(a)}_{n, t} \right) 
%
= O_p\left(  \frac{ \sigma_\max \sqrt{M_a} }{M}\right) \label{eq:ate_est_final_1}
%
\end{align}
%

{\em Bounding \eqref{eq:ate_est_target_3}.}

Using the definition of $\Delta_{\beta^{(a)}}$ we have
%
\begin{align}
%
&\frac{1}{M} \left(\sum_{n \in \Ic^{(a)}} \hbeta^{(a)}_n Y_{n, t^*} \right)  
%
- \frac{1}{M}\left(\sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \Ex\left[ Y_{n, t^*}  \mid \bA, \LF \right]\right) 
%
\\&= \frac{1}{M}\left(
%
\ldot{\beta^{(a)}}{\ \varepsilon_{\Ic^{(a)}} }  
%
+ \ldot{\Delta_{\beta^{(a)}}}{\ \varepsilon_{\Ic^{(a)}} } 
%
+ \ldot{\Delta_{\beta^{(a)}}}{\ \Ex\left[ Y_{\Ic^{(a)}} \mid \bA, \LF \right]} \right) \label{eq:ate_est_target_5}
%
\end{align}
%
We consider each term in \eqref{eq:ate_est_target_5} separately.

%
\noindent{\em Term 1 of \eqref{eq:ate_est_target_5}.}
%
\begin{align}
%
\frac{1}{M}\ldot{\beta^{(a)}}{\ \varepsilon_{\Ic^{(a)}} }
% %
% &= \frac{C_a}{N_a}\ldot{\beta^{(a)}}{\ \varepsilon_{\Ic^{(a)}} \mid \bA,\LF} 
%
= O_p\left(\frac{\sigma_\max\|\beta^{(a)} \|_2}{M}\right) \label{eq:ate_est_final_2}
%
\end{align}
%
where the last equality follows from Assumptions \ref{assumption:conditonal_independence}, \ref{assumption:outcome_generating_function_factor_structure}, and \ref{assumption:sub-gaussian_noise}, and using Lemma \ref{lemma:hoeffdings}.
%

\noindent{\em Term 2 of \eqref{eq:ate_est_target_5}.}
%
\begin{align}
%
&\frac{1}{M}\ldot{\Delta_{\beta^{(a)}}}{\ \varepsilon_{\Ic^{(a)}}}
%
= O_p\left( \frac{\sigma_\max\|\Delta_{\beta^{(a)}}\|_2 }{M}\right) \label{eq:ate_est_final_3}
%
\end{align}
%
where the last equality follows from Assumptions \ref{assumption:conditonal_independence}, \ref{assumption:outcome_generating_function_factor_structure}, and \ref{assumption:sub-gaussian_noise}, and using Lemma \ref{lemma:hoeffdings}.


\noindent{\em Collecting terms.}

%
Combining the bounds in \eqref{eq:ate_est_target}, \eqref{eq:ate_est_final_1}, \eqref{eq:ate_est_target_5}, \eqref{eq:ate_est_final_2}, \eqref{eq:ate_est_final_3} we have that
%
\begin{align}
%
\widehat{\mathsf{ATE}}_{\Mc} - \Ex\left[\mathsf{ATE}_{\Mc}  \right] 
%
&\le  \Delta_E \left(1 + \frac{\| \beta^{(0)}\|_1 + \| \beta^{(1)}\|_1}{M} \right)\\ 
%
&+ O_p\left( \sum_{a \in \{0, 1\}} \frac{\sigma_\max \left(\sqrt{M_a} +  \|\beta^{(a)} \|_2 + \|\Delta_{\beta^{(a)}}\|_2\right) +  \ldot{\Delta_{\beta^{(a)}}  }{\Ex\left[ Y_{\Ic^{(a)}} \right]}}{M} \right) \label{eq:ate_est_final_5}
%
\end{align}
%
Simplifying \eqref{eq:ate_est_final_5} completes the proof.
%

\subsection{Proof of Corollary \ref{cor:ate_estimation}.}
%
For simplicity, we suppress the conditioning on $\LF$ in the remainder of the proof.
%
Given Proposition \ref{prop:ate_estimation}, it suffices to bound $\textsf{ATE}_{\Mc} - \Ex[\textsf{ATE}_{\Mc}]$.
%
\begin{align}
%
\mathsf{ATE}_{\Mc} - \Ex\left[\mathsf{ATE}_{\Mc}  \right] 
%
&= \left(\frac{1}{M}\sum_{n \in \Mc} Y^{(1)}_{n, t^*} - Y^{(0)}_{n, t^*}   \right)
%
- \left(\frac{1}{M}\sum_{n \in \Mc} \Ex[Y^{(1)}_{n, t^*} - Y^{(0)}_{n, t^*} \mid \bA, \LF ] \right)
%
\\ &= \frac{1}{M}\sum_{n \in \Mc} \varepsilon^{(1)}_{n, t^*} - \varepsilon^{(0)}_{n, t^*} \label{eq:ate_cor_1}
%
\end{align}
%
Applying Hoeffding's inequality from Lemma \ref{lemma:hoeffdings}, we have that \eqref{eq:ate_cor_1} is bounded as
%
\begin{align}
%
\frac{1}{M}\sum_{n \in \Mc} \varepsilon^{(1)}_{n, t^*} - \varepsilon^{(0)}_{n, t^*} 
%
= O_p\left(\frac{\sigma_\max}{\sqrt{M}}\right) \label{eq:ate_cor_2}
%
\end{align}
%
Noticing that $\frac{\sigma_\max}{\sqrt{M}}$ is bounded above by $\mathsf{Bound}$ as defined in the statement of the corollary, and using the result of Proposition \ref{prop:ate_estimation} completes the proof.

\subsection{Proof of Theorem \ref{thm:consistency_summary}.}

\vspace{2mm}
\subsubsection{Bounding linear parameter estimation error of PCR.}

We first state and prove two key propositions required to establish Theorem \ref{thm:consistency_summary} that bound $\Delta_{\beta^{(a)}}$.

\begin{proposition}\label{prop:pcr_est}
Let the conditions of Theorem \ref{thm:ate_idenfication}, and Assumptions  \ref{assumption:sub-gaussian_noise}, \ref{assumption:pcr_well_balanced} hold.
Suppose we estimate $\hbeta^{(a)}$ via PCR (i.e., \eqref{eq:PCR_step1} and  \eqref{eq:PCR_step2}) and $k = \bar{r}$.
Then with probability $1 - O((N_a \bar{T})^{-10})$
\begin{align}
%
\|\Delta_{\beta^{(a)}}\|_2 \le 
%
C \cdot \sigma_\max^3 \cdot \ln^3(\bar{T} N_a) \cdot \left[\left\| \beta^{(a)} \right\|_2 \cdot \left( \frac{r}{\min(\sqrt{\bar{T}}, \sqrt{N_a})} + r \Delta_E \right) + \frac{M_{1-a} \sqrt{r} \Delta_E}{\sqrt{N_a}} \right].
\end{align}
\end{proposition}

\noindent
{\bf Proof of Proposition \ref{prop:pcr_est}.}
%

\begin{table}[h]
\centering
\begin{tabular}{||c c||} 
\hline
Notation of \cite{agarwal2021causal} & Our Notation \\ [1ex] 
\hline
$\bY$ & $\frac{\bY}{M_{1-a}}$  \\ [1ex]
\hline
$\bX$ & $\bX$ \\  [1ex]
\hline
$\bZ$ &  $\bZ$  \\ [1ex]
\hline
$\bX^{(lr)}$ &  $\bX^{lr}$  \\ [1ex]
\hline 
$n$ & $\bar{T}$ \\
\hline 
$p$ & $N_a$ \\
\hline 
$\bbeta^*$ & $\frac{\beta^{(a)}}{M_{1-a}}$ \\
\hline
$\hat{\bbeta}$ & $\frac{\hbeta^{(a)}}{M_{1-a}}$ \\
\hline
$\Delta_E$ & $\Delta_E$ \\
\hline 
$r$ & $\bar{r} \ (\le r)$ \\
\hline 
$\phi^{(lr)}$ & $\frac{\phi^{lr}}{M_{1-a}}$ \\ [1ex]
\hline
$\varepsilon$ & $\frac{\bar{\varepsilon}}{M_{1-a}}$ \\ [1ex]
\hline
$\Bar{A}$ & $C$ \\ 
\hline
$\Bar{K}$ & 0  \\ [1ex] 
\hline
$K_{a}, \kappa, \Bar{\sigma}$ & $C\sigma_{\max}$ \\
\hline 
$\rho_{min}$ & 1 \\
\hline 
\end{tabular}
\caption{A summary of the main notational differences between our setting and that of \cite{agarwal2021causal}.}
\label{tab:notational_changes}
\end{table}

Using \eqref{eq:PCR_remark_0}, \eqref{eq:PCR_remark_1}, \eqref{eq:PCR_remark_2}, and \eqref{eq:PCR_remark_3}, we have reduced our problem of estimating $\beta^{\Ic_t^{(a)}}$ to that of linear regression where:
%
(i) the covariates are noisily observed (i.e., error-in-variables regression), i.e. \eqref{eq:PCR_remark_3} holds;
%
(ii) the noiseless covariate matrix has an approximate low-rank representation, i.e. \eqref{eq:PCR_remark_2} holds;
%
(ii) an approximate linear model holds between the approximate low-rank representation of the noiseless covariates and the response variable, i.e. \eqref{eq:PCR_remark_1} holds.
%
We observe that bounding $\|\Delta_{\beta^{(a)}}\|_2 $ in such a setting is exactly the setup considered in Proposition E.3 of \cite{agarwal2021causal}, where they also analyze PCR.
%
We match notation with that of \cite{agarwal2021causal} as seen in Table \ref{tab:notational_changes}.
%
We then get
%
\begin{align}
%
\left\|\frac{\Delta_{\beta^{(a)}}}{M_{1 - a}}\right\|_2 
%
&\le  C \cdot (\sigma_\max)(2\sigma_\max) \cdot \sigma_\max \cdot \ln^3(\bar{T} N_a) \cdot \sqrt{r} \cdot \left( \frac{\|\phi^{\text{lr}}\|_2}{\sqrt{N_a \bar{T}}} + \sqrt{r} \cdot \left\| \frac{\beta^{(a)}}{M_{1 - a}} \right\|_2 \cdot \left( \frac{1}{\sqrt{\bar{T}}} + \frac{1}{\sqrt{N_a}} +  \Delta_E \right)\right) \label{eq:PCR_proof_4}
%
\end{align}
%
Using $\|\phi^{\text{lr}}\|_2  \le \Delta_E \sqrt{\bar{T}}$ and simplifying \eqref{eq:PCR_proof_4} completes the proof
%

\begin{proposition}\label{prop:pcr_est_proj}
%
Let the conditions of Proposition \ref{prop:pcr_est} hold.
%
Let $\mathsf{Proj}$ be the projection operator onto the rowspace of $\bX^{\text{lr}}$, i.e., $\mathsf{Proj} = \bV_r \bV_r^T$, where $\bV_r$ are the right singular vectors of $\bX^{\text{lr}}$.
%
Then with probability $1 - O((N_a \bar{T})^{-10})$
\begin{align}
%
&\|\mathsf{Proj}(\Delta_{\beta^{(a)}})\|_2 \ \le
%
\\&  
%
\quad C \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot 
%
\left\{ \left\| \beta^{(a)} \right\|_2 \cdot \left( \frac{r^{3/2}}{\min(\bar{T}, N_a)} + \frac{r^{3/2} \Delta_E}{\min(\sqrt{\bar{T}}, \sqrt{N_a})} + r^{3/2} \Delta^2_E \right) \right\},
%
\\& + C \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot  \left\{ \left\| \beta^{(a)} \right\|_1 \cdot \left( \frac{\sqrt{r}}{\left\| \frac{\beta^{(a)}}{M_{1 - a}} \right\|^{1/2}_1 \bar{T}^{\frac{1}{4}} \sqrt{N_a}} +
\frac{r}{\min(\bar{T}, N_a)} 
+ \frac{r \Delta_E}{\sqrt{N_a}} \right)
%
\right\},
\\& + C \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot M_{1-a} \cdot \left\{\frac{\sqrt{r} \Delta_E}{\sqrt{N_a}} + \frac{r \Delta^2_E}{\sqrt{N_a}} \right\}.
%
\end{align}
%
\end{proposition}

\noindent
{\bf Proof of Proposition \ref{prop:pcr_est_proj}.}
As in the proof of Proposition \ref{prop:pcr_est}, we use \eqref{eq:PCR_remark_1}, \eqref{eq:PCR_remark_2}, \eqref{eq:PCR_remark_3} and observe that bounding $\|\textsf{Proj}(\Delta_{\beta^{(a)}})\|_2$ in such a setting is exactly the setup considered in Corollary E.1 of \cite{agarwal2021causal}, where they also analyze PCR.
%
Matching notation with that of \cite{agarwal2021causal},
%
\footnote{
%
The additional notation compared to Proposition \ref{prop:pcr_est} that needs to be matched here is $\bV_r \bV^T_r = \textsf{Proj}(\cdot)$, where $\bV_r \bV^T_r$ is the notation used in \cite{agarwal2021causal}.
%
}
we get
%
\begin{align}
%
\left\|\frac{\textsf{Proj}(\Delta_{\beta^{(a)}})}{M_{1-a}} \right\|_2 
%
&\le  C \cdot (\sigma_\max)(2\sigma_\max)^2 \cdot \sigma_\max \cdot \ln^{9/2}(\bar{T} N_a) \cdot \sqrt{r} \cdot \Big[ (A) + (B) + (C)\Big]
%
\end{align}
%
where
%
\begin{align}
%
(A) &\coloneqq \frac{1}{\sqrt{\bar{T}}} \| \phi^{\text{lr}} \|_2 \left( \frac{1}{\sqrt{N_a}} + \frac{\sqrt{r}}{N_a} + \frac{\sqrt{r}}{\sqrt{\bar{T} N_a}} + \frac{\sqrt{r}}{\sqrt{N_a}} \Delta_E  \right)
%
\\ (B) &\coloneqq  \left\| \frac{\beta^{(a)}}{M_{1 - a}} \right\|_1 \left( \frac{\bar{T}^{1/4}}{\left\| \frac{\beta^{(a)}}{M_{1 - a}} \right\|^{1/2}_1 \sqrt{\bar{T} N_a}} +
\frac{\sqrt{r}}{\sqrt{\bar{T} N_a}} +
\frac{\sqrt{r}}{N_a}+
\frac{\sqrt{r}}{\sqrt{N_a}} \Delta_E  \right)
%
\\ (C) &\coloneqq \left\| \frac{\beta^{(a)}}{M_{1 - a}} \right\|_2 \cdot r \cdot \left( 
\frac{1}{\bar{T}} +
\frac{1}{N_a} +
\frac{1}{\sqrt{\bar{T} N_a}} +
\left( \frac{1}{\sqrt{\bar{T}}} + \frac{1}{\sqrt{N_a}} \right) \Delta_E  +
\Delta^2_E  \right)
%
\end{align}
%

Using $\|\phi^{\text{lr}}\|_2 \le \sqrt{\bar{T}}\Delta_E$ and $r \le \min(N_a, \bar{T})$, we have 
%
\begin{align}
%
(A) &\le \frac{\Delta_E}{\sqrt{N_a}} + \frac{\sqrt{r} \Delta^2_E}{\sqrt{N_a}}.
%
\end{align}
Simplifying (B) and (C), we have
\begin{align}
(B) &\le \left\| \frac{\beta^{(a)}}{M_{1 - a}} \right\|_1 \left( \frac{1}{\left\| \frac{\beta^{(a)}}{M_{1 - a}} \right\|^{1/2}_1 \bar{T}^{\frac{1}{4}} \sqrt{N_a}} +
\frac{\sqrt{r}}{\min(N_a, \bar{T})} 
+ \frac{\sqrt{r} \Delta_E}{\sqrt{N_a}} \right)
%
\\ (C) &\le \left\| \frac{\beta^{(a)}}{M_{1 - a}} \right\|_2 \cdot r \cdot \left( \frac{1}{\min(\bar{T}, N_a)} + \frac{\Delta_E}{\min(\sqrt{\bar{T}}, \sqrt{N_a})} + \Delta^2_E \right)
\end{align}
%
Collecting the various bounds completes this section.

\subsubsection{General conditions for ATE consistency.}
%
For simplicity, we suppress the conditioning on $\bA, \LF$ in the remainder of the proof.
%
\begin{proposition}\label{prop:ate_estimation_summary}
%
Let the conditions of Proposition \ref{prop:pcr_est} and Assumption \ref{assumption:pcr_subspace} hold.
%
For $a \in \{0, 1\}$, assume $$\|\beta^{(a)}\|_2 = O\left( \frac{M_{1-a}}{N^{w}_a} \right),$$ where $0 \le w \le \frac{1}{2}$.
%
Then,
%
\begin{align}
%
&\widehat{\mathsf{ATE}_{\Mc}} - \Ex[\mathsf{ATE}_{\Mc} \mid \LF]  
%
\\& = \sum_{a \in \{0, 1\}} C \cdot  \Delta_E \left( \frac{M_{1 - a} \cdot N_a^{0.5 - w}}{M} \right),
%
\\& \quad + C \cdot \frac{1}{\sqrt{M}},
%
\\& \quad + \sum_{a \in \{0, 1\}} C \cdot \frac{M_{1-a} \cdot N_a^{- w}}{M},
%
\\& \quad + \sum_{a \in \{0, 1\}}C \cdot \frac{M_{1-a}}{M N^w_a} \cdot  \sigma_\max^3 \cdot \ln^3(\bar{T} N_a) \cdot \left[r \left( \frac{1}{\min(\sqrt{\bar{T}}, \sqrt{N_a})} +  \Delta_E \right) \right],
%
\\& \quad + \sum_{a \in \{0, 1\}} C \cdot \frac{M_{1-a}}{M} \cdot N_a^{1/2 - w} \cdot \sigma_\max^3 \cdot \ln^3(\bar{T} N_a) \cdot \left[r \left( \frac{1}{\min(\sqrt{\bar{T}}, \sqrt{N_a})} +  \Delta_E \right) \right]\Delta_E,
%
\\& \quad + \sum_{a \in \{0, 1\}} C \cdot \frac{1}{M} \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot 
%
\left\{ \frac{M_{1-a}}{N^{w - 0.5}_a} \cdot \left( \frac{r^{3/2}}{\min(\bar{T}, N_a)} + \frac{r^{3/2} \Delta_E}{\min(\sqrt{\bar{T}}, \sqrt{N_a})} + r^{3/2} \Delta^2_E \right) \right\},
%
\\& \quad + \sum_{a \in \{0, 1\}} C \cdot \frac{\sqrt{N_a} M_{1-a}}{M} \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot  \left\{ \frac{\sqrt{r}}{ \bar{T}^{\frac{1}{4}} N_a^{0.5w + 0.25}} + \frac{ r}{N_a^{w - 0.5} \cdot \min(\bar{T}, N_a)} + \frac{ r \cdot \Delta_E}{N_a^{w}} \right\},
%
\\& \quad +\sum_{a \in \{0, 1\}} C \cdot \frac{ M_{1-a}}{M} \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot  \left\{\sqrt{r}\Delta_E + r \Delta^2_E \right\}.
%
\end{align}
%
\end{proposition}

\noindent
{\bf Proof of Proposition \ref{prop:ate_estimation_summary}.}

%
From Proposition \ref{prop:ate_estimation}, we have that
%
\begin{align}
%
&\widehat{\mathsf{ATE}_{\Mc}} - \Ex[\mathsf{ATE}_{\Mc} \mid \LF] 
%
\\&\le  C  \Delta_E \left(1 + \frac{\| \beta^{(0)}\|_1 + \| \beta^{(1)}\|_1}{M} \right) 
%
+ O_p\left( \sum_{a \in \{0, 1\}} \frac{\sigma_\max \left(\sqrt{M_a} +  \|\beta^{(a)} \|_2 + \|\Delta_{\beta^{(a)}}\|_2\right) +  \ldot{\Delta_{\beta^{(a)}}  }{\Ex\left[ Y_{\Ic^{(a)}} \right]}}{M} \right) 
%
\end{align}
%
We consider the various terms on the right-hand side above separately.

\vspace{2mm}
%
\noindent{\em 1. Bounding the $\Delta_E \left(1 + \frac{\| \beta^{(0)}\|_1 + \| \beta^{(1)}\|_1}{M} \right)$ term.}

\noindent
%
%
Given the assumption that $ \| \beta^{(a)} \|_2 = O\left( \frac{M_{1-a}}{N^w_a} \right)$, we have $\| \beta^{(a)} \|_1 = O\left( \frac{M_{1-a} N_a^{0.5}}{N_a^w} \right).$
%
Therefore
%
\begin{align}
%
\Delta_E \left(\frac{\| \beta^{(0)}\|_1 + \| \beta^{(1)}\|_1}{M} \right) 
%
&= C \cdot  \Delta_E \left( \frac{M_0 \cdot N_1^{0.5 - w} + M_1 \cdot N_0^{0.5 - w}}{M} \right) 
%
\\&= \sum_{a \in \{0, 1\}} C \cdot  \Delta_E \left( \frac{M_{1 - a} \cdot N_a^{0.5 - w}}{M} \right)
%
\label{eq:summary_4}
%
\end{align}

\noindent{\em 2. Bounding the $\sum_{a \in \{0, 1\}}  \frac{\sigma_\max (\sqrt{M_a} +  \|\beta^{(a)} \|_2)}{M}$ term.}

\noindent
Note that since $M_a < M$,
%
\begin{align}
%
\sum_{a \in \{0, 1\}}  \frac{\sigma_\max \sqrt{M_a}}{M}
%
= O\left(\frac{1}{\sqrt{M}}\right). \label{eq:summary_9}
%
\end{align}
%
Further,
%
\begin{align}
%
\sum_{a \in \{0, 1\}}  \frac{\|\beta^{(a)} \|_2}{M} 
%
= C \cdot \frac{M_0 \cdot N_1^{- w} + M_1 \cdot N_0^{- w}}{M} 
%
= \sum_{a \in \{0, 1\}} C \cdot \frac{M_{1-a} \cdot N_a^{- w}}{M} 
\label{eq:summary_10}
%
\end{align}

\noindent{\em 3. Bounding the $\sum_{a \in \{0, 1\}}  \frac{\sigma_\max \left\|\Delta_{\beta^{(a)}}\right\|_2}{M}$ term.}

\noindent
Using Proposition \ref{prop:pcr_est} and $ \| \beta^{(a)} \|_2 = O\left( \frac{M_{1-a}}{N^w_a} \right)$, we have
%
\begin{align}
%
&\sum_{a \in \{0, 1\}}\frac{\|\Delta_{\beta^{(a)}}\|_2}{M}
%
\\ &\le \sum_{a \in \{0, 1\}}\frac{1}{M} \cdot C \cdot \sigma_\max^3 \cdot \ln^3(\bar{T} N_a) \cdot \left[\left\| \beta^{(a)} \right\|_2 \cdot \left( \frac{r}{\min(\sqrt{\bar{T}}, \sqrt{N_a})} + r \Delta_E \right) + \frac{M_{1-a} \sqrt{r} \Delta_E}{\sqrt{N_a}} \right],
%
\\ &\le \sum_{a \in \{0, 1\}}\frac{M_{1-a}}{M} \cdot C \cdot \sigma_\max^3 \cdot \ln^3(\bar{T} N_a) \cdot \left[\frac{1}{N^w_a} \cdot \left( \frac{r}{\min(\sqrt{\bar{T}}, \sqrt{N_a})} + r \Delta_E \right) + \frac{\sqrt{r} \Delta_E}{\sqrt{N_a}} \right],
%
\\ &\le \sum_{a \in \{0, 1\}} C \cdot \frac{M_{1-a}}{M N^w_a} \cdot  \sigma_\max^3 \cdot \ln^3(\bar{T} N_a) \cdot \left[r \left( \frac{1}{\min(\sqrt{\bar{T}}, \sqrt{N_a})} +  \Delta_E \right) \right],
\label{eq:summary_2}
%
\end{align}
%
where in the third inequality we have used that $w \le \frac{1}{2}$.


\noindent{\em 4. Bounding the $\sum_{a \in \{0, 1\}}  \frac{\ldot{\Delta_{\beta^{(a)}} }{\Ex\left[ Y_{\Ic^{(a)}} \right]}}{M}$ term.}

\noindent
Assumptions \ref{assumption:conditonal_independence} and \ref{assumption:outcome_generating_function_factor_structure}, and
Definition \ref{def:linear_factor_approx}, we have that $\Ex[Y^{(a)}_{j, t^*}] = \ldot{\lambda_j}{\rho_{t^*, a}} + \eta^{(a)}_{j, t^*}$.
%
Hence
%
\begin{align}
%
\sum_{a \in \{0, 1\}} \left| \ldot{\Delta_{\beta^{(a)}} }{\Ex\left[ Y_{\Ic^{(a)}} \right]} \right|
%
&= \sum_{a \in \{0, 1\}} \left| \ldot{\Delta_{\beta^{(a)}} }{[\ldot{\lambda_j}{\rho_{t^*, a}} + \eta^{(a)}_{j, t^*}]_{n \in \Ic^{(a)}}} \right|
%
\\ &= \sum_{a \in \{0, 1\}}  \left| \ldot{\Delta_{\beta^{(a)}} }{[\ldot{\lambda_j}{\rho_{t^*, a}}]_{n \in \Ic^{(a)}}} + \ldot{\Delta_{\beta^{(a)}} }{[\eta^{(a)}_{j, t^*}]_{n \in \Ic^{(a)}}} \right|
%
\\ &\le \sum_{a \in \{0, 1\}} \left| \ldot{\Delta_{\beta^{(a)}} }{[\ldot{\lambda_j}{\rho_{t^*, a}}]_{n \in \Ic^{(a)}}} \right| + \|\Delta_{\beta^{(a)}}\|_2 \| [\eta^{(a)}_{j, t^*}]_{n \in \Ic^{(a)}} \|_2 
%
\\ &\le \sum_{a \in \{0, 1\}} \left| \ldot{\Delta_{\beta^{(a)}} }{[\ldot{\lambda_j}{\rho_{t^*, a}}]_{n \in \Ic^{(a)}}} \right| + \|\Delta_{\beta^{(a)}}\|_2 \sqrt{N_a} \Delta_E
%
\end{align}
%
Using Assumption \ref{assumption:pcr_subspace}, we have
%
\begin{align}
%
\left| \ldot{\Delta_{\beta^{(a)}} }{[\ldot{\lambda_j}{\rho_{t^*, a}}]_{n \in \Ic^{(a)}}} \right|
%
&= \left| \ldot{\Delta_{\beta^{(a)}} }{\mathsf{Proj}([\ldot{\lambda_j}{\rho_{t^*, a}}]_{n \in \Ic^{(a)}}}) \right|
%
\\&= \left| \ldot{\mathsf{Proj}(\Delta_{\beta^{(a)}})}{[\ldot{\lambda_j}{\rho_{t^*, a}}]_{n \in \Ic^{(a)}}} \right|
%
\\& \le \| \mathsf{Proj}(\Delta_{\beta^{(a)}}) \|_2 \| [\ldot{\lambda_j}{\rho_{t^*, a}}]_{n \in \Ic^{(a)}} \|_2
%
\\& \le C \| \mathsf{Proj}(\Delta_{\beta^{(a)}}) \|_2 \sqrt{N_a},
%
\end{align}
%
where recall $\mathsf{Proj} = \bV_r \bV_r^T$, and $\bV_r$ are the right singular vectors of $\bX^{\text{lr}}$.

%
Hence, we have
%
\begin{align}
%
\frac{1}{M}\sum_{a \in \{0, 1\}} \left| \ldot{\Delta_{\beta^{(a)}} }{\Ex\left[ Y_{\Ic^{(a)}}  \right]} \right|
%
&\le \sum_{a \in \{0, 1\}} \frac{1}{M}\|\Delta_{\beta^{(a)}}\|_2 \sqrt{N_a} \Delta_E + \frac{C}{M}  \| \mathsf{Proj}(\Delta_{\beta^{(a)}}) \|_2 \sqrt{N_a}  
%
\end{align}
%
We bound each term above separately. 


\noindent{\em 4a. Bounding the $ \sum_{a \in \{0, 1\}} \frac{1}{M}\|\Delta_{\beta^{(a)}}\|_2 \sqrt{N_a} \Delta_E$ term.}
%
For the first term, by applying a similar logic used to derive \eqref{eq:summary_2}, we have that
%
\begin{align}
%
&\sum_{a \in \{0, 1\}} \frac{1}{M}\|\Delta_{\beta^{(a)}}\|_2 \sqrt{N_a} \Delta_E 
%
\\&\le \sum_{a \in \{0, 1\}}\frac{M_{1-a}}{M N^w_a} \cdot C \cdot \sigma_\max^3 \cdot \ln^3(\bar{T} N_a) \cdot \left[r \left( \frac{1}{\min(\sqrt{\bar{T}}, \sqrt{N_a})} +  \Delta_E \right) \right]\sqrt{N_a}\Delta_E
%
\\&\le \sum_{a \in \{0, 1\}}\frac{M_{1-a}}{M} \cdot N_a^{1/2 - w} \cdot C \cdot \sigma_\max^3 \cdot \ln^3(\bar{T} N_a) \cdot \left[r \left( \frac{1}{\min(\sqrt{\bar{T}}, \sqrt{N_a})} +  \Delta_E \right) \right]\Delta_E
\label{eq:summary_5}
%
\end{align}

\noindent{\em 4b. Bounding the $\sum_{a \in \{0, 1\}} \frac{C}{M} \| \mathsf{Proj}(\Delta_{\beta^{(a)}}) \|_2 \sqrt{N_a}$ term.}

\noindent
%
Using Proposition \ref{prop:pcr_est_proj} and $ \| \beta^{(a)} \|_2 = O\left( \frac{M_{1-a}}{N^w_a} \right)$, we have
%
\begin{align}
%
&\sum_{a \in \{0, 1\}} \frac{C}{M} \| \mathsf{Proj}(\Delta_{\beta^{(a)}}) \|_2 \sqrt{N_a}
%
\\& \le \sum_{a \in \{0, 1\}}
%
\quad \frac{C\sqrt{N_a}}{M} \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot 
\left\{ \left\| \beta^{(a)} \right\|_2 \cdot \left( \frac{r^{3/2}}{\min(\bar{T}, N_a)} + \frac{r^{3/2} \Delta_E}{\min(\sqrt{\bar{T}}, \sqrt{N_a})} + r^{3/2} \Delta^2_E \right) \right\},
%
\\& \quad \quad + \frac{C\sqrt{N_a}}{M} \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot  \left\{ \left\| \beta^{(a)} \right\|_1 \cdot \left( \frac{\sqrt{r}}{\left\| \frac{\beta^{(a)}}{M_{1 - a}} \right\|^{1/2}_1 \bar{T}^{\frac{1}{4}} \sqrt{N_a}} +
\frac{r}{\min(\bar{T}, N_a)} + \frac{r \Delta_E}{\sqrt{N_a}} \right) \right\},
%
\\& \quad \quad + \frac{C\sqrt{N_a}}{M} \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot M_{1-a} \cdot  \left\{\frac{\sqrt{r}\Delta_E}{\sqrt{N_a}} + \frac{r \Delta^2_E}{\sqrt{N_a}} \right\}. \label{eq:summary_3}
%
\end{align}

We bound the three terms on the r.h.s above separately. 

\begin{enumerate}
%
\item First term of \eqref{eq:summary_3}.
%
\begin{align}
%
&\sum_{a \in \{0, 1\}}
%
\frac{C\sqrt{N_a}}{M} \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot 
\left\{ \left\| \beta^{(a)} \right\|_2 \cdot \left( \frac{r^{3/2}}{\min(\bar{T}, N_a)} + \frac{r^{3/2} \Delta_E}{\min(\sqrt{\bar{T}}, \sqrt{N_a})} + r^{3/2} \Delta^2_E \right) \right\}
%
\\& \le \sum_{a \in \{0, 1\}}
%
\quad \frac{C}{M} \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot 
%
\left\{ \frac{M_{1-a}}{N^{w - 0.5}_a} \cdot \left( \frac{r^{3/2}}{\min(\bar{T}, N_a)} + \frac{r^{3/2} \Delta_E}{\min(\sqrt{\bar{T}}, \sqrt{N_a})} + r^{3/2} \Delta^2_E \right) \right\}. \label{eq:summary_6}
%
\end{align}

\item Second term of \eqref{eq:summary_3}.
%
\begin{align}
%
&\sum_{a \in \{0, 1\}} \frac{C\sqrt{N_a}}{M} \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot  \left\{ \left\| \beta^{(a)} \right\|_1 \cdot \left( \frac{\sqrt{r}}{\left\| \frac{\beta^{(a)}}{M_{1 - a}} \right\|^{1/2}_1 \bar{T}^{\frac{1}{4}} \sqrt{N_a}} +
\frac{r}{\min(\bar{T}, N_a)} + \frac{r \Delta_E}{\sqrt{N_a}} \right) \right\}
%
\\ &\le \sum_{a \in \{0, 1\}} \frac{C\sqrt{N_a}}{M} \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot  \left\{ \frac{\sqrt{r} \left\| \beta^{(a)} \right\|^{0.5}_1 M_{1 - a}^{0.5}}{ \bar{T}^{\frac{1}{4}} \sqrt{N_a}} + \frac{ \left\| \beta^{(a)} \right\|_1 r}{\min(\bar{T}, N_a)} + \frac{ \left\| \beta^{(a)} \right\|_1 r \Delta_E}{\sqrt{N_a}} \right\},
% 
\\ &\le \sum_{a \in \{0, 1\}} \frac{C\sqrt{N_a}}{M} \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot  \left\{ \frac{\sqrt{r} \cdot M_{1-a} }{ \bar{T}^{\frac{1}{4}} N_a^{0.5w + 0.25}} + \frac{ M_{1-a} \cdot r}{N_a^{w - 0.5} \cdot \min(\bar{T}, N_a)} + \frac{ M_{1-a} \cdot r \cdot \Delta_E}{N_a^{w}} \right\},
%
\\ &\le \sum_{a \in \{0, 1\}} \frac{C\sqrt{N_a} M_{1-a}}{M} \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot  \left\{ \frac{\sqrt{r} }{ \bar{T}^{\frac{1}{4}} N_a^{0.5w + 0.25}} + \frac{ r}{N_a^{w - 0.5} \cdot \min(\bar{T}, N_a)} + \frac{ r \cdot \Delta_E}{N_a^{w}} \right\}. \label{eq:summary_7}
\end{align}

\item Third term of \eqref{eq:summary_3}.
%
\begin{align}
%
&\sum_{a \in \{0, 1\}} \frac{C\sqrt{N_a}}{M} \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot M_{1-a} \cdot  \left\{\frac{\sqrt{r}\Delta_E}{\sqrt{N_a}} + \frac{r \Delta^2_E}{\sqrt{N_a}} \right\}
%
\\ &= \sum_{a \in \{0, 1\}} C \cdot \frac{ M_{1-a}}{M} \cdot \sigma_\max^4 \cdot \ln^{9/2}(\bar{T} N_a) \cdot  \left\{\sqrt{r}\Delta_E + r \Delta^2_E \right\}
\label{eq:summary_8}
%
\end{align}
%
\end{enumerate}

\noindent{\em Summarizing all terms.}

Using \eqref{eq:summary_4}, \eqref{eq:summary_9}, \eqref{eq:summary_10}, \eqref{eq:summary_5}, \eqref{eq:summary_3}, \eqref{eq:summary_6}, \eqref{eq:summary_7}, \eqref{eq:summary_8}, we complete the proof of the proposition.
%


\subsubsection{Finishing proof of Theorem \ref{thm:consistency_summary}.}

Recall from Proposition \ref{prop:factor_model_approx}, we have that
%
\begin{align}\label{eq:summary_0}
%
r \le C \cdot \delta^{-q}, \quad \Delta_E \le C \cdot \delta^S.
%
\end{align}
%

{\bf $\textsf{ATT}$ consistency.}

%
For estimation of $\textsf{ATT}$, we have that $M = M_1 = N_1$ and $M_0 = 0$.
%
Hence, by simplifying the result in Proposition \ref{prop:ate_estimation_summary}, we get that
%
\begin{align}
%
&\widehat{\mathsf{ATE}_{\Mc}} - \Ex[\mathsf{ATE}_{\Mc} \mid \LF]  
%
\\&\le C \cdot  \Delta_E \left(  N_0^{0.5 - w}\right), \label{eq:ATT_summary_1}
%
\\& \quad + C \cdot \frac{1}{\sqrt{M}}, \label{eq:ATT_summary_2}
%
\\& \quad + C \cdot  N_0^{- w}, \label{eq:ATT_summary_3}
%
\\& \quad + C \cdot \frac{1}{N^w_0} \cdot \ln^3(\bar{T} N_0) \cdot \left[r \left( \frac{1}{\min(\sqrt{\bar{T}}, \sqrt{N_0})} +  \Delta_E \right) \right], \label{eq:ATT_summary_4}
%
\\& \quad + C \cdot N_0^{1/2 - w} \cdot \ln^3(\bar{T} N_0) \cdot \left[r \left( \frac{1}{\min(\sqrt{\bar{T}}, \sqrt{N_0})} +  \Delta_E \right) \right]\Delta_E, \label{eq:ATT_summary_5}
%
\\& \quad + C \cdot \ln^{9/2}(\bar{T} N_0) \cdot 
%
\left\{ \frac{1}{N^{w - 0.5}_0} \cdot \left( \frac{r^{3/2}}{\min(\bar{T}, N_0)} + \frac{r^{3/2} \Delta_E}{\min(\sqrt{\bar{T}}, \sqrt{N_0})} + r^{3/2} \Delta^2_E \right) \right\}, \label{eq:ATT_summary_6}
%
\\& \quad + C \cdot \sqrt{N_0}   \cdot \ln^{9/2}(\bar{T} N_0) \cdot  \left\{ \frac{\sqrt{r}}{ \bar{T}^{\frac{1}{4}} N_0^{0.5w + 0.25}} + \frac{ r}{N_0^{w - 0.5} \cdot \min(\bar{T}, N_0)} + \frac{ r \cdot \Delta_E}{N_0^{w}} \right\},  \label{eq:ATT_summary_7}
%
\\& \quad + C  \cdot \ln^{9/2}(\bar{T} N_0) \cdot  \left\{\sqrt{r}\Delta_E + r \Delta^2_E \right\}. \label{eq:ATT_summary_8}
%
\end{align} 

We deal with the seven terms above separately. 

Let $G = \min(N_0, \bar{T})$.
%
For $\gamma > 0$, take $\delta = \left(\frac{1}{G}\right)^{\gamma / q}$.
%
Then \eqref{eq:summary_0} implies
%
\begin{align}\label{eq:summary_1}
%
r \le C G^\gamma, \quad \Delta_E &\le C \left(\frac{1}{G}\right)^{ \gamma \alpha}.
%
\end{align}
%
We set $\gamma = \frac{1}{2\alpha}$ and so we have $r \le C G^{\frac{1}{2\alpha}}$, and that $\Delta_E \le C G^{-0.5}$.


{\em Term \eqref{eq:ATT_summary_1}}.
%
\begin{align}
%
&C \cdot  \Delta_E \left(  N_0^{0.5 - w}\right)
%
\le G^{-\gamma \alpha} N_0^{0.5 - w} 
% 
= G^{-0.5} N_0^{0.5 - w}
%'
= o_p(1)
%
\end{align}
%
where in the last line we have used $\alpha > 1$ and the assumption $\frac{N_0^{1 - w}}{\bar{T}^{1 - \frac{1}{2 \alpha}}} = o(1) \implies \frac{N_0^{0.5 - w}}{\bar{T}^{0.5}} = o(1)$; we also use the assumption that $w > 0$. 

{\em Term \eqref{eq:ATT_summary_2} and \eqref{eq:ATT_summary_3}}.

Given the assumption that $M (= N_1), N_0 \to \infty$, and that $w > 0$, 
%
\begin{align}
%
C \cdot \frac{1}{\sqrt{M}} &= o_p(1),
%
\\ C \cdot  N_0^{- w} &= o_p(1).
%
\end{align}

{\em Term \eqref{eq:ATT_summary_4}}.
%
\begin{align}
%
&C \cdot \frac{1}{N^w_0} \cdot \ln^3(\bar{T} N_0) \cdot \left[r \left( \frac{1}{\min(\sqrt{\bar{T}}, \sqrt{N_0})} +  \Delta_E \right) \right]
%
\\&\le C \cdot \frac{1}{N^w_0} \cdot \ln^3(\bar{T} N_0) \cdot \left[G^{\gamma} \left( \frac{1}{\min(\sqrt{\bar{T}}, \sqrt{N_0})} +  G^{-\gamma \alpha} \right) \right]
%
\\&\le C \cdot \ln^3(\bar{T} N_0) \cdot \left[G^{\gamma - w - 0.5} + G^{\gamma (1 - \alpha) - w}   \right]
%
\\&= C \cdot \ln^3(\bar{T} N_0) \cdot \left[G^{0.5(\frac{1}{\alpha} - 1) - w} \right] \label{eq:ATT_normality_helper_1}
%
\\&= o_p(1)
%
\end{align}
%
where in the last line we use the inequality that $w > \frac{1}{2 \alpha} - \frac{1}{2}$.

{\em Term \eqref{eq:ATT_summary_5}}.
%
\begin{align}
%
&C \cdot N_0^{1/2 - w} \cdot \ln^3(\bar{T} N_0) \cdot \left[r \left( \frac{1}{\min(\sqrt{\bar{T}}, \sqrt{N_0})} +  \Delta_E \right) \right]\Delta_E
%
\\&\le C \cdot \ln^3(\bar{T} N_0) \cdot \left[G^{\frac{1}{2 \alpha} - 0.5}   \right] \cdot  G^{-0.5} \cdot N_0^{0.5 - w}  
%
\\&= o_p(1)
%
\end{align}
%
where in the last line we have used $\alpha > 1$ and the assumption $\frac{N_0^{1 - w}}{\bar{T}^{1 - \frac{1}{2 \alpha}}} = o(1) \implies \frac{N_0^{0.5 - w}}{\bar{T}^{0.5}} = o(1)$; we also use the assumption that $w > 0$. 

{\em Term \eqref{eq:ATT_summary_6}}.
%
\begin{align}
%
&C \cdot \ln^{9/2}(\bar{T} N_0) \cdot 
\left\{ \frac{1}{N^{w - 0.5}_0} \cdot \left( \frac{r^{3/2}}{\min(\bar{T}, N_0)} + \frac{r^{3/2} \Delta_E}{\min(\sqrt{\bar{T}}, \sqrt{N_0})} + r^{3/2} \Delta^2_E \right) \right\}
%
\\&\le  C \cdot \ln^{9/2}(\bar{T} N_0) \cdot \left\{ \frac{1}{N^{w - 0.5}_0} \cdot \left( G^{1.5\gamma - 1} + G^{\gamma(1.5 - \alpha) - 0.5} + G^{\gamma(1.5 - 2\alpha)}\right) \right\}
%
%\\&\le  C \cdot \ln^{9/2}(\bar{T} N_0) \cdot \left\{ \frac{ G^{\frac{0.75}{\alpha} - 1}  }{N^{w - 0.5}_0}  \right\}
%
\\&\le  C \cdot \ln^{9/2}(\bar{T} N_0) \cdot \left\{ \frac{ N_0 ^{0.5 - w} }{G^{1 - \frac{0.75}{\alpha}}}  \right\}
%
\\&= o_p(1)
%
\end{align}
%
where in the last line we have used the fact that $w > \frac{1}{2 \alpha}$, $\alpha > \frac{1}{2}$ and the assumption that $\frac{N_0^{1 - w}}{\bar{T}^{1 - \frac{1}{2 \alpha}}} = o(1)$.

{\em Term \eqref{eq:ATT_summary_7}}.
%
\begin{align}
%
&C \cdot \sqrt{N_0}   \cdot \ln^{9/2}(\bar{T} N_0) \cdot  \left\{ \frac{\sqrt{r}}{ \bar{T}^{\frac{1}{4}} N_0^{0.5w + 0.25}} + \frac{ r}{N_0^{w - 0.5} \cdot \min(\bar{T}, N_0)} + \frac{ r \cdot \Delta_E}{N_0^{w}} \right\}
%
\\&\le C  \cdot \ln^{9/2}(\bar{T} N_0) \cdot  \left\{ \frac{\sqrt{r}}{ \bar{T}^{\frac{1}{4}} N_0^{0.5w - 0.25}} + \frac{r}{N_0^{w -1} \cdot \min(\bar{T}, N_0)} + \frac{ r \cdot \Delta_E}{N_0^{w - 0.5}} \right\}
%
\\&\le C  \cdot \ln^{9/2}(\bar{T} N_0) \cdot  \left\{ \frac{G^{\frac{1}{4 \alpha}} N_0^{0.25 - 0.5w}}{ \bar{T}^{\frac{1}{4}} } + \frac{N_0^{1 - w}}{G^{1 - \frac{1}{2 \alpha}}} + \frac{N_0^{0.5 - w}}{G^{0.5 - \frac{1}{2\alpha}}} \right\}
%
\\&= o_p(1)
%
\end{align}
%
where in the last line we have used the fact that $w > \frac{1}{2 \alpha}$ and the assumption that $\frac{N_0^{1 - w}}{\bar{T}^{1 - \frac{1}{2 \alpha}}} = o(1)$.

{\em Term \eqref{eq:ATT_summary_8}}.

%
Using the assumption that $\alpha > \frac{1}{2}$,  we have that 
%
\begin{align}
%
&\sqrt{r}\Delta_E \le C G^{0.5 \gamma} \cdot G^{- \gamma \alpha} = G^{\gamma(0.5 - \alpha)} = o_p(1),
%
\end{align} 
%
which also implies that $r\Delta^2_E = o_p(1)$.
%

{\em Completing the proof of $\mathsf{ATT}$ consistency.}
%

The above inequalities establish that $\widehat{\mathsf{ATT}}  - \Ex[\mathsf{ATT} \mid \LF] = o_p(1)$.
%
Additionally, the fact that $\widehat{\mathsf{ATT}}  - \mathsf{ATT} \mid \LF = o_p(1)$ follows from Corollary \ref{cor:ate_estimation} and using that $M (= N_1) \to \infty$.


{\bf $\textsf{ATU}$ consistency.}

%
The proof follows in an analogous manner to that of $\mathsf{ATT}$, where we switch the roles of the treated and untreated. 
%
That is, $M = M_0 = N_0$ and $M_1 = 0$.

{\bf $\textsf{ATE}$ consistency.}

%
The proof follows in an analogous manner to that of $\mathsf{ATT}$, where now $M_0, M_1 = \Theta(M)$, and we have $M_0 = N_0$, $M_1 = N_1$, $M = N$.




\subsection{Proof of Proposition \ref{prop:beta_norm}.}
%
For simplicity and without loss of generality, we let the $N_a$ units in $\Ic^{(a)}$ be the indexed as the first $N_a$ units.

Now, given the assumption in the statement of Proposition \ref{prop:beta_norm}, we have that for $k \in [N_{a}^{1 - \theta}]$ there exists $\beta^{n, k} \in \Rb^{N_{a}^{\theta}}$ such that for all $n \in \Mc^{(1-a)}$
%
\begin{align}
%
\lambda_n = \sum^{k N_{a}^\theta}_{i = 1 + (k - 1)N_{a}^\theta} \beta^{n, k}_i \lambda_i
%
\end{align}
%
and 
%
\begin{align}
%
\| \beta^{n, k} \|_2 = O(\sqrt{r}).
%
\end{align}
%
Define $\tilde{\beta}^n \in \Rb^{N_a}$ as follows
%
\begin{align}
%
\tilde{\beta}^n = \frac{1}{N_{a}^{1 - \theta}}[\beta^{n, 1}, \dots, \beta^{n, N_{a}^{1 - \theta}}].
%
\end{align}
%
Note
%
\begin{align}
%
\lambda_n = \sum^{N_a}_{i = 1} \tilde{\beta}^n_i \lambda_i.
%
\end{align}
%
Then using $1 -  \frac{3}{2\alpha} > \theta   \Longleftrightarrow  \frac{1 - \theta}{2} - \frac{1}{4\alpha} > \frac{1}{2\alpha}$, we have
%
\begin{align}
%
\| \tilde{\beta}^n \|_2 
%
= O\left( \frac{\sqrt{r}}{N_{a}^{\frac{1 - \theta}{2}}} \right) 
%
= O\left( \frac{N_{a}^{\frac{1}{4\alpha}}}{N_{a}^{\frac{1 - \theta}{2}}} \right)  
%
= o\left(\frac{1}{N_{a}^{{\frac{1}{2\alpha}}}}\right).
%
\end{align}
%
Then define 
%
\begin{align}
%
\tilde{\beta}^{\Ic^{(a)}} &= \sum_{n \in \Mc^{(1-a)}} \tilde{\beta}^n,    
%
\\\implies \sum^{N_a}_{i = 1} \tilde{\beta}^{\Ic^{(a)}}_i \lambda_i &= \sum_{n \in \Mc^{(1-a)}} \sum^{N_a}_{i = 1} \tilde{\beta}^n_i   \lambda_i = \sum_{n \in \Mc^{(1-a)}} \lambda_n = \lambda_{\Mc^{(1-a)}}.
%
\end{align}

Hence, 
%
\begin{align}
%
\| \tilde{\beta}^{\Ic^{(a)}} \|_2 = o\left(\frac{M_{1-a}}{N_{a}^{{\frac{1}{2\alpha}}}}\right).
%
\end{align}
%
Since we define $\beta^{(a)}$ to be linear weight with minimum $\ell_2$-norm in Assumption \ref{assumption:linear_span_inclusion}, it follows that 
%
$\| \beta^{(a)} \|_2 =  o\left(\frac{M_{1-a}}{N_{a}^{{\frac{1}{2\alpha}}}}\right)$.
%
This completes the proof.





==> Old/proofs/proofs_ate_normality.tex <==
\section{ATE: Asymptotic Normality}

\subsection{Proof of Proposition \ref{prop:ate_normality}.}

\noindent
%
Write $\tau_{a} = \tau_{a, a} + \tau_{a, 1 - a}$, where 
%
\begin{align}
%
\tau_{a, a} &\coloneqq \frac{1}{M
} \left( \sum_{n \in \Mc^{(a)}} Y_{n, t^*}  -  \Ex[Y_{n, t^*} \mid \bA, \LF] \right) 
%
\\ \tau_{a, 1 - a} &\coloneqq \frac{1}{M} \left( \sum_{n \in\Ic^{(a)}} \hbeta^{(a)}_n Y_{n, t^*}  -  \beta^{(a)}_n \Ex\left[ Y_{n, t^*} \mid \bA, \LF \right] \right)
%
\end{align}
%
Using the definition of $\tau_{a, a}$ we have 
%
\begin{align}
%
\frac{\sqrt{M}}{\bar{\sigma}} \cdot \tau_{a, a} &= \frac{1}{\bar{\sigma} \sqrt{M}} \left( \sum_{n \in \Mc^{(a)}} \varepsilon^{(a)}_{{n, t^*}}  \right). \label{eq:ate_normality_helper_0}
%
\end{align}
%
Using the definition of $\tau_{a, 1 - a}$ we have 
%
\begin{align}
%
\frac{\sqrt{M}}{\bar{\sigma}} \cdot \tau_{a, 1 - a} 
%
&= \frac{1}{\bar{\sigma} \sqrt{M}} \left( \sum_{n \in \Ic^{(a)}} \hbeta^{(a)}_n Y_{n, t^*} -  \beta^{(a)}_n \Ex\left[ Y_{n, t^*} \mid \bA, \LF \right] \right)
%
\\&= \frac{1}{\bar{\sigma} \sqrt{M}} \left( \ldot{\Delta_{\beta^{(a)}}}{\varepsilon_{\Ic^{(a)}}} + \ldot{\Delta_{\beta^{(a)}}}{\Ex\left[ Y_{\Ic^{(a)}} \mid \bA, \LF \right]} + \ldot{\beta^{(a)}}{\varepsilon_{\Ic^{(a)}} } \right) \label{eq:ate_normality_helper_1}
%
\end{align}
%
Using Condition {\em 1} and {\em 2} in the proposition statement, we immediately have that
%
\begin{align}
%
\frac{1}{\bar{\sigma} \sqrt{M}} \left( \ldot{\Delta_{\beta^{(a)}}}{\varepsilon_{\Ic^{(a)}}} + \ldot{\Delta_{\beta^{(a)}}}{\Ex\left[ Y_{\Ic^{(a)}} \mid \bA, \LF \right]}\right)
%
= o_p(1). \label{eq:ate_normality_helper_2}
%
\end{align}
%
Hence,
%
\begin{align}
%
\frac{\sqrt{M}}{\bar{\sigma}} \cdot \tau_{a, 1 - a} 
%
= \frac{1}{\bar{\sigma} \sqrt{M}} \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \varepsilon^{(a)}_{n, t^*}
%
+ o_p(1) \label{eq:ate_normality_helper_3}
%
\end{align}
%
Using \eqref{eq:ate_normality_helper_0} and \eqref{eq:ate_normality_helper_3}, we have
%
\begin{align}
%
\frac{\sqrt{M}}{\bar{\sigma}} \cdot \tau_{a} 
%
&= o_p(1) + \frac{1}{\bar{\sigma} \sqrt{M}} \left( \sum_{n \in \Mc^{(a)}} \varepsilon^{(a)}_{{n, t^*}} + \sum_{n \in \Ic^{(a)}} \beta^{(a)}_n \varepsilon^{(a)}_{n, t^*} \right).
%
\end{align}
%
Hence, letting $\tilde{\sigma} = \bar{\sigma} \sqrt{M}$, we have
%
\begin{align}
%
&\frac{\sqrt{M}}{\bar{\sigma}} \left( \widehat{\mathsf{ATE}_{t}}  - \Ex[\mathsf{ATE}_{t} \mid \mathsf{U}] \right)
%
\\&= \frac{\sqrt{M}}{\bar{\sigma}} (\tau_{1} - \tau_{0}) + \frac{\sqrt{M}}{\bar{\sigma}}  \mathsf{Approx}_t
%
\\&= o_p(1) + \frac{1}{\bar{\sigma} \sqrt{M}} \left[ \left( \sum_{n \in \Mc^{(1)}} \varepsilon^{(1)}_{{n, t^*}} + \sum_{n \in \Ic^{(1)}} \beta^{(1)}_n \varepsilon^{(1)}_{n, t^*} \right) - \left( \sum_{n \in \Mc^{(0)}} \varepsilon^{(0)}_{{n, t^*}} + \sum_{n \in \Ic^{(0)}} \beta^{(0)}_n \varepsilon^{(0)}_{n, t^*} \right)\right]
%
\\&= o_p(1) + \frac{1}{\tilde{\sigma}} \left[ \left(\sum_{n \in \Ic^{(1)} \setminus \Mc^{(1)}} \beta^{(1)}_n \varepsilon^{(1)}_{n, t^*} + \sum_{n \in \Mc^{(1)}} (1 + \beta^{(1)}_n) \varepsilon^{(1)}_{{n, t^*}} \right) - \left(\sum_{n \in \Ic^{(0)} \setminus \Mc^{(0)}} \beta^{(0)}_n \varepsilon^{(0)}_{n, t^*} + \sum_{n \in \Mc^{(0)}} (1 + \beta^{(0)}_n) \varepsilon^{(0)}_{{n, t^*}}  \right)\right] \label{eq:ate_normality_helper_4}
%
\\&\to \Nc(0, 1), 
%
\end{align}
%
where the last line follows from using the Lyapunov central limit theorem (CLT) (\cite{billingsley2008probability}) as $N \to \infty$.
%
In particular, the sequence of independent random variables are $(X_n)_{n \in [N]}$, where 
%
\begin{align}
X_n 
%
= \begin{cases}
%
(1 + \beta^{(a)}_n) \varepsilon^{(a)}_{n, t^*}  & \text{ if } n \in \Mc^{(a)}, \\
%
\beta^{(a)}_n \varepsilon^{(a)}_{n, t^*}  & \text{ if } n \in \Ic^{(a)} \setminus \Mc^{(a)}.
%
\end{cases}
\end{align}
%
If $\varepsilon^{(a)}_{n, t^*} \in \Mc^{(a)}$, then its variance is given by $[(1 + \beta^{(a)}_n)\sigma^{(a)}_{n, t}]^{2}$, and if $\varepsilon^{(a)}_{n, t^*} \in \Ic^{(a)} \setminus \Mc^{(a)}$, this its variance is given by $[\beta^{(a)}_n\sigma^{(a)}_{n, t}]^{2}$.
%
We note that the sum of the variances of the sequence of random variables $(X_n)_{n \in [N]}$ is exactly given by $\tilde{\sigma}^{2}$.
%
To apply the Lyapunov CLT, it remains to verify the Lyapunov condition (with $\delta = 2$):
%
\begin{align}\label{eq:Lyapunov}
%
\frac{1}{\tilde{\sigma}^{4}} \sum^{N}_{n = 1} \Ex\left[ X^{4}_n \right] \to 0, \quad \text{ as } N \to \infty.
%
\end{align}
%
Since $\varepsilon^{(a)}_{n, t^*}$ is a sub-Gaussian random variable by Assumption \ref{assumption:sub-gaussian_noise}, we have that $\Ex[(\varepsilon^{(a)}_{n, t^*})^{4}] \le C$. Hence,
%
\begin{align}
\Ex\left[ X^{4}_n \right]
%
\le \begin{cases}
%
C (1 + \beta^{(a)}_n)^4  & \text{ if } n \in \Mc^{(a)}, \\
%
C (\beta^{(a)}_n)^4  & \text{ if } n \in \Ic^{(a)} \setminus \Mc^{(a)}.
%
\end{cases}
\end{align}
%
Hence, by Condition 4 in the proposition statement, \eqref{eq:Lyapunov} is verified. 

==> Old/proofs/sandbox_normality_proof.tex <==
\subsection{Proof of Theorem \ref{thm:att_atu_normality_PCR}.}
%
Given Proposition \ref{prop:ate_normality}, it suffices to show that for $a \in \{0, 1\}$,
%
\begin{enumerate}
%
\item $\frac{1}{\bar{\sigma}}  \ldot{\Delta_{\beta^{(a)}}}{\varepsilon_{\Ic^{(a)}}}
= o_p(1).$ ({\color{blue} AA: Proven})
%
\item $\frac{1}{\bar{\sigma}}\ldot{\Delta_{\beta^{(a)}}}{\Ex\left[ Y_{\Ic^{(a)}} \mid \Omega, \mathsf{U}\right]} = o_p(1).$
%
\item $\frac{M}{\bar{\sigma}}  \mathsf{Approx} = o_p(1).$ 
%
\end{enumerate}

As in Theorem \ref{thm:consistency_summary}, we let $G = \min(N_0, \bar{T})$.
%
For $\gamma > 0$, take $\delta = \left(\frac{1}{G}\right)^{\gamma / q}$.
%
Then \eqref{eq:summary_0} implies
%
\begin{align}\label{eq:summary_1}
%
r \le C G^\gamma, \quad \Delta_E &\le C \left(\frac{1}{G}\right)^{ \gamma \alpha}.
%
\end{align}
%
We set $\gamma = \frac{1}{2\alpha}$ and so we have $r \le C G^{\frac{1}{2\alpha}}$, and that $\Delta_E \le C G^{-0.5}$.


{\bf $\textsf{ATT}$ normality.}

For estimation of $\textsf{ATT}$, we have that $M = M_1 = N_1$ and $M_0 = 0$.

\noindent
{\em 1. $\frac{1}{\bar{\sigma}}  \ldot{\Delta_{\beta^{(a)}}}{\varepsilon_{\Ic^{(a)}}}$ term.}

\noindent
%
Using \eqref{eq:ate_est_final_3} and the assumption that $C \sqrt{M}< \bar{\sigma}$, we have 
\begin{align}
%
\sum_{a \in \{0, 1\}}\frac{1}{\bar{\sigma}}\ldot{\Delta_{\beta^{(a)}}}{\ \varepsilon_{\Ic^{(a)}}}
%
= O_p\left( \sum_{a \in \{0, 1\}} \frac{\|\Delta_{\beta^{(a)}}\|_2 \cdot \sigma_\max}{\sqrt{M}}\right)
\end{align}
%
Using \eqref{eq:summary_2} and \eqref{eq:ATT_normality_helper_1}, we have 
%
\begin{align}
%
\sum_{a \in \{0, 1\}}\frac{\|\Delta_{\beta^{(a)}}\|_2}{\sqrt{M}}
%
&\le C \cdot \ln^3(\bar{T} N_0) \cdot \sqrt{N_1} \cdot \left[G^{0.5(\frac{1}{\alpha} - 1) - w} \right]
%
\\ &\le C \cdot \ln^3(\bar{T} N_0) \cdot \sqrt{N_1} \cdot \left[G^{-0.5} \right] \label{eq:ATT_normality_PCR_1}
%
\\ &= o_p(1) \label{eq:ATT_normality_PCR_2}
\end{align}
%
where in \eqref{eq:ATT_normality_PCR_1}, we used $w > \frac{1}{2\alpha}$. In \eqref{eq:ATT_normality_PCR_2}, we used $N_1 = o(\min(N_0, \bar{T}))$.

\noindent
{\em 2. $\frac{1}{\bar{\sigma}}\ldot{\Delta_{\beta^{(a)}}}{\Ex\left[ Y_{t, \Ic^{(a)}} \mid \Omega, \mathsf{U}\right]}$ term.}



\noindent
{\em 3. $\frac{N}{\bar{\sigma}}  \mathsf{Approx}_t$ term.}

\noindent
\begin{align}
\frac{N}{\bar{\sigma}}  \mathsf{Approx}_t 
%
&= \frac{1}{\bar{\sigma}} \left(\sum_{a \in \{0, 1\}}  \sum_{n \in\Ic^{(1-a)}_{t}} \eta^{(a)}_{n, t} - \sum_{n \in\Ic^{(a)}} \beta^{(a)}_j \eta^{(a)}_{n, t} \right)
%
\\&\le \Delta_E \left(\sqrt{N} + \frac{\| \beta^{(0)}\|_1 + \| \beta^{(1)}\|_1}{\sqrt{N}} \right)
%
\\&\le C \left(\frac{1}{N}\right)^{ \gamma \alpha} \cdot \left(\sqrt{N} + \frac{\| \beta^{(0)}\|_1 + \| \beta^{(1)}\|_1}{\sqrt{N}} \right)
%
\\&\le C \left(\frac{1}{N}\right)^{ \gamma \alpha} \cdot \left(\sqrt{N} + \frac{N^{\frac{3}{2} - w}}{\sqrt{N}} \right)
%
\\&= C \cdot \left(N^{(\frac{1}{2} - \gamma \alpha)} + N^{1 - \gamma \alpha - w} \right)
%
\end{align}
%
Thus for $\frac{N}{\bar{\sigma}}  \mathsf{Approx}_t = o_p(1)$, we require that
\begin{align}
%
\gamma \alpha > \frac{1}{2}, \quad \gamma \alpha + w > 1.
%
\end{align}
